The price of ignorance: how much does it cost to forget noise structure in low-rank matrix estimation?

We consider the problem of estimating a rank-1 signal corrupted by structured rotationally invariant noise, and address the following question: how well do inference algorithms perform when the noise statistics is unknown and hence Gaussian noise is assumed? While the matched Bayes-optimal setting with unstructured noise is well understood, the analysis of this mismatched problem is only at its premises. In this paper, we make a step towards understanding the effect of the strong source of mismatch which is the noise statistics. Our main technical contribution is the rigorous analysis of a Bayes estimator and of an approximate message passing (AMP) algorithm, both of which incorrectly assume a Gaussian setup. The first result exploits the theory of spherical integrals and of low-rank matrix perturbations; the idea behind the second one is to design and analyze an artificial AMP which, by taking advantage of the flexibility in the denoisers, is able to "correct" the mismatch. Armed with these sharp asymptotic characterizations, we unveil a rich and often unexpected phenomenology. For example, despite AMP is in principle designed to efficiently compute the Bayes estimator, the former is outperformed by the latter in terms of mean-square error. We show that this performance gap is due to an incorrect estimation of the signal norm. In fact, when the SNR is large enough, the overlaps of the AMP and the Bayes estimator coincide, and they even match those of optimal estimators taking into account the structure of the noise.

==> images/sections/01Intro.tex <==
\jean{
In spiked matrix models, a rank-1 signal wants to be estimated from a matrix of noisy observations. These models have many applications in different fields including machine learning, principal component analysis (PCA, from now on), and image processing, among others. In these applications, the high-dimensional limit of the model is of particular interest. That is, the limit in which the dimension of the data matrix (and thus, also of the signal) go to infinity. Most of the standard approaches for this model require the statistician to specify the statistical properties of the noise involved. The most common assumption for it is to assume that the noise matrix has i.i.d. gaussian components (i.e., it is a \emph{Wigner matrix}). Nevertheless, in many practical situations this may not be a realistic assumption as the noise's components may be correlated in some complicated way. In this paper we study the impact on the quality of the estimation on a rank-1 matrix factorization setting when the statistician wrongfully assumes the noise to be given by a Wigner matrix but in reality it comes from a rotationally invariant ensemble with correlated components.

Specifically, in spiked matrix models the statistician is interested in recovering a matrix of the form $X X^T$ constructed from a random vector $X\in\R^N$ through some noisy observations $\bY = \sqrt{\frac{\lambda}{N}} X X^T + \bZ$; where $N\geq1$ is the dimension of the system, $\lambda > 0$ is a fixed constant that quantifies the signal strength, and $\bZ\in\R^{N\times N}$ is a random matrix that gives the noise. In this context, the high-dimensional limit is given by the dimension parameter $N$ going to infinity. In this limit, non-trivial estimation is obtained when the norm of $X$ and the eigenvalues of $\bZ$ are of order $\sqrt{N}$. In this paper we will be concerned with a situation in which the noise $\bZ$ comes from a rotationally invariant ensemble; that is, is of the form $\bO^T \bD \bO$ with $\bO\in\R^{N\times N}$ some random rotation sampled from the Haar measure on the orthogonal group in $\R^N$ and $\bD:=\mbox{diag}(\gamma_1,\dots,\gamma_N)\in\R^{N\times N}$ is some diagonal matrix containing the eigenvalues of $\bZ$. Although the noise will be assumed to come from this distribution, we will study the case in which the statistician models it as a Wigner matrix (a matrix ensemble with independent and normally distributed components).

The results obtained for this model include characterizations of the \emph{mismatched Bayes estimator} (obtained through the wrong likelihood corresponding to a model with gaussian noise) and algorithmic results for the \emph{mismatched AMP algorithm} (constructed using the optimal denoiser for a model with gaussian noise). For the analytical results for Bayes estimator the heuristic replica method from physics to obtain a general prediction on the \emph{mean square error} (MSE) obtained by this estimator. We also present rigorous proof for the MSE formula for the model with a spherical prior and for the free entropy in the gaussian case. These are based on a combination of large deviation techniques along with a previous characterization of spherical integrals and the spectrum of low-rank perturbations of rotationally invariant matrices. We then use these results to approach the main questions of the paper: how does the estimation of the spike in a model in this model with mismatch compare to the case where the noise is really gaussian? What is the relationship between Bayes estimator, AMP, and PCA in this context?


\subsection{Background and related works}

Spiked matrix models have been for a long time one of the central models for the analysis of threshold phenomena in high-dimensional statistics. Some of the first rigorous results on these models relied on spectral techniques to establish information theoretical limits for the inference of the spike. On more recent works, these have been complemented with finite size bounds and the analysis of variants where the spike comes from a sparse vector. Closer to the scope of this paper, the performance of PCA for spiked matrix models with rotationally invariant noise has been studied using spectral methods. Also, in [X] the authors study spiked matrix models with Wigner noise but in a setting where there is possible a mismatch in the signal to noise ratio and the strength of the noise. Some of the proofs present here are extensions of the one given there.

As pointed out above, in this work we will analyze the mismatched spiked matrix model studied by comparing the performances of three families of estimators: Bayes estimators, Approximate Message Passing algorithms (AMP), and Principal Component Analysis (PCA) with different scalings. For the characterization of PCA, we use the results of [X] already cited above. While for the rest of the analytical results, we use a combination of the replica method, large deviations, and adaptations of convergence bounds for AMP.


As in [X], for the rigorous characterization of the MSE of the mismatched Bayes estimator we use existing results on the asymptotic value of spherical integrals [X] along with the results on the spectrum of low-rank perturbations of rotationally invariant matrices present in [X]. These results allow to compute the free entropy of the model in the case when the priors are either spherical or gaussian. In the gaussian case, we apply some straightforward large deviation tools as presented in [X]. It is important to point out that there are not many rigorous results on inference problems with mismatch, two exceptions being [X][X]. This is due to inherent complications that appear in mismatched settings that make most of the usual approaches fail.

From an algorithmic perspective, AMP constitutes a family of iterative algorithms with two particularly attractive features: \emph{(i)} they can be tailored to take advantage of prior information on the structure of the signal; and \emph{(ii)} under suitable model assumptions, their performance in the high-dimensional limit is precisely characterized by a succinct deterministic recursion called \emph{state evolution} \cite{bayati2011dynamics, bolthausen2014iterative, javanmard2013state}.  
AMP algorithms have been applied to a wide range of inference problems: estimation in linear models \cite{lassoMontanariBayati,bayati2011dynamics,Donoho10112009,  Krzakala_CS,maleki2013asymptotic}, generalized linear models \cite{barbier2019optimal,ma2019optimization, maillard2020phase,mondelli2021approximate,rangan2011generalized,schniter2014compressive,sur2019modern}, and
low-rank matrix estimation with Gaussian noise \cite{barbier2020all,6875223,fletcher2018iterative,kabashima2016phase, lesieur2017constrained,montanari2017estimation}. The survey \cite{feng2021unifying} provides a unified description of AMP for these applications. Using the state evolution analysis, it has been proved that AMP achieves Bayes-optimal performance in some Gaussian models \cite{6875223,donoho2013information, montanari2017estimation}, and a bold conjecture from statistical physics posits that AMP is optimal among polynomial-time algorithms. Here we will study two AMP algorithms for this model: a mismatched AMP that implements the optimal denoiser for gaussian noise and the variant of AMP proposed in [X] and studied rigorously in [X] for rotationally invariant noise.
}

\subsection{Summary of contributions}

The main contributions that are derived from the results of the paper are the following:

\begin{itemize}
    \item We provide rigorous algorithmic performance guarantees in an emblematic inference problem: structured PCA, modeled using a spiked matrix model. Although simple the model presents a strong mismatch that makes usual techniques not applicable.
    \item Our analysis combines the complementary points of view of Bayesian inference along side with important practical algorithms.
    \item The Bayes estimator presents unexpected behaviors. For example, even though there is mismatch, for certain noise distributions the Bayes estimator performs better than with Wigner noise (i.e., without mismatch): some noise structures help even if unknowns.
    \item Surprisingly, the gaussian AMP does not necessarily match the gaussian Bayes estimator. The mismatch thus implies that AMP does not approximately sample the posterior. 
    \item We also show that, similarly to the Bayes-optimal case with Wigner noise, a properly scaled version of the PCA estimator matches the Bayes estimator. Moreover, another scaling of PCA yields the same performance as the fined-tuned structure-exploiting AMP.
\end{itemize}

These conclusions emphasize that unexpected phenomena result from the presence of mismatch in the model and the structure of the noise present in the data. They open many general questions for future research.

% \subsection{Structure of the paper}

% \jean{
% The rest of the paper is structured in the following way. On Section \ref{sec:setting} we define precisely the model considered and present some technical results from bibliography that will be needed later on. After that, in Section \ref{sec:mainres}, we present the main results of the paper. These include the computation of the replica fixed point equations, the MSE for the Bayes estimator with spherical priors, and the characterization of algorithmic performance of AMP and PCA. In Section \ref{sec:applic}, we apply the results derived on the previous section to some relevant examples and discuss their implications. All the proofs of our results are deferred to Appendices \ref{app:proofAMP} and \ref{app:proofBayes}.
% }

==> images/sections/02ModelResults.tex <==
\subsection{Description of the model}

Vectors are always considered as column vectors and their transpose as rows. Let $\bX\in \mathbb{R}^N$ a random vector uniformly distributed on the sphere $\mathbb{S}^{N-1}(\sqrt{N})$ of dimension $N$ and radius $\sqrt{N}$. Consider a data matrix $\bY\in\R^{N\times N}$ given by
\begin{align}\label{eq:spikedmodel}
    \bY = \frac{\sqrt{\lambda_*}} {N} \bX\bX^\intercal + \bZ
\end{align}
where $\bZ\in\R^{N\times N}$ is a symmetric random matrix which represents additive noise and $\lambda_*\in\mathbb{R}_{\ge 0}$ is the signal-to-noise ratio (SNR). The rank-one \emph{spike} $\bX\bX^\intercal$ represents the information to be retrieved; given that $\bX$ is spherical it is essentially structureless. In the special case when the noise $\bZ$ is a standard Wigner matrix, the resulting model is a paradigmatic case study of phase transition phenomena in high-dimensional inference which is often called \emph{spiked Wigner model}, whose study has lead to the understanding of the famous BBP transition \cite{baik2005phase}.

We assume that the noise $\bZ$ is a random matrix drawn from a \emph{rotationally-invariant ensemble} with some deterministic spectrum with $\mathcal{O}(1)$ elements. In other words, there exist some constants $\gamma_1,\dots,\gamma_N\in\R$ independent of $N$ and a diagonal matrix $\bSig := \mbox{diag}(\gamma_1,\dots,\gamma_N)\in\R^{N\times N}$ such that 
\begin{align}
    \bZ \overset{\rm d}{=} \bO\bSig\bO^\intercal	\label{Z_eigen}
\end{align}
where $\bO$ is distributed according to the Haar measure over the group $\mathcal{O}(N)$ (i.e., it is a uniform). Let $\overline{\gamma}_N$ and $\underline{\gamma}_N$ denote $\max\{\gamma_1,\dots,\gamma_N\}$ and $\min\{\gamma_1,\dots,\gamma_N\}$, respectively. Similarly, we will let $\eigmax_N$ and $\underline{\nu}_N$ be the largest and smallest eigenvalues of the data matrix $\bY$.
%Here, the diagonal matrix $\bSig={\rm diag}(\Sigma_1,\dots,\Sigma_N)$ has eigenvalues that are assumed to be of order $1$ and . 

Throughout the paper, the main technical assumption will be the following.
\begin{hypothesis}\label{hyp:eigen} 
    The empirical measure $N^{-1}\sum_{i\leq N} \delta_{\gamma_i}(\cdot)$ of eigenvalues of the noise matrix $\bZ$ converges weakly towards a limiting measure $\rho(\cdot)$ of compact support $K\subseteq\R$. Moreover, $\overline{\gamma}_N$ and $\underline{\gamma}_N$ converge a.s. to the constants $\overline{\gamma}:=\max  K$ and $\underline{\gamma}:=\min  K$, respectively.
\end{hypothesis}
\noindent
As explained in Appendix \ref{app:PCA}, under the above hypothesis we have that $\eigmax_N$ and $\underline{\nu}_N$ converge a.s. to well defined finite limits which we will denote by $\eigmax$ and $\underline{\nu}$, respectively. These have an explicit form in terms of $\rho(\cdot)$ and $\lambda_*$ given in \cite[Theorem 2.1]{benaych2011eigenvalues} and which we reproduce for convenience in the appendix.
% That is, we assume that the empirical distribution of eigenvalues of $\bZ/\sqrt{N}$ converges to some weak limit of compact support and its extreme eigenvalues converge a.s. to the extremes of this support.

If $\rho$ is the semicircle law of radius $2$ then the noise matrix $\bZ=\bW$ is asymptotically equal in distribution to a standard Wigner matrix with density $\sim \exp(-\frac N4\Tr\bW^2)$. Because the independent elements of this type of symmetric matrices are i.i.d. gaussian, in this case we say that there is \emph{gaussian noise}. For other limiting $\rho$ the elements of the matrix $\bZ\neq \bW$ remain correlated and thus it is said that there is \emph{structured noise}. To distinguish between structured and gaussian noise, we will denote by $\bW$ sequence of matrices asymptotically distributed as standard Wigner matrices while we will reserve $\bZ$ for generic sequences of rotationally invariant matrices. 

In the present contribution we consider what happens when there is a mismatch between the assumptions on the noise statistics made by the statistician performing the inference and the true noise statistics, in particular when a wrong \emph{gaussian statistics} is assumed. Gaussianity is probably the most standard assumption made when precise knowledge is lacking. More precisely, despite the noise $\bZ$ not being a Wigner matrix, because of her ignorance of its spectral measure $\rho$ the statistician assumes $\bZ$ to be a Wigner matrix. Secondly, she may also assume a wrong incorrect value for the SNR $\lambda\neq \lambda_*$. In other words, she wrongly assumes that data $\bY$ is equal to some $\bY_W$ generated according to 
\begin{align}
\bY_W = \frac{\sqrt{\lambda}}N \bX\bX^\intercal + \bW    
\end{align}
instead of the correct model \eqref{eq:spikedmodel}.
% \begin{itemize}
% 	\item When the measure $P_\bX(\cdot)$ associated to the random vector $\bX$ is known, we will assume it is used by the statistician to construct her model. On the other hand, if $P_\bX(\cdot)$ is unknown to the statistician, we will assume she uses as the prior for the signal a standard gaussian measure on $\R^N$.
% 	\item Despite the noise $\bZ$ not being a Wigner matrix, because the asymptotic spectral measure $\rho$ is unknown to the statistician, she assumes it to be a Wigner matrix. In other words, she wrongly assumes that the observation matrix $\bY$ is equal to some $\bY_W$ generated according to $$\bY_W \overset{d}{=} \sqrt{\frac\lambda N} \bX\bX^\intercal + \bW.$$
% \end{itemize}
Our goal is to quantify how this ignorance affects her performance. 

\subsection{Three classes of inference algorithms for PCA}

%
% During our analysis of the Bayesian estimator associated to the model proposed by the statistician, we will focus on three different situations:
% %
% \begin{enumerate}
% 	\item[$(A)$] The Bayesian-optimal setting on which the noise is in fact a standard Wigner matrix $\bW$ and the distribution of the signal $\bX$ is known. The resulting posterior is then given by
% 	\begin{align*}
%     	P_{\rm opt}(d\bx \mid \bY_W)&=\frac{1 }{Z_{N,{\rm opt}}(\bY_W)}  \exp\Big(\sqrt\frac{\lambda}{4N}\bx^\intercal\bY_W\bx -\frac{\lambda}{4N}\|\bx\|^4\Big)\,P_X(d\bx)   \\ %\label{postOpt}
%     	& = \frac{1}{Z'_{N,{\rm opt}}} \exp\Big(-\frac14\Tr\Big[\bY_W-\sqrt\frac{\lambda}{N}\bx\bx^\intercal \Big]^2\Big)\,P_X(d\bx)\nonumber;
% 	\end{align*} 
% 	where, as before, $P_X(\cdot)$ is the probability measure associated to $\bX$.
% 	\item[$(B)$] A second setting where the correct prior $P_X(\cdot)$ is still known but the noise is not given by a Wigner matrix. Instead, it is a generic rotationally invariant matrix distributed according to \eqref{Z_eigen}. Yet the statistician assumes the noise is Wigner and therefore uses the following (mismatched) posterior distribution:
% 	\begin{align*}
%     	&P_{{\rm mis}\, 1}(d\bx\mid \bY)=\frac{1}{Z_{N,{{\rm mis}\, 1}}(\bY)}  \exp\Big(\sqrt\frac{\lambda}{4N}\bx^\intercal\bY\bx -\frac{\lambda}{4N}\|\bx\|^4\Big)\,P_X(d\bx) . %\label{estimatorMis1}
% 	\end{align*}	
% \end{enumerate}
% In all these posterior distributions, $Z_{N,{\rm opt}},Z'_{N,{\rm opt}},Z_{N,{\rm mis}\,1},Z_{N,{\rm mis}\,2} > 0$ are normalizing constants. 
%
\noindent \textbf{Mismatched Bayes estimator.}\ \ The mismatched posterior distribution reads, using the mismatched gaussian log-likelihood $-\frac N4\Tr[\bY-\sqrt{\lambda/N}\bx\bx^\intercal ]^2$,
    \begin{align}
        P_{{\rm mis}}(d\bx\mid \bY)&=\frac{1}{Z_{N}(\bY)}  \exp\Big(\frac{\sqrt\lambda}{2N}\bx^\intercal\bY\bx \Big)\,\mu_N(d\bx) \label{estimatorMis1}
    \end{align}    
where $Z_{N}(\bY)$ is the normalization constant and $\mu_N$ is the uniform measure over $\mathbb{S}^{N-1}(\sqrt{N})$. The Bayes estimator we analyze is obtained as the posterior mean
%
\begin{align}
 M_{\rm mis}(\bY):= \int \bx \bx^{\intercal} P_{{\rm mis}}(d\bx\mid \bY)  \label{BayesEst},
\end{align}
which may not be practical to compute. We will also consider the estimation performance of spectral PCA and two versions of AMP for the setting described above. Notice that if the noise is Wigner $\bZ=\bW$ then the posterior \eqref{estimatorMis1} is correct. This Bayesian-optimal setting has already been thoroughly studied and rigorously characterized (see, for example, \cite{barbier2019adaptive,lelarge2019fundamental}). It will serve us as a base case for comparison with the mismatched case studied here.

The performance of a sequence of estimators $M_N(\bY)=M(\bY)\in\R^{N\times N}$ of the spike $\bX\bX^\intercal$ will be quantified using its asymptotic mean-square error (MSE). E.g., for the Bayes estimator it reads
%
\begin{align*}
    {\rm MSE}(M_{\rm mis})=\lim_{N\to+\infty} \frac{1}{2 N^2} \E\| \bX \bX^\intercal-M_{\rm mis}(\bY) \|_{\rm F}^2;
\end{align*}
with $\|\cdot\|^2_{\rm F}$ the Frobenius norm and $\mathbb{E}$ the expectation over the problem instance (i.e., the spike $\bX\bX^T$ and the noise $\bZ$).
% Another quantity of main interest is expected \emph{free entropy}
%
%\begin{align}
%f_{{\rm mis},N}&:=\frac1N\E\ln Z_{N}(\bY)
%\end{align}
%that we will later connect to the MSE of the Bayes estimator.


\noindent \textbf{Approximate message passing.}\ \ We will need that $\|\bX\|/\sqrt{N}$ is bounded by a constant (independent of $N$) \mm{I'll need finite second moment of $X$} and the eigenvalues of $\bZ$ are $\Theta(1)$\mm{I'll need that $\bZ$ has bounded operator norm}. We consider the following approximate message passing (AMP) algorithm to estimate $\bX\in\mathbb R^N$ from the data matrix $\bY\in \mathbb R^{N\times N}$. For simplicity, we assume to have access to an initialization $\hat{\bx}^1\in \mathbb R^N$, which is independent of the noise $\bZ$ and has a strictly positive correlation with $\bX$, i.e., 
\begin{equation}\label{eq:AMPinit}
(\bX, \hat{\bx}^1)\stackrel{\mathclap{W_2}}{\longrightarrow} (X, \hat{x}_1), \quad \mathbb E[X \,\hat{x}_1]:=\epsilon>0, \quad \mathbb E[\hat{x}_1^2]\le 1.
\end{equation}
We note that this initialization is impractical and one can initialize AMP with the principal component analysis (PCA) estimate, see e.g. \cite{mondelli2021pca,zhong2021approximate}. 
Then, for $t\ge 1$, we compute:
\begin{equation}\label{eq:AMP}
\bx^t = \bY\hat{\bx}^t-\beta_t\hat{\bx}^{t-1},\quad \hat{\bx}^{t+1} = h_{t+1}(\bx^t),
\end{equation} 
where we assume that $\hat{\bx}^{0}=\bzero$.
Here, the function $h_{t+1}:\mathbb R\to\mathbb R$ is applied component-wise; $\beta_1=0$ and, for $t\ge 2$, $\beta_t=\langle h_t'(\bx^{t-1}) \rangle$, where $h_t'$ denotes the first derivative of $h_t$.

\noindent \textbf{Spectral PCA.}\ \ We also consider spectral estimators proportional to the rank-1 matrix obtained by the tensor product of the unit-norm eigenvector $\overline{\bv}_N$ associated to the largest eigenvalue $\overline{\nu}_N$ of the data matrix with itself. In other words, these are estimators of the form $C \overline{\bv}_N\overline{\bv}_N^T$; with $C > 0$ some scaling constant that takes into account the spectrum of the data matrix. The asymptotic description of $\overline{\bv}_N$ and $\overline{\nu}_N$ for low rank perturbations of rotationally invariant matrices has been obtained in \cite{benaych2011eigenvalues,benaych2012singular}; we recall these results in Appendix \ref{app:PCA}. In particular, by \cite[Theorem 2.2]{benaych2012singular}, under Hypothesis \ref{hyp:eigen} $|\bX^T \overline{\bv}_N|^2/N$ converges a.s. to some constant $C(\rho,\lambda_*)$. In Appendix \ref{app:PCA} we give the explicit expression for this constant.

There are two variants of spectral estimators that we study:
\begin{itemize}
    \item \emph{Optimal spectral estimator (OptSpec):} given by $M_{OS} := C_{\rm SO} \overline{\bv}_N\overline{\bv}_N^T$, where $C_{\rm SO}$ is the optimal scaling that minimizes the MSE given by $C_{\rm SO}(\rho,\lambda_*) := C(\rho,\lambda_*)$.
    \item \emph{Gaussian mismatched spectral estimator (GauSpec):} given by $M_{\rm GS} := C_{\rm GS} \overline{\bv}_N\overline{\bv}_N^T$, where $C_{\rm GS}$ is the optimal scaling if the noise were Wigner and the SNR was equal to $\lambda > 0$. If $\rho_{SC}(\cdot)$ is the standard semi-circle law, we have $C_{\rm GS}(\lambda) := C(\rho_{SC},\lambda)=(1 - 1/\lambda)$.
\end{itemize}
Notice that while (OptSpec) requires knowing exactly the statistics of the noise and the SNR, (GauSpec) represents the spectral estimator that would be used by a statistician that assumes the noise is Wigner and the SNR has value $\lambda$. From the definitions of these estimators and \cite[Theorem 2.2]{benaych2012singular} we have that
\begin{equation*}
    {\rm MSE}(M_{\rm OS}) = \frac{1}{2}(1 - C^2(\rho,\lambda_*)) \,\, \mbox{  and  } \,\, {\rm MSE}(M_{\rm GS}) = \frac{1}{2}(1 + (1 - 1/\lambda)^2 - 2(1 - 1/\lambda) C(\rho,\lambda_*)).
\end{equation*}
Observe that ${\rm MSE}(M_{\rm GS}) = {\rm MSE}(M_{\rm OS}) + \frac{1}{2}\big( C(\rho,\lambda_*) - (1 - 1/\lambda)\big)^2$. Thus, as expected, we have ${\rm MSE}(M_{\rm OS}) \leq {\rm MSE}(M_{\rm GS})$.



% \subsection{Some definitions}
% We define the rank-one log-spherical integral:
% %
% \begin{align}
%  \phi_N(\theta,\bSig):= \frac1N \ln \int \mu_N(d\bO)  \exp \Big(N\theta \sum_{i\le N}O_{i1}^2\Sigma_i\Big) 
% \end{align}
% It has a well-studied asymptotic limit which is a functional of the asymptotic limit $\rho$ of the empirical spectrum of $\bSig$ given by ??
% %
% \begin{align}\label{rankonespherical}
%  \phi_\rho(\theta) :=\lim_{N\to+\infty}\phi_N(\theta,\bSig)=\theta g(\theta)-\frac12\int d\rho(x)\ln\big(1+2\theta (g(\theta) - x)\big),
% \end{align}
% where
% \begin{align}\label{funcg_sphInt}
% g(\theta)=
% \begin{cases}
% R_\rho(2\theta) \quad \mbox{if}\ H_{\rm min} \le 2\theta \le \hmax,\\
% \lambda_{\rm max}    -\frac{1}{2\theta} \quad \mbox{if}\  2\theta > \hmax,\\
% \lambda_{\rm min}    -\frac{1}{2\theta} \quad \mbox{if}\  2\theta < H_{\rm min}.\\
% \end{cases}    
% \end{align}
% Let us define the various quantities appearing above. Let ${\rm supp}(\rho):=[\lambda_{\rm min},\lambda_{\rm max}]$ the uniform in $N$ support of $\rho$. The Hilbert transform, with domain $\mathbb{R}\,\backslash\,{\rm supp}(\rho)$, is
% %
% \begin{align}
%  H_\rho(x)  =\int d\rho(\lambda)\frac1{x-\lambda}.
% \end{align}
% The R-transform with domain $H_\rho(\mathbb{R}\,\backslash\, {\rm supp}(\rho))$ is defined from the functional inverse of the Hilbert transform as
% %
% \begin{align}
%  R_\rho(x)=  H_\rho^{-1}(x) -\frac1x.
% \end{align}
% Then the quantities $H_{\rm min}:=\lim_{x\uparrow \lambda_{\rm min}} H_\rho(x)$ and $\hmax:=\lim_{x\downarrow \lambda_{\rm max}} H_\rho(x)$. Finally, it can be shown (??) that in the first regime $H_{\rm min} \le 2\theta \le \hmax$, then one equivalently has the simplest expression
% %
% \begin{align}\label{rankonespherical_Rtrans}
%  \phi_\rho(\theta) =\frac12 \int_0^{2\theta} R_\rho(x)dx.
% \end{align}


% To state our results, we will need a series of functions depending on the asymptotic eigenvalue distribution. Let $H_\rho : \R\backslash K \to \R$ be the Hilbert transform of the distribution $\rho(\cdot)$ given by
% \begin{equation*}
%     H_\rho(z) := \int_ K \frac{\rho(d\gamma)}{z-\gamma}. \quad \mbox{Also let} \ \ \hmax := \lim_{z\downarrow\Sigma_{\rm max}} H_\rho(z),\ \ H_{\rm min} := \lim_{z\uparrow \Sigma_{\rm min}} H_\rho(z)
% \end{equation*}
% %Define also $\hmax := \lim_{z\downarrow\Sigma_{\rm max}} H_\rho(z)$ and $H_{\rm min} := \lim_{z\uparrow \Sigma_{\rm min}} H_\rho(z)$ 
% which can be infinite. Because $H_\rho$ is a bijection between $\R\backslash K$ and its image $(H_{\rm min},\hmax)\backslash\{0\}$, it has some inverse 
% \begin{equation*}
%     K_\rho :(H_{\rm min},\hmax)\backslash\{0\}\mapsto\R\backslash K.
% \end{equation*}
% We will then define the \emph{R-transform of} $\rho(\cdot)$ as the function
% \begin{equation*}
%     R_\rho:(H_{\rm min},\hmax)\backslash\{0\}\mapsto\R\backslash K \quad \mbox{given by} \quad R_\rho(x) := K_\rho(x) - 1/x.
% \end{equation*}
% % Finally, for every $\theta > 0$ and matrix $\bA\in\R^{N\times N}$ the rank-1 spherical integral is
% % \begin{equation*}
% %     I_N(\theta,\bA) := \int d\mu_N(\bs) \exp\big(\theta \bs^\intercal\bA \bs\big).
% % \end{equation*}
% %When the arguments are clear, we will sometimes omit them and write $I_N$. 

==> images/sections/03Replica.tex <==
% \subsection{One-step replica symmetry breaking theory}
% In this section we perform a replica analysis at the one-step replica symmetric level for a generic mismatched model. All three settings $(A)$, $(B)$ and $(C)$ will be special cases. 

% We thus consider a setting where both the prior and noise statistics are possibly mismatched. Namely we consider the free entropy (we denote the statistician's prior $P_x(d\bx):=\prod_{i\le N} p_x(dx_i)$)
% \begin{align*}
%     f_N &:= \frac{1}{N}\E \ln \int P_x(d\bx) \exp\Big(\sqrt\frac{\lambda}{4N}\bx^\intercal\bY\bx -\frac{\lambda}{4N}\|\bx\|^4\Big)\\
%     &=\frac{1}{N}\E \ln \int P_x(d\bx)  \exp\Big(\frac{\lambda}{2N}(\bX\cdot\bx)^2+\sqrt\frac{\lambda}{4N}\bx^\intercal\bZ\bx -\frac{\lambda}{4N}\|\bx\|^4\Big).
% \end{align*}
% When $P_x=P_X$ it means the correct prior is known and used, and when $\bZ=\bW$ then the correct noise statistics is assumed. If we denote by $Z_N$ the partition function defined by the integral argument of the logarithm above, the replica trick reads
% %
% $$\lim_{N\to+\infty} f_N=\lim_{N\to+\infty} \frac1N\EE\ln Z_N=\lim_{k\to 0_+}\lim_{N\to+\infty} \frac{d}{dk}\frac1N\ln \EE Z_N^k
% $$
% where we assumed the commutation of the $k$ and $N$ limits. We thus compute the following (integer) moments; the expectation below does not act on the noise eigenvalues $\bSig$ which are fixed, but it does act on its Haar distributed eigenbasis $\bO$ (recall \eqref{Z_eigen}):
% \begin{align}
%         \E Z_N^k & =  \int\Big(\prod_{\ell\le k} P_x(d\bx^\ell)\Big)\,P_X(d\bX)\, \exp\sum_{\ell \le k}\Big(\frac{\lambda}{2N}(\bX\cdot \bx^\ell)^2 -\frac{\lambda}{4N}\|\bx^\ell\|^4\Big)\nonumber \\
%         &\qquad\qquad\times \int \mu_N(d\bO)  \exp N \tr\Big[\sqrt\frac{\lambda}{4} \bO\bSig\bO^\intercal \frac1N\sum_{\ell \le k} \bx^\ell(\bx^\ell)^\intercal \Big].
% \end{align}
% Given that the rank $k$ of the singular positive definite matrix $\bA:=N^{-1}\sum_{\ell \le k} \bx^\ell(\bx^\ell)^\intercal$ will remain finite when the rank $N$ of the full-rank $\bSig$ will diverge, the integral over $\bO$ at the second line above is a low-rank spherical integral that can be evaluated. To do so we need to find the $k$ non-zero eigenvalues $(a_j)_{j\le k}$ of $\bA$; its eigenbasis is irrelevant as it can be absorbed in the random $\bO$. The $(a_j)$ are complicated functions of all overlaps $\bx^\ell\cdot \bx^{\ell'}$ between the pairs of replicas, as well as of their norm. So in order to continue the computation we need here to make an ansatz. 

% We are soon going to enforce that the $k\times k$ symmetric overlap matrix 
% $$\bQ:=\Big(\frac{\bx^\ell\cdot  \bx^{\ell '}}N \Big)_{\ell,\ell'\le k}$$ 
% has a one-step replica symmetry breaking (1RSB) form. To define this form we first need to partition the replica indices into $k/t$ distinct groups (i.e., sets) each of cardinal $t$: $\{1,2,\ldots,t\},\{t+1,\ldots,2t\},\ldots,\{k-t+1,\ldots,k\}$. With this partitioning we can now define how the overlap matrix would look like if we enforce a $1$RSB structure:
% %
% \begin{align}\label{1RSBansatz}
% \mbox{1RSB ansatz:}\quad \begin{cases}
%  Q_{\ell\ell'}=Q_{\ell'\ell} = q_1 \   &\mbox{if} \ 1\le \ell< \ell'\le k\ \mbox{are in a same group},\\ 
%  Q_{\ell\ell'}=Q_{\ell'\ell} = q_0 \ &\mbox{if} \ 1\le \ell< \ell'\le k\  \mbox{are in different groups},\\
% Q_{\ell\ell} \hspace{3pt} = v \ &\mbox{for} \ 1\le \ell \le k.
% \end{cases}.
% \end{align}
% With this form the overlap matrix is parametrized by only four non-negative parameters $(q_0, q_1, v, t)$ with $v\ge q_1\ge q_0\ge 0$. Matrix $\bA$ has same eigenvalues as the block matrix $\bQ$ and these are (to show):
% %
% \begin{align}
% \begin{cases}
%     \lambda_1=v-q_1 \ &\mbox{of degeneracy} \ k(t-1)/t,\\
%     \lambda_2=v-(1-t)q_1-tq_0 \ &\mbox{of degeneracy} \ (k-t)/t,\\
%     \lambda_3=v-(1-t)q_1-(t-k)q_0 \ &\mbox{of degeneracy} \ 1.
% \end{cases}    
% \end{align}

% We define the rank-one log-spherical integral:
% %
% \begin{align}
%  \phi_N(\theta,\bSig):= \frac1N \ln \int \mu_N(d\bO)  \exp N\theta \sum_{i\le N}O_{i1}^2\Sigma_i 
% \end{align}
% It has a well-studied asymptotic limit which is a functional of the asymptotic limit $\rho$ of the empirical spectrum of $\bSig$ given by ??
% %
% \begin{align}\label{rankonespherical}
%  \phi_\rho(\theta) :=\lim_{N\to+\infty}\phi_N(\theta,\bSig)=\theta g(\theta)-\frac12\int d\rho(x)\ln\big(1+2\theta (g(\theta) - x)\big),
% \end{align}
% where
% \begin{align}\label{funcg_sphInt}
% g(\theta)=
% \begin{cases}
% R_\rho(2\theta) \quad \mbox{if}\ H_{\rm min} \le 2\theta \le \hmax,\\
% \lambda_{\rm max}    -\frac{1}{2\theta} \quad \mbox{if}\  2\theta > \hmax,\\
% \lambda_{\rm min}    -\frac{1}{2\theta} \quad \mbox{if}\  2\theta < H_{\rm min}.\\
% \end{cases}    
% \end{align}
% Let us define the various quantities appearing above. Let ${\rm supp}(\rho):=[\lambda_{\rm min},\lambda_{\rm max}]$ the uniform in $N$ support of $\rho$. The Hilbert transform, with domain $\mathbb{R}\,\backslash\,{\rm supp}(\rho)$, is
% %
% \begin{align}
%  H_\rho(x)  =\int d\rho(\lambda)\frac1{x-\lambda}.
% \end{align}
% The R-transform with domain $H_\rho(\mathbb{R}\,\backslash\, {\rm supp}(\rho))$ is defined from the functional inverse of the Hilbert transform as
% %
% \begin{align}
%  R_\rho(x)=  H_\rho^{-1}(x) -\frac1x.
% \end{align}
% Then the quantities $H_{\rm min}:=\lim_{x\uparrow \lambda_{\rm min}} H_\rho(x)$ and $\hmax:=\lim_{x\downarrow \lambda_{\rm max}} H_\rho(x)$. Finally, it can be shown (??) that in the first regime $H_{\rm min} \le 2\theta \le \hmax$, then one equivalently has the simplest expression
% %
% \begin{align}\label{rankonespherical_Rtrans}
%  \phi_\rho(\theta) =\frac12 \int_0^{2\theta} R_\rho(x)dx.
% \end{align}

% Denote by $\bA$ a generic $N\times N$ rank-$k$ symmetric matrix with non-zero eigenvalues $(a_{N,i})_{i\le k}$ that are bounded uniformly in $N$. Let $a_i:=\lim_{N\to+\infty}a_{N,i}$. It is known that if $k$ is fixed then
% %
% \begin{align}
% \phi^{(k)}_N((a_{N,i}),(\Sigma_i)):=\frac1N\ln\int \mu_N(d\bO)  \exp N\tr\big[ \bO\bSig\bO^\intercal  \bA \big]   =\sum_{i\le k} \phi_\rho(a_i)+o_N(1).
% \end{align}
% Now letting $\bA:=N^{-1}\sum_{\ell \le k} \bx^\ell(\bx^\ell)^\intercal$, which indeed has $\mathcal{O}(1)$ eigenvalues. For convenience, let also
% %
% \begin{align}
% \phi^{\lambda}_\rho(x):=\phi_\rho\Big(\sqrt\frac\lambda 4 x\Big).
% \end{align}
% It implies that if the overlap matrix has the $1$RSB structure then  
% %
% \begin{align*}
%  &\phi^{(k)}_N\Big(\sqrt\frac{\lambda}{4}(a_{N,i}),(\Sigma_i)\Big)= \frac1N \ln\int \mu_N(d\bO)  \exp N\tr\Big[\sqrt\frac{\lambda}{4} \bO\bSig\bO^\intercal \frac1N\sum_{\ell \le k} \bx^\ell(\bx^\ell)^\intercal \Big]\\
%  &\qquad= \frac{k(t-1)}{t}\phi^{\lambda}_\rho(v-q_1)+\Big(\frac{k}{t}-1\Big)\phi^{\lambda}_\rho(v-(1-t)q_1-tq_0)+\phi^{\lambda}_\rho(v-(1-t)q_1-(t-k)q_0)+o_N(1).
% \end{align*}

% We now introduce delta functions in order to later enforce the $1$RSB structure for the overlap; these will introduce entropic contributions. Let us identify the ground-truth signal with the $0$th replica $\bX=\bx^0$. We also want to enforce the following constraint $\bx^\ell\cdot\bX/N = m_\ell$ for all replicas. We thus re-write the moment of the partition function as
% %
% \begin{align}
%         \E Z_N^k & =  \int\Big(\prod_{\ell\le k} P_x(d\bx^\ell)\Big)\,P_X(d\bX)\,  d\bq d\bmm\, \Big(\prod_{\ell\le \ell'\le k}\delta(\bx^\ell\cdot\bx^{\ell'}-Nq_{\ell\ell'})\Big)\prod_{\ell\le k}\delta(\bx^\ell\cdot\bX-Nm_\ell) \nonumber \\
%         &\qquad\qquad\times \exp\sum_{\ell \le k}\Big(\frac{N\lambda}{2}m_\ell^2 -\frac{N\lambda}{4}q_{\ell\ell}^2\Big)\int \mu_N(d\bO)  \exp N\tr\Big[\sqrt\frac{\lambda}{4} \bO\bSig\bO^\intercal \frac1N\sum_{\ell \le k} \bx^\ell(\bx^\ell)^\intercal \Big].
% \end{align}
% Introducing the Fourier representation of the delta function $1=\int \delta(x-q)dq\propto \int \exp{\rm i}\hat q(x-q)  dqd\hat q$ we get
% %
% \begin{align*}
% &\E Z_N^k  
% % & = \int\Big(\prod_{\ell\le k} P_x(d\bx^\ell)\Big)\,P_X(d\bX)\, \exp\sum_{\ell \le k}\Big(\frac{\lambda}{2N}(\bX\cdot \bx^\ell)^2 -\frac{\lambda}{4N}\|\bx^\ell\|^4\Big) \nonumber \\
% % %
% % &\qquad\times \int d\bq d\hat \bq \exp{\rm i}\sum_{\ell\le \ell'\le k}\Big(\hat q_{\ell\ell'} \bx^\ell\cdot\bx^{\ell'}-N\hat q_{\ell\ell'}q_{\ell\ell'}\Big) \int \mu_N(d\bO)  \exp\tr\Big[\sqrt\frac{\lambda}{4N} \bO\bSig\bO^\intercal \sum_{\ell \le k} \bx^\ell(\bx^\ell)^\intercal \Big]\\
% % %
% % %
% \propto  \int d\bq d\hat \bq d\bmm d\hat \bmm \exp N\Big(-{\rm i}  \sum_{\ell\le \ell'\le k} \hat q_{\ell\ell'}q_{\ell\ell'}-{\rm i} \sum_{\ell\le k} \hat m_\ell m_\ell+\frac{ \lambda}{2}\sum_{\ell \le k}m_\ell^2 -\frac{\lambda}{4}\sum_{\ell \le k} q_{\ell\ell}^2\Big) \\
% &\times \int\Big(\prod_{\ell\le k} P_x(d\bx^\ell)\Big)\,P_X(d\bX)\exp \Big(N \phi^{(k)}_N\Big(\sqrt\frac{\lambda}{4}(a_{N,i}),(\Sigma_i)\Big)+{\rm i}\sum_{\ell\le \ell'\le k}\hat q_{\ell\ell'} \,\bx^\ell\cdot \bx^{\ell'}+{\rm i}\sum_{\ell\le k}\hat m_{\ell}\, \bx^\ell\cdot \bX\Big)\Big.  
% \end{align*}
% Now we restrict the integral over $\bq$ and $\hat \bq$ to matrices having the $1$RSB structure given by \eqref{1RSBansatz}, which in turns implies the $1$RSB structure for the overlap too due to the delta functions. We also restrict the integrals over $\bmm$ and $\hat\bmm$ to vectors of the following form:
% \begin{align}
% \begin{cases}
% m_\ell = m_1 \ &\mbox{if} \ 1\le \ell \le t,\\
% m_\ell = m_0 \ &\mbox{if} \ t+1\le \ell\le k,
% \end{cases}
% \end{align} 
% and similarly for $\hat \bmm$. This formalizes the idea that in the $1$RSB picture where clusters of solutions appear, there is one ``special'' cluster (the first in this case) which contains the ground-trough signal $\bX$, and the replicas in it have a higher overlap $m_1$ with  while the replicas in the other clusters have an overlap $m_0$ with it. \magenta{At the moment the computation assumes that the first cluster is of same size as the others; I wonder if this should be relaxed by allowing it to be of different size. This could actually be interesting in order to understand whether this cluster has a different size, in the 1RSB clustered phase, as the SNR varies.}


% Let $d\btau:=dq_0 dq_1 dv dm_0dm_1 d\hat q_0 d\hat q_1 d\hat v  d\hat m_0d\hat m_1$. We absorb the imaginary $\rm i=\sqrt{-1}$ in the hat-variables by integrating them over the imaginary axis. We reach that at leading exponential order the replicated partition function is
% \begin{align*}
% \E Z_N^k  & =  \int d\btau \exp N \Big\{- k v\hat v - \frac k2 (t-1) q_1\hat q_1-\frac12\big(k(k-1)-k(t-1)\big)q_0\hat q_0 - t m_1\hat m_1-(k-t)m_0\hat m_0  \\
% &\qquad+\frac{ \lambda}{2}\big(t m_1^2+(k-t)m_0^2\big) -\frac{k \lambda}{4}v^2\\
% &\qquad+\frac{k(t-1)}{t}\phi^\lambda_\rho(v-q_1)+\Big(\frac{k}{t}-1\Big)\phi^\lambda_\rho(v-(1-t)q_1-tq_0)+\phi^\lambda_\rho(v-(1-t)q_1-(t-k)q_0)\\
% &\qquad+\ln\int\Big(\prod_{\ell\le k} P_x(dx^\ell)\Big)\,P_X(dX)\exp  \Big(\sum_{\ell\le  \ell'\le k}\hat q_{\ell\ell'} x^\ell x^{\ell'}+\hat m_1 \sum_{\ell\le t} x^\ell X+\hat m_0 \sum_{\ell\ge t+1} x^\ell X\Big)\Big\}
% \end{align*}
% where we used the decoupled nature of the priors to factorize the last integral over the variables index $i$. We now need to decouple replicas using gaussian integrals. Denote $(\ell^j_i)_{i\le t}$ the replica indices of replicas in group $j\in[k/t]$. Under the $1$RSB structure we have
% \begin{align}
%  \sum_{\ell\le  \ell'\le k}\hat q_{\ell\ell'} x^\ell x^{\ell'}  =\Big(\hat v -\frac{\hat q_1}2\Big)\sum_{\ell\le k}(x^\ell)^2+ \frac{\hat q_0}2\Big(\sum_{\ell\le k} x^\ell \Big)^2+\frac{\hat q_1-\hat q_0}2\sum_{j\le k/t}\Big(\sum_{i\le t}x^{\ell^j_i}\Big)^2.\label{beforeHS}
% \end{align}
% The gaussian integral 
% %
% \begin{align}
%   \sqrt\frac a\pi \int dz \exp(-az^2+bz)=\exp\frac{b^2}{4a}  
% \end{align}
% allows us to decouple the replicas as follows:
% \begin{align*}
%  &\exp \sum_{\ell\le  \ell'\le k}\hat q_{\ell\ell'} x^\ell x^{\ell'}\\
%  &\propto {\frac{1}{\sqrt {\hat q_0(\hat q_1-\hat q_0)^{k/t}}}}\int d\bz \exp\Big(\Big(\hat v -\frac{\hat q_1}2\Big)\sum_{\ell\le k}(x^\ell)^2-\frac{z_0^2}{2\hat q_0}+ z_0\sum_{\ell\le k}x^\ell +  \sum_{j\le k/t}\Big(-\frac{z_j^2}{2(\hat q_1-\hat q_0)}+z_j\sum_{i\le t}x^{\ell^j_i}\Big)\Big).
% \end{align*}
% Thus we reach that at leading exponential order and under a $1$RSB ansatz,
% %
% \begin{align}
%  \E Z_N^k    \propto  \int d\btau \exp N S(k,t,\btau)
% \end{align}
% where the effective action is (here $\btau:=(q_0, q_1, v, m_0, m_1, \hat q_0, \hat q_1, \hat v,  \hat m_0, \hat m_1)$)
% %
% \begin{align}
%  S(k,t,\btau)&:=- k v\hat v - \frac k2 (t-1) q_1\hat q_1-\frac12(k^2-kt)q_0\hat q_0 -t m_1\hat m_1-(k-t)m_0\hat m_0 \nn
%  &\qquad+\frac{ \lambda}{2}\big(t m_1^2+(k-t)m_0^2\big) -\frac{k \lambda}{4}v^2+\frac{k(t-1)}{t}\phi_\rho^\lambda(v-q_1)\nn
% &\qquad+\Big(\frac{k}{t}-1\Big)\phi^\lambda_\rho(v-(1-t)q_1-tq_0)+\phi^\lambda_\rho(v-(1-t)q_1-(t-k)q_0)\nn
% &\qquad-\frac12\ln \Big(\hat q_0(\hat q_1-\hat q_0)^{k/t}\Big)+\ln\int P_X(dX)\,d\bz\,\Big(\prod_{\ell\le k} P_x(dx^\ell)\Big) \exp \Big(\Big(\hat v -\frac{\hat q_1}2\Big)\sum_{\ell\le k}(x^\ell)^2 \nn
% &\qquad-\frac{z_0^2}{2\hat q_0}+ z_0\sum_{\ell\le k}x^\ell+  \sum_{j\le k/t}\Big(-\frac{z_j^2}{2(\hat q_1-\hat q_0)}+z_j\sum_{i\le t}x^{\ell^j_i}\Big)+\hat m_1 \sum_{\ell\le t} x^\ell X+\hat m_0 \sum_{\ell\ge t+1} x^\ell X\Big).\label{1RSBaction}
% \end{align}
% A saddle-point estimate of the integral over $\btau$ as $N\to+\infty$ combined with the replica trick implies
% \begin{align}
% \lim_{N\to+\infty} \frac1N\EE\ln Z_N=\lim_{k\to 0_+}\lim_{N\to+\infty} \frac{d}{dk}\frac1N\ln \EE Z_N^k=  \lim_{k\to 0_+}\lim_{N\to+\infty} \frac{d}{dk}S(k,t,\btau^*)
% \end{align}
% where $\btau^*$ is the saddle point (i.e., the critical point of $S$) that maximizes the log-partition function \magenta{Explain more here}. We have, at a critical point $\btau=\btau^*$,
% %
% \begin{align*}
%   \lim_{k\to0_+}\frac{d}{dk}S(k,t,\btau) &= - v\hat v - \frac 12 (t-1) q_1\hat q_1+\frac t2q_0\hat q_0 - m_0\hat m_0 +\frac{ \lambda}{2}m_0^2 -\frac{\lambda}{4}v^2-\frac1{2t}\ln (\hat q_1-\hat q_0)\\
% &\qquad+\frac{t-1}{t}\phi^\lambda_\rho(v-q_1)+\frac{1}{t}\phi^\lambda_\rho(v-(1-t)q_1-tq_0)+\sqrt\frac\lambda 4q_0\phi^{\lambda \prime}_\rho(v-(1-t)q_1-tq_0)\\
% &\qquad+\lim_{k\to0_+}\frac{d}{dk}\ln\int d\bz\, P_X(dX)\,\Big(\prod_{\ell\le k} P_x(dx^\ell)\Big) \exp \Big(\Big(\hat v -\frac{\hat q_1}2\Big)\sum_{\ell\le k}(x^\ell)^2 \\
% &\qquad-\frac{z_0^2}{2\hat q_0}+ z_0\sum_{\ell\le k}x^\ell+  \sum_{j\le k/t}\Big(-\frac{z_j^2}{2(\hat q_1-\hat q_0)}+z_j\sum_{i\le t}x^{\ell^j_i}\Big)+\hat m_1 \sum_{\ell\le t} x^\ell X+\hat m_0 \sum_{\ell\ge t+1} x^\ell X\Big).
% \end{align*}
% Here $\phi_\rho^{\lambda\prime}(x):=\partial_x \phi^\lambda_\rho(x)$. We denote by $J$ the integral appearing above. Let us manipulate it in order to then simplify it in the limit $k\to 0_+$, first by isolating the contribution of the first special cluster where the signal lies. It is equal to
% \begin{align*}
%   J&=\int dz_0 \exp \Big(-\frac{z_0^2}{2\hat q_0}\Big) P_X(dX) \int \prod_{j\le k/t} \exp\Big( -\frac{z_j^2}{2(\hat q_1-\hat q_0)}\Big)  \Big(\prod_{\ell\le k} P_x(dx^\ell)\Big) \\
%   &\qquad \times \exp \sum_{\ell\le t} \Big(\Big(\hat v -\frac{\hat q_1}2\Big)(x^\ell)^2+ (z_0+z_1+\hat m_1  X)x^\ell\Big)\exp\sum_{j=2}^{k/t}\sum_{i\le t}\Big(\Big(\hat v -\frac{\hat q_1}2\Big)(x^{\ell^j_i})^2+(z_0+z_j+\hat m_0  X)x^{\ell^j_i} \Big)  \\
%   %
%   &= \int dz \exp \Big(-\frac{z^2}{2\hat q_0}\Big) P_X(dX) \\
%   &\qquad\times \int \exp\Big( -\frac{\xi^2}{2(\hat q_1-\hat q_0)}\Big) \Big[\int P_x(dx)  \exp  \Big(\Big(\hat v -\frac{\hat q_1}2\Big)x^2+ (z+\xi+\hat m_1  X)x\Big)\Big]^t\\
%   %
%   &\qquad\qquad \times  \Big(\int\exp\Big( -\frac{\xi^2}{2(\hat q_1-\hat q_0)}\Big)  \Big[\int P_x(dx)   \exp\Big(\Big(\hat v -\frac{\hat q_1}2\Big)x^2+(z+\xi+\hat m_0  X)x \Big)\Big]^t\Big)^{k/t-1}.
% \end{align*}
% This integral is of the form 
% %
% \begin{align*}
%   J&=\EE_{X,z}\Big(\EE_{\xi} f_1^t(X,z,\xi) (\EE_{\xi} f_0^t(X,z,\xi))^{k/t-1}\Big)=\EE_{X,z}\Big(\frac{\EE_{\xi} f_1^t(X,z,\xi)}{\EE_{\xi} f_0^t(X,z,\xi)} \exp\Big(\frac kt\ln \EE_{\xi} f_0^t(X,z,\xi)\Big)\Big)\\
%   &=\EE_{X,z}\Big(\frac{\EE_{\xi} f_1^t(X,z,\xi)}{\EE_{\xi} f_0^t(X,z,\xi)} \Big(1+\frac kt\ln \EE_{\xi} f_0^t(X,z,\xi)+O(k^2)\Big) \Big),
% \end{align*}
% where, for $i=0,1$ we have
% \begin{align}\label{fi}
%    f_i^t(X,z,\xi,\hat v,\hat q_1,\hat m_i)=f_i^t(X,z,\xi)&:=  \Big[\int P_x(dx)  \exp  \Big(\Big(\hat v -\frac{\hat q_1}2\Big)x^2+ (z+\xi+\hat m_i  X)x\Big)\Big]^t.
% \end{align}
% Therefore
% \begin{align*}
%   \frac d {dk}  \ln J &=   \frac d {dk}  \ln \EE_{X,z}\Big(\frac{\EE_{\xi} f_1^t(X,z,\xi)}{\EE_{\xi} f_0^t(X,z,\xi)} \Big(1+\frac kt\ln \EE_{\xi} f_0^t(X,z,\xi)\Big)+O(k^2) \Big)\\
%   &=\frac 1t\frac{\EE_{X,z}\Big(\frac{\EE_{\xi} f_1^t(X,z,\xi)}{\EE_{\xi} f_0^t(X,z,\xi)} \ln \EE_{\xi} f_0^t(X,z,\xi) +O(k) \Big)}{\EE_{X,z}\Big(\frac{\EE_{\xi} f_1^t(X,z,\xi)}{\EE_{\xi} f_0^t(X,z,\xi)} \big(1+\frac kt\ln \EE_{\xi} f_0^t(X,z,\xi)\big) +O(k^2)\Big)}\\
%   &\xrightarrow{k\to 0_+} \frac 1t{\EE_{X,z}\Big(\frac{\EE_{\xi} f_1^t(X,z,\xi)}{\EE_{\xi} f_0^t(X,z,\xi)} \ln \EE_{\xi} f_0^t(X,z,\xi) \Big)}\Big(\EE_{X,z}\frac{\EE_{\xi} f_1^t(X,z,\xi)}{\EE_{\xi} f_0^t(X,z,\xi)} \Big)^{-1}.
% \end{align*}
% Combining everything we finally obtain the following replica prediction at the $1$RSB level:

% \begin{prediction}[One-step replica symmetry breaking prediction] \label{1RSBpred}
% The free energy is given, at the 1RSB level of the replica theory, by the following expression:
% %
% \begin{align*}
%   \lim_{N\to+\infty} f_N &= \sup_{(t,\btau)\in \mathcal{C}^{\rm 1RSB}}f^{\rm 1RSB}(\lambda,t,\btau),
% \end{align*}
% where recall $\btau:=(q_0, q_1, v, m_0, m_1, \hat q_0, \hat q_1, \hat v,  \hat m_0, \hat m_1)$ and $\mathcal{C}^{\rm 1RSB}$ is the set of critical points of the following 1RSB replica potential:
% \begin{align*}
% &f^{\rm 1RSB}(\lambda,t,\btau):=- v\hat v - \frac 12 (t-1) q_1\hat q_1+\frac t2q_0\hat q_0 - m_0\hat m_0 +\frac{ \lambda}{2}m_0^2 -\frac{\lambda}{4}v^2-\frac1{2t}\ln (\hat q_1-\hat q_0)\nonumber \\
% &+\frac{t-1}{t}\phi_\rho\Big(\sqrt\frac\lambda 4(v-q_1)\Big)+\frac{1}{t}\phi_\rho\Big(\sqrt\frac\lambda 4(v-(1-t)q_1-tq_0)\Big)+\sqrt\frac\lambda 4q_0\phi_\rho'\Big(\sqrt\frac\lambda 4(v-(1-t)q_1-tq_0)\Big)\nonumber \\
% &+\frac 1t{\EE_{X,z}\Big(\frac{\EE_{\xi} f_1^t(X,z\sqrt{\hat q_0},\xi\sqrt{\hat q_1-\hat q_0},\hat v,\hat q_1,\hat m_1)}{\EE_{\xi} f_0^t(X,z\sqrt{\hat q_0},\xi\sqrt{\hat q_1-\hat q_0},\hat v,\hat q_1,\hat m_0)} \ln \EE_{\xi} f_0^t(X,z\sqrt{\hat q_0},\xi\sqrt{\hat q_1-\hat q_0},\hat v,\hat q_1,\hat m_0) \Big)}\\
% &\qquad\times\Big(\EE_{X,z}\frac{\EE_{\xi} f_1^t(X,z\sqrt{\hat q_0},\xi\sqrt{\hat q_1-\hat q_0},\hat v,\hat q_1,\hat m_1)}{\EE_{\xi} f_0^t(X,z\sqrt{\hat q_0},\xi\sqrt{\hat q_1-\hat q_0},\hat v,\hat q_1,\hat m_0)} \Big)^{-1} 
% \end{align*}
% with definitions \eqref{fi} and \eqref{rankonespherical}, $\rho$ is the asymptotic density of eigenvalues $\bSig$ of the noise \eqref{Z_eigen}, $\xi$ and $z\sim \mathcal{N}(0,1)$ independently and $X\sim P_X$.
% %
% \end{prediction}

\subsubsection{Replica symmetric free energy}

We can deduce the replica symmetric prediction by starting over the computation from \manunote{Here we have a reference (eqref\{beforeHS\}) to an equation that is commented} and taking $q_0=q_1=q$, $\hat q_0=\hat q_1=\hat q$, $m_0=m_1=m$, $\hat m_0=\hat m_1=\hat m$ and $t=k$:
%
\begin{align}\label{beforeHS_RS}
 \sum_{\ell\le  \ell'\le k}\hat q_{\ell\ell'} x^\ell x^{\ell'}  =\Big(\hat v -\frac{\hat q}2\Big)\sum_{\ell\le k}(x^\ell)^2+ \frac{\hat q}2\Big(\sum_{\ell\le k} x^\ell \Big)^2,
\end{align}
%
and thus
\begin{align*}
 &\exp \sum_{\ell\le  \ell'\le k}\hat q_{\ell\ell'} x^\ell x^{\ell'}\propto {\frac{1}{\sqrt {\hat q}}}\int dz \exp\Big(\Big(\hat v -\frac{\hat q}2\Big)\sum_{\ell\le k}(x^\ell)^2-\frac{z^2}{2\hat q}+ z\sum_{\ell\le k}x^\ell \Big).
\end{align*}
Let $\bsig:=(q, v, m, \hat q, \hat v,  \hat m)$. The RS action becomes
%
\begin{align}
 S(k,\bsig)&:=- k v\hat v - \frac k2 (k-1) q\hat q -k m\hat m +\frac{ \lambda}{2}k m^2 -\frac{k \lambda}{4}v^2+(k-1)\phi_\rho^\lambda(v-q)+\phi_\rho^\lambda(v-(1-k)q)\nn
&\qquad-\frac12\ln \hat q+\ln\int P_X(dX)\,dz\exp\Big(-\frac{z^2}{2\hat q}\Big)\,\Big[\int P_x(dx) \exp \Big(\Big(\hat v -\frac{\hat q}2\Big)x^2 + zx+\hat m  x X\Big)\Big]^k.\label{RSaction}
\end{align}
Taking its $k$-derivative and the limit $k\to0_+$ yields
\begin{align}
\lim_{k\to 0_+}\frac d {dk}S(k,\bsig)&:=- v\hat v + \frac 12 q\hat q - m\hat m +\frac{ \lambda}{2} m^2 -\frac{\lambda}{4}v^2+\phi^\lambda_\rho(v-q)+\sqrt\frac\lambda 4q\phi_\rho^{\lambda \prime}(v-q)\nn
&\quad\quad +\int P_X(dX)\,dz\exp\Big(-\frac{z^2}{2\hat q}\Big) \ln\int P_x(dx) \exp \Big(\Big(\hat v -\frac{\hat q}2\Big)x^2 + zx+\hat m  x X\Big),\label{1RSBaction}
\end{align}
using $\partial_k \ln\EE U^k\to \EE\ln U$ as $k\to 0_+$. 

%
\begin{prediction}[Replica symmetric prediction] \label{RSpred}
The free energy is given, at the RS level of the replica theory, by the following expression:
%
\begin{align*}
  \lim_{N\to+\infty} f_N &= \sup_{\bsig\in \mathcal{C}^{\rm RS}}f^{\rm RS}(\lambda,\bsig),
\end{align*}
where $\bsig:=(q,v, m, \hat q, \hat v,  \hat m)$ and $\mathcal{C}^{\rm RS}$ is the set of critical points of the following RS potential:
\begin{align}
f^{\rm RS}(\lambda,\bsig)&:=- v\hat v + \frac 12 q\hat q - m\hat m +\frac{ \lambda}{2} m^2 -\frac{\lambda}{4}v^2+\phi_\rho\Big(\sqrt\frac\lambda 4(v-q)\Big)+\sqrt\frac\lambda 4q\phi'_\rho\Big(\sqrt\frac\lambda 4(v-q)\Big)\nn
&\quad\quad +\EE_{X,z} \ln\int P_x(dx) \exp \Big(\Big(\hat v -\frac{\hat q}2\Big)x^2 + \sqrt{\hat q} zx+\hat m  x X\Big),
\end{align}
with definition \eqref{rankonespherical} with $\rho$ the asymptotic density of eigenvalues $\bSig$ of the noise \eqref{Z_eigen}, $z\sim \mathcal{N}(0,1)$ and $X\sim P_X$. At $\bsig=\bsig^*$ the supremum among the critical points, the physical meaning of the following quantities is
%
\begin{align}
 m^*=\lim_{N\to+\infty}\Big|\frac1N \bx\cdot\bX\Big|, \qquad q^*=\lim_{N\to+\infty}\Big|\frac1N \bx\cdot\bx'\Big|, \qquad v^*=\lim_{N\to+\infty}\frac1N \|\bx\|^2,
\end{align}
for conditionally i.i.d. replicas (i.e., samples of the posterior) $\bx,\bx'$ and ground-truth $\bX$ drawn from $P_X(d\bX)$. In particular, letting $X\sim p_X$, the asymptotic mean-square error is
%
\begin{align}
 \lim_{N\to+\infty}\frac1{N^2}\EE\|\bX\bX^\intercal -\EE[\bx\bx^\intercal \mid \bY ]\|^2_{\rm F}  =  (\EE X^2)^2-2(m^*)^2+(q^*)^2.
\end{align}
\end{prediction}

\subsubsection{Fixed point equations}

Let the ``decoupled quenched Gibbs mean'' be defined as
%
\begin{align}
\EE\langle f(x)\rangle_{\rm d}:= \E_{X,z}\frac{\int  P_x(dx) \exp \big((\hat v -\frac{\hat q}2)x^2 + \sqrt{\hat q} zx+\hat m  x X\big) f(x)  }{\int  P_x(dx) \exp \big((\hat v -\frac{\hat q}2)x^2 + \sqrt{\hat q} zx+\hat m  x X\big) }.\label{decoupGibbs}
\end{align}
The critical points of this RS potential verify (we indicate on the left w.r.t. what variable we took a partial derivative of the potential)
%
\begin{align*}
(v) \qquad &\hat v =-\frac\lambda2 v + \frac{\sqrt\lambda}2\phi'_\rho\Big(\frac{\sqrt\lambda}2(v-q)\Big)+\frac\lambda4 q \phi''_\rho\Big(\frac{\sqrt\lambda}2(v-q)\Big)\\
(q) \qquad &\hat q =\frac{\lambda}2 q \phi''_\rho\Big(\frac{\sqrt\lambda}2(v-q)\Big)\\
(m) \qquad &\hat m =\lambda m\\
(\hat v) \qquad &v =\EE \langle x^2\rangle_{\rm d}\\
(\hat q) \qquad & q=\EE \langle x^2-\hat q^{-1/2} zx\rangle_{\rm d}=\EE \langle x\rangle_{\rm d}^2\\
(\hat m) \qquad &m =\EE \langle X x\rangle_{\rm d}
\end{align*}
where we used the gaussian integration by part formula $\E zf(z)=\E f'(z)$, $z\sim\mathcal{N}(0,1)$, in order to simplify the $(\hat q)$ equation. 
In particular we have 
$$ \hat v -\frac{\hat q}2=\frac{\sqrt\lambda}2\phi'_\rho\Big(\frac{\sqrt\lambda}2(v-q)\Big)-\frac\lambda2 v .$$
Let $\hat \delta:=\hat v -\hat q/2$. An iteration scheme to find a fixed point is as follows. Initialise $(q^0=(\EE_{P_x} x)^2,v^0= \EE_{P_x}(x^2),m^0=\varepsilon\ll 1)$. Then for $\tau\ge 0$ iterate
%
\begin{align*}
&\hat \delta^{\tau+1}  =\frac{\sqrt\lambda}2\phi'_\rho\Big(\frac{\sqrt\lambda}2(v^{\tau}-q^{\tau}) \Big)-\frac\lambda2 v^\tau, \\
&\hat q^{\tau+1} =\frac{\lambda}2 q^\tau \phi''_\rho\Big(\frac{\sqrt\lambda}2(v^{\tau}-q^{\tau})\Big),\\
&\hat m^{\tau+1}=\lambda m^\tau,\\
&q^{\tau+1} =\EE \langle x\rangle_{\rm d}^2(\hat \delta^{\tau +1},\hat q^{\tau+1},\hat m^{\tau+1}),\\
&v^{\tau+1} =\EE \langle x^2\rangle_{\rm d}(\hat \delta^{\tau +1},\hat q^{\tau+1},\hat m^{\tau+1}),\\
&m^{\tau+1} =\EE \langle X x\rangle_{\rm d}(\hat \delta^{\tau +1},\hat q^{\tau+1},\hat m^{\tau+1})
\end{align*}
where
\begin{align}
\EE\langle f(x)\rangle_{\rm d}(\hat \delta,\hat q,\hat m):= \E_{X,z}\frac{\int  P_x(dx) \exp \big(\hat \delta x^2 + \sqrt{\hat q} zx+\hat m  x X\big) f(x)  }{\int  P_x(dx) \exp \big(\hat \delta x^2 + \sqrt{\hat q} zx+\hat m  x X\big) }.
\end{align}
The MSE can thus be tracked as $${\rm MSE}^{\tau}=(\EE X^2)^2-2(m^\tau)^2+(q^\tau)^2,$$ still with $X~\sim P_X$. This corresponds to the state evolution recursion of the gaussian approximate message-passing algorithm wrongly used for a spiked Wigner model with structured (i.e., non-Wigner) noise.

% These allow to implify the RS formula to
% %
% \begin{align}
%  \lim_{N\to+\infty} f_N &= \sup_{(v,q,m)\in \mathcal{C}^{\rm RS}}\Big\{ \frac\lambda4 (v^2- 2 m^2)+\phi_\rho(v-q) - (v-q)\phi'_\rho(v-q)-q(v-q) \phi''_\rho(v-q)  \nn
% &\quad\quad +\EE_{X,z} \ln\int P_x(dx) \exp \Big(\Big(\phi'_\rho(v-q)-\frac\lambda2 v\Big)x^2 + \sqrt{2 q \phi''_\rho(v-q)} zx+\lambda m  x X\Big)\Big\}.
% \end{align}
% Let us re-define the quenched decoupled Gibbs mean:
% \begin{align*}
% \EE\langle f(x)\rangle_{\rm d}:= \E_{X,z}\frac{\int  P_x(dx) \exp \big((\phi'_\rho(v-q)-\frac\lambda2 v)x^2 + \sqrt{2 q \phi''_\rho(v-q)} zx+\lambda m  x X\big) f(x)  }{\int  P_x(dx) \exp \big((\phi'_\rho(v-q)-\frac\lambda2 v)x^2 + \sqrt{2 q \phi''_\rho(v-q)} zx+\lambda m  x X\big) }.
% \end{align*}
% With this new definition the critical conditions for the simplified RS potential become
% %
% \begin{align*}
% (v) \qquad &\frac \lambda2 v=(v+q)\phi''_\rho(v-q)+q(v-q)\phi'''_\rho(v-q)+\Big(\frac\lambda2-\phi''_\rho(v-q)+q\phi'''_\rho(v-q)\Big) \EE \langle x^2\rangle_{\rm d}\\
% &\qquad\qquad\qquad\qquad-q\phi'''_\rho(v-q) \EE \langle x\rangle_{\rm d}^2\\
% (q) \qquad &q = q(q-v)\frac{\phi'''_\rho(v-q)}{\phi''_\rho(v-q)}+q\frac{\phi'''_\rho(v-q)}{\phi''_\rho(v-q)}\EE\langle x^2\rangle_{\rm d}+\EE\langle x\rangle_{\rm d}^2\Big(1-q\frac{\phi'''_\rho(v-q)}{\phi''_\rho(v-q)}\Big) \\
% (m)\qquad &m =\EE \langle X x\rangle_{\rm d}
% \end{align*}
% using the gaussian integration by part formula $\EE\langle zx\rangle_{\rm d}=\sqrt{2q\phi''_\rho(v-q)}(\EE \langle x^2\rangle_{\rm d}-\EE \langle x\rangle_{\rm d}^2)$.

\subsubsection{Applications}

\emph{Rademacher prior}\ \ As a base case let us start by considering that the prior is known and Rademacher $p_X=p_x=\frac12(\delta_{-1}+\delta_1)$ or gaussian $p_X=p_x=\mathcal{N}(0,1)$. In these simple cases we straightforwardly obtain the three following functions:
%
\begin{align}
\mbox{Known Rademacher prior:}\ 
\begin{cases}
&\EE \langle x\rangle_{\rm d}^2(\hat q,\hat m)=\EE \tanh^2(\hat m + \sqrt{\hat q}z),\\
&\EE \langle x^2\rangle_{\rm d}=1,\\
&\EE \langle X x\rangle_{\rm d}(\hat q,\hat m)=\EE \tanh(\hat m + \sqrt{\hat q}z).
\end{cases}
\end{align}
or in the gaussian case,
\begin{align}
\mbox{Known gaussian prior:}\ 
\begin{cases}\label{31}
&\EE \langle x\rangle_{\rm d}^2(\hat \delta,\hat q,\hat m)=\frac{\hat m^2+\hat q}{(1-2\hat \delta)^2},\\
&\EE \langle x^2\rangle_{\rm d}(\hat \delta,\hat q,\hat m)=\frac{1+\hat m^2+\hat q-2\hat \delta }{(1-2\hat \delta )^2},\\
&\EE \langle X x\rangle_{\rm d}(\hat \delta,\hat q,\hat m)=\frac{\hat m}{1-2\hat \delta}.
\end{cases}
\end{align}

Let us assume for a moment that in formulas \eqref{rankonespherical} and \eqref{funcg_sphInt} we are always in the regime $H_{\rm min} \le 2\theta \le \hmax$. This will anyway be the case when taking a convex combination of Diracs for $\rho$.

Before considering mismatched settings, as a sanity check we verify that we recover the known results in the Bayes-optimal case where the noise is truly Wigner as assumed by the statistician, so the data is $\bY_W$. In this case, using $$\phi_\rho'(\theta) =R_\rho(2\theta), \qquad \phi_\rho''(\theta) =2R_\rho'(2\theta),$$ the following functions read
%
\begin{align}
\mbox{Semicircle law of radius $2$ (standard Wigner noise):}\ 
\begin{cases}
&\phi'_\rho(\theta) = 2\theta,\\
&\phi''_\rho(\theta) =2.
\end{cases}
\end{align}
Therefore the recursion becomes simply:
\begin{align*}
\begin{cases}
&q^{\tau+1} =\EE \tanh^2(\lambda m^\tau + \sqrt{\lambda q^\tau}z),\\
&m^{\tau+1} =\EE \tanh(\lambda m^\tau + \sqrt{\lambda q^\tau}z).
\end{cases}
\end{align*}

Let $t\in (0,1)$. If instead we consider $$\rho=t\delta_{-\sqrt{1/t-1}}+(1-t)\delta_{\frac{1}{\sqrt{1/t-1}}}$$ so that it satisfies $\EE_\rho \lambda=0$ and $\EE_\rho \lambda^2=1$, then the functions are 
%
\begin{align}
\mbox{Two Diracs:}\ 
\begin{cases}
&\phi'_\rho(\theta) =\frac{1}{4\theta \sqrt{t-t^2}}\Big(4\theta t-2\theta-\sqrt{t-t^2}+\sqrt{t+4\theta\sqrt{t-t^2}+4\theta^2-t^2(1+8\theta\sqrt{1/t-1})}\Big),\\
&\phi''_\rho(\theta) =\Big(4\theta^2\sqrt{t+4\theta t\sqrt{1/t-1} +4\theta^2-t^2(1+8\theta\sqrt{1/t-1})}\Big)^{-1}\\
& \qquad \times\Big(-\sqrt{t-t^2}-2\theta+4\theta t+\sqrt{t+4\theta\sqrt{t-t^2}+4\theta^2-t^2(1+8\theta\sqrt{1/t-1})}\Big).
\end{cases}
\end{align}
In the special case of $t=1/2$ it becomes
%
\begin{align}\label{34}
\mbox{Two Diracs:}\ 
\begin{cases}
&\phi'_\rho(\theta) =\frac{1}{4\theta}\big(\sqrt{1+16\theta^2}-1\big),\\
&\phi''_\rho(\theta) =\frac{1}{4\theta^2}\big(1-1/\sqrt{1+16\theta^2}\big).
\end{cases}
\end{align}
Therefore the recursion becomes simply, in the case of Rademacher prior,
\begin{align*}
\begin{cases}
&\hat q^{\tau+1} =\frac{\lambda}2 q^\tau \phi''_\rho(\frac{\sqrt\lambda}2(1-q^{\tau})),\\
&q^{\tau+1} =\EE \tanh^2(\lambda m^\tau + \sqrt{\hat q^{\tau+1}}z),\\
&m^{\tau+1} =\EE \tanh(\lambda m^\tau + \sqrt{\hat q^{\tau+1}}z),
\end{cases}
\end{align*}
with the above functions. Or in the gaussian prior case,
\begin{align*}
\begin{cases}
&\hat \delta^{\tau+1}  =\frac{\sqrt\lambda}2\phi'_\rho(\frac{\sqrt\lambda}2(v^{\tau}-q^{\tau}) )-\frac\lambda2 v^\tau, \\
&\hat q^{\tau+1} =\frac{\lambda}2 q^\tau \phi''_\rho(\frac{\sqrt\lambda}2(v^{\tau}-q^{\tau})),\\
&q^{\tau+1} =\EE \langle x\rangle_{\rm d}^2(\hat \delta^{\tau +1},\hat q^{\tau+1},\lambda m^\tau),\\
&v^{\tau+1} =\EE \langle x^2\rangle_{\rm d}(\hat \delta^{\tau +1},\hat q^{\tau+1},\lambda m^\tau),\\
&m^{\tau+1} =\EE \langle X x\rangle_{\rm d}(\hat \delta^{\tau +1},\hat q^{\tau+1},\lambda m^\tau),
\end{cases}
\end{align*}
with \eqref{31} and \eqref{34}.

% In order to compute the eigenvalues $(a_j)$ under the constraint that the overlap matrix has the above 1RSB structure, consider $(\bx^\ell)_{\ell \le k}$ with $\|\bx^\ell\|^2=Nv$. Let $(\boldsymbol{e}_j)_{j\le N}$ be an arbitrary orthonormal basis of $\mathbb{R}^N$ that we may take as the standard basis. After applying the same partitioning in distinct groups to this basis as for the replicas, let $\bsig(i,j)$ with $(i,j)\in[t]\times[k/t]$ be the $i$th member of the $j$th group, so $\bsig(i,j):=\boldsymbol{e}_{i+tj}$. Then we may write $$\bx^{i+t(j-1)}=\sqrt{CN}\Big(\bsig(i,j)+\sqrt{A}\sum_{i'(\neq i)}^t\bsig(i',j) +\sqrt{B} \sum_{j'(\neq j)}^{k/t} \bsig(i,j')\Big)$$
% where $A,B,C$ enforces the conditions of the 1RSB ansatz. For two different members of the same group $j$,
% %
% \begin{align*}
%  \frac{\bx^{i+t(j-1)}\cdot \bx^{i'+t(j-1)}}N   &=C\Big(\bsig(i,j)+\sqrt{A}\sum_{i'(\neq i)}^t\bsig(i',j) +\sqrt{B} \sum_{j'(\neq j)}^{k/t} \bsig(i,j')\Big)\\
%  &\qquad\cdot\Big(\bsig(i',j)+\sqrt{A}\sum_{i''(\neq i')}^t\bsig(i'',j) +\sqrt{B} \sum_{j'(\neq j)}^{k/t} \bsig(i',j')\Big)\\
%  &=C\big(\sqrt{A}+\sqrt A + A(t-2)\big)= q_1.
% \end{align*}
% For the same member $i$ of two different groups,
% %
% \begin{align*}
%  \frac{\bx^{i+t(j-1)}\cdot \bx^{i+t(j'-1)}}N   &=C\Big(\bsig(i,j)+\sqrt{A}\sum_{i'(\neq i)}^t\bsig(i',j) +\sqrt{B} \sum_{j'(\neq j)}^{k/t} \bsig(i,j')\Big)\\
%  &\qquad\cdot\Big(\bsig(i,j')+\sqrt{A}\sum_{i'(\neq i)}^t\bsig(i',j') +\sqrt{B} \sum_{j''(\neq j')}^{k/t} \bsig(i,j'')\Big)\\
%  &=C\big(\sqrt{B}+\sqrt{B}+B(k/t-2)\big)= q_0.
% \end{align*}
% And finally for the squared norm,
% \begin{align*}
%  \frac{\|\bx^{i+t(j-1)}\|^2}N   =C\big(1+A(t-1) +B(k/t -1)\big)=v.
% \end{align*}

% \blue{

% \subsection{Fixed point equations}

% Define the \emph{decoupled Gibbs measure} by the one-dimensional Hamiltonian with disorder $(X_*,z)$
% \begin{equation*}
%     H_d(X) := -\frac{\hat q - \hat v}{2}X^2 + \hat m X X_* + \sqrt{\hat q} X z,
% \end{equation*}
% where $X_*$ is distributed as a component of the ground-truth and $z$ is an independent standard gaussian r.v. Also, denote by $\langle \cdot \rangle_d$ the associated thermal mean. 

% Then, computing the gradient of the potential that defines $f_{mis}$ and equating it to zero gives the following set of fixed point equations
% \begin{equation}\label{eq:FPEl1}
%     v = \E\langle X^2 \rangle_d, \,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\, q = \E\langle X \rangle_d^2, \,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\, m = \E\langle X X_* \rangle_d,
% \end{equation}
% \begin{equation}\label{eq:FPEl2}
%     \hat q - \hat v =  \lambda v - \sqrt{\lambda} \Phi'\left(\sqrt{\lambda}\frac{(v-q)}{2}\right), \,\,\,\,\,\,\,\,\,\, \hat q =  \frac{\lambda q}{2} \Phi''\left(\sqrt{\lambda}\frac{(v-q)}{2}\right), \,\,\,\,\,\,\,\,\,\, \hat m = \lambda m.
% \end{equation}
% Define a new decoupled one dimensional Hamiltonian by
% \begin{equation*}
%     H_{d'}(X) := -\frac{1}{2}\left[\lambda v - \sqrt{\lambda} \Phi'\left(\sqrt{\lambda}\frac{(v-q)}{2}\right)\right] X^2 + \lambda m X X_* + \sqrt{\frac{\lambda q}{2} \Phi''\left(\sqrt{\lambda}\frac{(v-q)}{2}\right)} X z,
% \end{equation*}
% where $X_*$ and $z$ are as before. Again, let $\langle \cdot \rangle_{d'}$ be the associated thermal mean. Then, replacing \eqref{eq:FPEl2} in \eqref{eq:FPEl1} we get a closed system of $3$ equations given by
% \begin{equation}\label{eq:FPEfinal}
%     v = \E\langle X^2 \rangle_{d'}, \,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\, q = \E\langle X \rangle_{d'}^2, \,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\, m = \E\langle X X_* \rangle_{d'}.
% \end{equation}

% \subsection{Bayes-optimal case}

% In the case when the noise is really given by a Gaussian matrix we have that $\Phi(x) = x^2$. Thus,
% \begin{equation*}
%     H_{d'}(X) = -\frac{\lambda q}{2} X^2 + \lambda m X X_* + \sqrt{\lambda q} X z.
% \end{equation*}
% And also, because in this case the posterior is Bayes optimal we will have that the overlap and the magnetisation have to be equal (by Nishimori). That is, $m = q$. Therefore,
% \begin{equation*}
%     H_{d'}(X) = -\frac{\lambda q}{2} X^2 + \lambda q X X_* + \sqrt{\lambda q} X z;
% \end{equation*}
% and the only remaining fixed point equation becomes
% \begin{equation}\label{eq:FPEfinal}
%     q = \E\langle X \rangle_{d'}^2,
% \end{equation}
% which is the correct fixed point equation for the WSM in the Bayes-optimal case.
% }

==> images/sections/04Bayes.tex <==
We now present our main results, first on the performance of the mismatched Bayes estimator and whose proof will be based on large deviation theory. Then our results on the AMP algorithm (gaussian and fine-tuned) based on a state evolution analysis. 

To state our results we need some definitions. Let $\rho(\cdot)$ and $K$ be as in Hypothesis \ref{hyp:eigen} and $H_\rho : \R\backslash K \to \R$ be the Hilbert transform of the distribution $\rho(\cdot)$ defined according to
\begin{equation*}
    H_\rho(z) := \int_ K \frac{\rho(d\gamma)}{z-\gamma}. \quad \mbox{Also let} \ \ \hmax := \lim_{z\downarrow\overline{\gamma}} H_\rho(z),\ \ \hmin := \lim_{z\uparrow \underline{\gamma}} H_\rho(z)
\end{equation*}
%Define also $\hmax := \lim_{z\downarrow\overline{\gamma}} H_\rho(z)$ and $\hmin := \lim_{z\uparrow \underline{\gamma}} H_\rho(z)$ 
which exist due to the monotonicity of $H_\rho$ but may be infinite. Because $H_\rho$ is a bijection between $\R\backslash K$ and its image $(\hmin,\hmax)\backslash\{0\}$, it has some inverse 
\begin{equation*}
    K_\rho :(\hmin,\hmax)\backslash\{0\}\mapsto\R\backslash K.
\end{equation*}
We will then define the \emph{R-transform of} $\rho(\cdot)$ as the function
\begin{equation*}
    R_\rho:(\hmin,\hmax)\backslash\{0\}\mapsto\R\backslash K \quad \mbox{given by} \quad R_\rho(x) := K_\rho(x) - 1/x.
\end{equation*}
% Finally, for every $\theta > 0$ and matrix $\bA\in\R^{N\times N}$ the rank-1 spherical integral is
% \begin{equation*}
%     I_N(\theta,\bA) := \int d\mu_N(\bs) \exp\big(\theta \bs^\intercal\bA \bs\big).
% \end{equation*}
%When the arguments are clear, we will sometimes omit them and write $I_N$. 

\subsection{Mismatched Bayesian estimator}\label{sec:bayes}
% It will be useful to define a slight generalization of the model \eqref{eq:spikedmodel} with a ``Wigner regularization'' of the rotationally-invariant noise. Namely we consider the following model for the data:
% %
% \begin{align}\label{eq:spikedmodel_wigReg}
% \bY_\epsilon=\frac{\sqrt{\lambda}} {N} \bX\bX^\intercal + \bZ+\sqrt{\epsilon}\,\bW
% \end{align}
% with $\bW$ a standard Wigner matrix as before and some small $\epsilon>0$. 
% %Recall the form of the log-likelihood when assuming purely Wigner noise:
% % \begin{equation*}
% %     \mathcal{L}_N(\bx) = \frac{1}{2}\sqrt{\frac{\lambda }{N}}\bx^\intercal\bY_\epsilon \bx - \frac{\lambda}{4 N}\|\bx\|^4 .
% % \end{equation*}
% % Recall hypothesis \ref{hyp:eigen} for the noise $\bZ$.
% % Our first intermediate result is a limit for the so-called expected \emph{free entropy}:
% %     \begin{equation*}
% %         f_{\veps,N} := \frac{1}{N}\E  \ln \int d\mu(\bx) \ e^{ \frac{1}{2}\sqrt{\frac{\lambda }{N}}\bx^\intercal\bY_\epsilon \bx  },
% %     \end{equation*}
% %     where, as before, $\mu(\cdot)$ is the uniform measure over $\mathbb{S}^{N-1} (\sqrt{N})$. Here we removed the term proportional to $\|\bx\|^4$ from the log-likelihood as in this case it is just a constant. In other words, in this case we have the free entropy is the mean rank-one spherical integral $$f_{\veps,N} = \frac{1}{N}\E\ln I_N(\sqrt{\lambda}/2,\bY_\epsilon/\sqrt{N}).$$

% Recall hypothesis \ref{hyp:eigen}.
% Our first intermediate result Proposition~\ref{prop:fe_spherical} for the mean log-spherical integral is interesting in itself. But it will also be useful in order to then derive the Bayes MSE by from its derivatives with respect to ${\epsilon}$ and ${\lambda_*}$ (thus the introduction of the Wigner regularization).
 

% % To state the result in this section, for every $\sqrt{\lambda_*}>1/\hmax$ and $\lambda > 0$ we will define the function $\tilde\phi_\rho(\lambda,\lambda_*)$ according to
% % \begin{equation*}
% %     \tilde\phi_\rho(\lambda,\lambda_*) :=
% %     \begin{cases}
% %         \frac{1}{2}\int_0^{\sqrt{\lambda}} R_\rho(t) dt & \mbox{if }  \sqrt{\lambda \lambda_*} < 1\\
% %         \frac{\sqrt \lambda}2K_\rho(1/\sqrt{\lambda_*}) - \frac{1}{2}\int_\Sigma d\rho(t)\ln\left(\sqrt{\lambda} e(K_\rho(1/\sqrt{\lambda_*})-t)\right) & \mbox{if } \sqrt{\lambda\lambda_*} \geq 1.
% %     \end{cases}
% % \end{equation*}
% % We will also define for $\lambda,\lambda_* > 0$ another function
% % \begin{equation*}
% %     \psi_\rho(\lambda,\lambda_*) :=
% %     \begin{cases}
% %         \phi_\rho(\sqrt{\lambda}/2) & \mbox{if }  \sqrt{\lambda_*} < \frac{1}{\hmax}\\
% %         \tilde\phi_ {\rho}(\lambda,\lambda_*) & \mbox{if } \sqrt{\lambda_*} \geq \frac{1}{\hmax}.
% %     \end{cases}
% % \end{equation*}

% % \begin{proposition}\label{prop:fe_spherical}
% %     Under this setting, for each $\lambda,\lambda_* > 0$ we have $\lim_{N\to\infty} f_{\veps,N} = \psi_\rho(\lambda,\lambda_*)$.
% % \end{proposition}

% % \paragraph{Example.} \manunote{Add computation of example of noise with Rademacher eigenvalues. Include graphs and discussion.}


% % JEAN: my computations yield the following (which matches Manuel's computation):
%     % In the next proposition, we establish the limit value of the free entropy in the setting considered. 
%     % For this, define
%     % \begin{equation*}
%     %     g_{\lambda,\epsilon}(x):=\frac{\sqrt\lambda}2x- \frac{1}{2}\int_K d\rho_{\epsilon}(t)\ln( x-t)-\frac12-\frac14\ln\lambda.
%     % \end{equation*}
%     % Notice that its derivative is given by
%     % \begin{equation*}
%     %     g'_{\lambda,\epsilon}(x)=\frac{\sqrt\lambda}2- \frac{1}{2}H_\veps(x).
%     % \end{equation*}
    
%     \begin{proposition}[Mean spherical integral]\label{prop:fe_spherical}
%     Let $\rho_\veps(\cdot)$ be the weak limit of the empirical spectral density of $\bY_\veps$ with associated R-transform be $R_\epsilon$ and define
%     \begin{equation*}
%         g_{\lambda,\epsilon}(x):=\frac{\sqrt\lambda}2x- \frac{1}{2}\int d\rho_{\epsilon}(t)\ln( x-t)-\frac12-\frac14\ln\lambda.
%     \end{equation*}
%         For each $\lambda,\lambda_* > 0$ we have that 
%         \begin{align*}
%         \lim_{N\to+\infty} \frac{1}{N}\E\ln I_N\Big(\frac{\sqrt{\lambda}}2, \bY_\veps\Big)= f_\veps(\lambda_*,\lambda) :=
%              \begin{cases}        
%                 g_{\lambda,\epsilon}(K_\veps(1/\sqrt{\lambda_*}))  &\mbox{if }  \sqrt{\lambda_*} \ge \frac{1}{\hmax} \ \mbox{and}\ \lambda\lambda_*> 1,\\
%                 g_{\lambda,\epsilon}(\overline{\gamma}) &\mbox{if }  \sqrt{\lambda_*} < \frac{1}{\hmax} \ \mbox{and}\ \sqrt{\lambda}>  \hmax,\\
%                 \frac12 \int_0^{\sqrt \lambda} R_\veps(t)dt   &\mbox{else}.
%             \end{cases}   
%         \end{align*}
%     \end{proposition}
    
    In order to state our result for the MSE of the Bayes estimator \eqref{BayesEst} we define the following two functions of $\lambda,\lambda_* > 0$ and the asymptotic spectral measure of the noise $\rho(\cdot)$:
    \begin{equation}
    \begin{cases}
        M(\lambda,\lambda_*) &:=
            \big( 1- \frac{1}{\sqrt{\lambda\lambda_*}} \big) \big(1 - R'_{\rho}(\lambda_*^{-1/2}){\lambda_*}^{-1}\big) \boldsymbol{1}(\hmax\sqrt{\lambda_*} \geq 1 \cap \lambda \lambda_* > 1),\\
            Q(\lambda,\lambda_*) &:=
            \big(1 - \frac{1}{\sqrt{\lambda\lambda_*}}\big)^2 \boldsymbol{1}(\hmax\sqrt{\lambda_*} \geq 1 \cap \lambda \lambda_* > 1) + \big(1 - \frac{\hmax}{\sqrt{\lambda}}\big)^2  \boldsymbol{1}(\hmax \sqrt{\lambda_*} < 1 \cap \sqrt{\lambda} > \hmax);
            \end{cases}      
    \end{equation}
    where $\boldsymbol{1}(\cdot)$ stands for the indicator function of event $\{\cdot\}$. In terms of these functions, we have the next result for the mismatched Bayes estimator \eqref{BayesEst} which characterizes its associated MSE.
    \begin{thm}[MSE of mismatched Bayes estimator]\label{thm:lim_mse}
        Assume Hypothesis \ref{hyp:eigen} holds, then
        \begin{equation*}
            {\rm MSE}(M_{\rm mis})= \frac{1}{2}\left(1 + Q(\lambda,\lambda_*) - 2 M(\lambda,\lambda_*)\right).
        \end{equation*}
    \end{thm}
    
    It is easy to check that in the special case in which $\lambda = \lambda_*$ (i.e., there is no mismatch in the SNR) and $\hmax \geq 1$, ${\rm MSE}(M_{\rm mis}) = {\rm MSE}(M_{\rm GS})$. However, in general they defer. For example, when the assumed SNR $\lambda$ is different from the real one $\lambda_*$, the norm of $M_{\rm mis}$ incorporates some information about $\lambda_*$ while the one for $M_{\rm GS}$ only depends on $\lambda$.

==> images/sections/05Algo.tex <==
\subsection{Approximate message-passing algorithm}\label{sec:AMP}

% For convenience, throughout this section, we will consider a different scaling of spiked model, namely,
% \begin{align}\label{eq:spikedmodelnew}
% \bY=\frac{\sqrt{\lambda}}{N} \bX\bX^\intercal + \bZ,
% \end{align}
% We will need that $\|\bX\|/\sqrt{N}$ is bounded by a constant (independent of $N$) \mm{I'll need finite second moment of $X$} and the eigenvalues of $\bZ$ are $\Theta(1)$\mm{I'll need that $\bZ$ has bounded operator norm}. We consider the following approximate message passing (AMP) algorithm to estimate $\bX\in\mathbb R^N$ from the data matrix $\bY\in \mathbb R^{N\times N}$. For simplicity, we assume to have access to an initialization $\hat{\bx}^1\in \mathbb R^N$, which is independent of the noise $\bZ$ and has a strictly positive correlation with $\bX$, i.e., 
% \begin{equation}\label{eq:AMPinit}
% (\bX, \hat{\bx}^1)\stackrel{\mathclap{W_2}}{\longrightarrow} (X, \hat{x}_1), \quad \mathbb E[X \,\hat{x}_1]:=\epsilon>0, \quad \mathbb E[\hat{x}_1^2]\le 1.
% \end{equation}
% We note that this initialization is impractical and one can initialize AMP with the principal component analysis (PCA) estimate, see e.g. \cite{mondelli2021pca,zhong2021approximate}. 
% Then, for $t\ge 1$, we compute:
% \begin{equation}\label{eq:AMP}
% \bx^t = \bY\hat{\bx}^t-\beta_t\hat{\bx}^{t-1},\quad \hat{\bx}^{t+1} = h_{t+1}(\bx^t),
% \end{equation} 
% where we assume that $\hat{\bx}^{0}=\bzero$.
% Here, the function $h_{t+1}:\mathbb R\to\mathbb R$ is applied component-wise; $\beta_1=0$ and, for $t\ge 2$, $\beta_t=\langle h_t'(\bx^{t-1}) \rangle$, where $h_t'$ denotes the first derivative of $h_t$.

Theorem \ref{thm:AMP} shows that the joint empirical distribution of the iterates $(\bx^1, \ldots, \bx^t, \hat{\bx}^1, \ldots,\hat{\bx}^{t+1})$ converges (in Wasserstein $W_2$ distance) to the random vector $(x_1, \ldots, x_t, \hat{x}_1, \ldots, \hat{x}_{t+1})$. The law of this random vector is captured by a deterministic \emph{state evolution} recursion, which can be  expressed via a sequence of vectors $\bmu_t=(\mu_1, 
\ldots, \mu_t)$ and matrices $\bSigma_t, \bDelta_t, \bB_t\in \mathbb R^{t\times t}$. We start with the initialization 
\begin{equation}\label{eq:SEinit}
\mu_1 = \sqrt{\lambda}\epsilon,\quad \bSigma_1 =\bar{\kappa}_2 \mathbb E[\hat{x}_1^2], \quad \bDelta_1 =\mathbb E[\hat{x}_1^2],\quad \bB_1 = \bar{\kappa}_1,
\end{equation}
where we recall that $\{\bar{\kappa}_k\}_{k\ge1}$ is the sequence of free cumulants associated to $\rho$. \mm{maybe worth defining free cumulants at the beginning?} For $t\ge 1$, given $\bmu_t, \bSigma_t, \bDelta_t, \bB_t$, let 
\begin{equation}\label{eq:SElaws}
\begin{split}
(z_1&, \ldots, z_t)\sim\mathcal N(\bzero, \bSigma_t) \mbox{ and independent of }(X, \hat{x}_1),\\
 x_t &= z_t+\mu_t X- \bar{\beta}_t\hat{x}_{t-1}+\sum_{i=1}^t (\bB_t)_{t, i}\hat{x}_i,\quad \hat{x}_{t+1}=h_{t+1}(x_t),
\end{split}
\end{equation}
where we have defined $\hat{x}_0=0$, $\bar{\beta}_1= 0$, and for $t\ge 2$, $\bar{\beta}_t=\mathbb E[h_t'(x_{t-1})]$. Then, the parameter $\mu_{t+1}$ is given by
\begin{equation}\label{eq:SEmu}
\mu_{t+1} = \sqrt{\lambda}\mathbb E[X\,\hat{x}_{t+1}].
\end{equation}
Next, we compute the entries of the matrix $\bDelta_{t+1}$ as
\begin{equation}
(\bDelta_{t+1})_{i, j} = \mathbb E[\hat{x}_{i}\,\hat{x}_{j}], \quad 1\le i, j\le t+1.
\end{equation}
Furthermore, the matrix $\bB_{t+1}$ is given by
\begin{equation}\label{eq:defB}
\bB_{t+1} = \sum_{j=0}^t \bar{\kappa}_{j+1}\bar{\bPhi}_{t+1}^j,
\end{equation}
where
\begin{equation}\label{eq:defbPhibar}
(\bar{\bPhi}_{t+1})_{i, j}=0 \quad \mbox{ for }i\le j \quad \mbox{and}\quad (\bar{\bPhi}_{t+1})_{i, j}=\mathbb E[\partial_j \hat{x}_i] \quad \mbox{ for }i> j,
\end{equation}
and $\partial_j \hat{x}_i$ denotes the partial derivative $\partial_{z_j} h_i\left(z_{i-1}+\mu_{i-1} X- \bar{\beta}_{i-1}\hat{x}_{i-2}+\sum_{k=1}^{i-1} (\bB_t)_{i-1, k}\hat{x}_k)\right)$. Finally, we define the covariance matrix $\bSigma_{t+1}$ as
\begin{equation}\label{eq:defSigma}
\bSigma_{t+1} = \sum_{j=0}^{2t}\bar{\kappa}_{j+2}\bTheta_{t+1}^{(j)}, \qquad \mbox{with}\quad\bTheta_{t+1}^{(j)} = \sum_{i=0}^j (\bar{\bPhi}_{t+1})^i\bDelta_{t+1}(\bar{\bPhi}_{t+1}^\intercal)^{j-i}.
\end{equation}
We remark that the $t\times t$ top left sub-matrices of $\bSigma_{t+1}, \bDelta_{t+1}$ and $\bB_{t+1}$ are given by $\bSigma_t, \bDelta_t$ and  $\bB_t$, respectively. 

At this point, we are ready to state our state evolution characterization of the AMP algorithm \eqref{eq:AMP}. We make the following assumption on the functions $\{h_{t+1}\}_{t\ge 1}$:
\begin{enumerate}
   \item[\textbf{(A1)}]  The function $h_{t+1}:\mathbb R\to\mathbb R$ is Lipschitz, and the partial derivatives $$\partial_{z_k} h_{t+1}\left(z_{t}+\mu_{t} X- \bar{\beta}_t\hat{x}_{t-1}+\sum_{k=1}^{t} (\bB_t)_{t, k}\hat{x}_k\right)$$ are continuous on a set of probability $1$, under the laws of $(z_1 \ldots, z_t)$ and $(\hat{x}_1,\ldots, \hat{x}_{t})$ given in  \eqref{eq:SElaws}.
    \label{assump:A1}
\end{enumerate}
We note that this assumption is milder than requiring $h_{t+1}$ to be Lipschitz and continuously differentiable.\mm{need to define somewhere PL(2) functions}

\begin{thm}
    Consider a spiked model \eqref{eq:spikedmodel} with the assumptions in Section \ref{sec:intro} and the AMP \eqref{eq:AMP}, initialized as in \eqref{eq:AMPinit} with the assumption \textbf{(A1)} above.
    Let  $\psi:\mathbb R^{2t+2} \to \mathbb R$ be any pseudo-Lipschitz functions of order $2$. Then for each $t \ge 1$,  we almost surely have
    %
    \begin{align}
        & \lim_{N \to \infty} \frac{1}{N} \sum_{i=1}^{N} \psi((\bx^1)_i, \ldots, (\bx^t)_i, \,  (\hat{\bx}^1)_i, \ldots, (\hat{\bx}^{t+1})_i, \, (\bX)_i) = \E[ \psi(x_1, \ldots, x_t, \hat{x}_1, \ldots, \hat{x}_{t+1}, \, X) ], \label{eq:PL2_main_resultx} 
    \end{align}
    where the random variables on the right are defined in \eqref{eq:SElaws}.
    Equivalently, as $N \to \infty$, almost surely:
    \begin{equation}
        \begin{split}
                & (\bx^1, \ldots, \bx^t, \,  \hat{\bx}^1, \ldots, \hat{\bx}^{t+1}, \, \bX) \, \stackrel{W_2}{\longrightarrow}  \,  (x_1, \ldots, x_t, \, \hat{x}_1, \ldots, \hat{x}_{t+1}, \, X).
        \end{split}
        \label{eq:W2_result}
    \end{equation}
    \label{thm:AMP}
\end{thm}

To obtain the state evolution characterization of Theorem \ref{thm:AMP}, the idea is to design an auxiliary AMP algorithm whose iterates are close to those of the AMP in \eqref{eq:AMP}. This auxiliary AMP is an instance of the abstract  AMP iteration for rotationally invariant matrices analyzed in \cite{fan2020approximate,zhong2021approximate}. Therefore, a state evolution result for the auxiliary AMP  can be readily obtained.
We then show that each iterate of the AMP \eqref{eq:AMP} is close to one of the auxiliary AMP and, therefore, the state evolution for the auxiliary AMP also captures the high-dimensional behavior of the AMP \eqref{eq:AMP}. The details are deferred to Appendix \ref{app:proofAMP}: in Appendix \ref{subsec:auxAMP}, we define the auxiliary AMP; in Appendix \ref{subsec:auxAMPSE}, we prove a state evolution result for the auxiliary AMP; and in Appendix \ref{subsec:proof}, we give the proof of Theorem \ref{thm:AMP}.
%
\mm{discuss somewhere (maybe in Preliminaries) the equivalence between \eqref{eq:PL2_main_resultx} and \eqref{eq:W2_result}}

\mm{discuss choices of the pseudo-Lipschitz functions to obtain MSE and overlap}



% \subsection{Spectral algorithm: PCA}

% THe results of ?? state 

% \begin{thm}[Theorem x.x, cite]\label{thm:larg_eigen2}
%     Recall $\Sigma_{\rm max} := \max\{\Sigma_1,\dots,\Sigma_N\}$. As $N\to\infty$, the largest eigenvalue of $\bY$ converges a.s. to
%     \begin{equation*}
%         \tilde\Sigma_{\rm max} := 
%         \begin{cases}
%             K_\rho(N/(\sqrt{\lambda_*}||\bX||^2)) & \mbox{if }\ \frac{\sqrt{\lambda_*}}{N}||\bX||^2 \geq \frac{1}{H_{\rm max}}, \\
%             \Sigma_{\rm max} & \mbox{if } \ \frac{\sqrt{\lambda_*}}{N}||\bX||^2 < \frac{1}{H_{\rm max}}.
%         \end{cases}
%     \end{equation*}
% \end{thm}

% and OVERLAP PCA

==> images/sections/06ApplicDiscuss.tex <==
We will consider a number of examples of applications of these results.

    

    \manunote{In what follows we should add some discussion about the plots obtained. The script with which I made all the plots in this section can be found in \href{https://colab.research.google.com/drive/11Llmm0jr7-nz7x9AGkG4GaHtsTpB3jv1?usp=sharing}{this link}.}

    \paragraph{Rademacher spectrum.} In the special case of a spectrum with Rademacher law $\rho=\frac12(\delta_{1}+\delta_{-1})$ (which implies that the noise is a random orthogonal matrix) we have $\Sigma_{\rm max}=1$, $H_{\rm max}=+\infty$ and for $x > 0$
        \begin{equation*}
            R_\rho(x) = \frac{\sqrt{4 x^2 + 1}-1}{2x} \ \mbox{  and  } \ R'_\rho(x) = \frac{2}{\sqrt{4 x^2 + 1}} - \frac{\sqrt{4 x^2 + 1}-1}{2x^2}.
        \end{equation*}
        Because $H_{max} \geq 1$, by Theorem \ref{thm:lim_mse} we get from this that if $\lambda = \lambda_*$ then
        \begin{equation*}
            \lim_{N\to\infty} \frac{1}{2N^2} \E||\langle x x^T\rangle - X X^T||^2 =
            \begin{cases}
                1 - \frac{1}{2\lambda}\left(2-\frac{1}{\lambda}\right) - \left(1-\frac{1}{\lambda}\right)\left( 1 - \frac{2}{\lambda\sqrt{4 / \lambda+ 1}} + \frac{1}{2}(\sqrt{4 / \lambda + 1}-1) \right) & \mbox{if } \ \lambda > 1 \\
                \frac{1}{2} & \mbox{else}.
            \end{cases}
        \end{equation*}
        
        Let us compare this to the performance of the spectral algorithm. From (Benaych-georges and Nadakuditi), for the Rademacher spectrum (for which $(H_{\rm min},H_{\rm max})=\mathbb{R}$) we have almost surely that for any $\lambda_*>0$,
        \begin{align*}
            \lim_{N\to\infty}\frac{1}{N}\big|\bx_{\rm PCA}^\intercal\bX\big|^2 = \frac{-K'_{\rm rad}(1/\sqrt{\lambda_*})}{\lambda_*}.
        \end{align*}
        Because $K'_{\rm rad}(x) = R'_{\rm rad}(x) - 1/x^2$, this gives
        \begin{align*}
            \lim_{N\to\infty}\frac{1}{N}\big|\bx_{\rm PCA}^\intercal\bX\big|^2 = \frac{1}{2}\left(\sqrt{4/\lambda_*+1}+1\right) - \frac{2}{\lambda_* \sqrt{4/\lambda_*+1}}.
        \end{align*}
        If we rescale the norm of the PCA estimator $\bx_{\rm PCA}\bx_{\rm PCA}^T$ by a factor $v(\lambda_*)$ and choose the $v$ that minimises the MSE, we get that
        \begin{equation*}
            v(\lambda_*) = \frac{1}{2}\left(\sqrt{4/\lambda_*+1}+1\right) - \frac{4}{\lambda_* \sqrt{4/\lambda_*+1}};
        \end{equation*}
        from which we obtain that for every $\lambda_* > 0$
        \begin{equation*}
            {\rm MSE}_{\rm PCA} = \lim_{N\to\infty} \frac{1}{2N^2}||v(\lambda_*) \bx_{\rm PCA}\bx_{\rm PCA}^T - X X^T||^2 = \frac{1}{2}\left[1 -\left(\frac{1}{2}\left(\sqrt{4/\lambda_*+1}+1\right) - \frac{2}{\lambda_* \sqrt{4/\lambda_*+1}}\right)^2 \right].
        \end{equation*}
        
        \manunote{Plot uninformed PCA also. And gaussian noise scaling.}
        
        In Figure \ref{fig:MSE_radspec} we plot the MSE corresponding to the mismatched Bayes estimator and the PCA estimator with optimal norm.
        \begin{figure}[ht]\label{fig:MSE_radspec}
            \centering{
                \includegraphics[width=0.4\linewidth]{images/MSE_RadSpec_BayesPCA.png}
            }
            \caption{Value of the asymptotic MSE of the mismatched Bayes estimator for noise spectrum given by the Rademacher distribution and PCA estimator with optimal norm.}
        \end{figure}

    \paragraph{Free convolution of Rademacher and Semicircle spectra.} In this example, we will consider the noise matrix $\bZ$ to be given, for some $t\in(0,1)$, by $\bZ_t:=\sqrt t\,\bW + \sqrt{1-t}\,\bA$; where $\bW$ is a standard Wigner matrix with spectral distribution given by the semicircle law of radius $2$ while $\bA$ is a matrix with Rademacher spectrum as before. Notice that if $R_\bX(x)$ is the $R$-transform fo some matrix $\bX$ and $a > 0$, then $R_{a\bX}(x)=aR_{\bX}(ax)$. Thus, denoting $R_t(x)$ the $R$-transform of $\bZ_t$ we obtain
        \begin{align}
          R_{t}(x)= tx + \frac{\sqrt{4(1-t)x^2 +1}-1}{2x} \ \mbox{ and } \ R'_{t}(x)=t+\frac{2(1-t)}{\sqrt{4(1-t)x^2 + 1}} - \frac{\sqrt{4(1-t)x^2 + 1}-1}{2x^2}.
        \end{align}
        When $\lambda_*=\lambda$ and because $H_{max} \geq1$ for all $t\in[0,1]$, applying Theorem \ref{thm:lim_mse} and the above expression for $R'_t(x)$ we can readily obtain the MSE for this interpolation model. In Figure \ref{fig:MSE_interpspec} we plot the MSE corresponding to the mismatched Bayes estimator for different values of $t\in[0,1]$.
        \begin{figure}[ht]\label{fig:MSE_interpspec}
            \centering{
                \includegraphics[width=0.4\linewidth]{images/MSE_InterpSpec_Bayes.png}
            }
            \caption{Value of the asymptotic MSE of the mismatched Bayes estimator for spectrum given by the above interpolation. For comparison, we present the results for three values of $t$: 0.001, 0.5, and 1.}
        \end{figure}

    \paragraph{Marcenko-Pastur spectrum.} Consider a centered Marcenko-Pastur density of variance $\alpha > 0$
        \begin{equation*}
            \rho(x) = \frac{\sqrt{(\alpha_{+}+1 - x)(x - (\lambda_{-}+1))}}{2\pi\alpha (x-1)} \,\mathbf{1}_{x\in[\alpha_{-}, \alpha_{+}]}
        \end{equation*}
        with $\alpha_{\pm} = \sigma^2(1 \pm \sqrt{\alpha})^2$. Because we have that
        \begin{equation*}
            H_{max}(\alpha) = \frac{1}{\sqrt{\alpha}(1+\sqrt{\alpha})},
        \end{equation*}
        then if $\alpha \leq (\sqrt{5}-1)^2/4$ we have $H_{max}(\alpha) \geq 1$. Also, because $\rho_\alpha(\cdot)$ can be thought of as the density of a Wishart matrix minus the identity, by additivity of the $R$-transform and the fact that the $R_{\mathbb{I}}(x)=1$ for the identity, we have that for all $\alpha > 0$
        \begin{align*}
            R_{\rho_\alpha}(x) =\frac1{1-\alpha x}-1=\frac{\alpha x}{1-\alpha x}, \qquad R'_{\rho_\alpha}(x)=\frac{\alpha}{(\alpha x-1)^2}.
        \end{align*}
        Thus, if $\alpha \leq (\sqrt{5}-1)^2/4$ and $\lambda = \lambda_*$ we get by Theorem \ref{thm:lim_mse}
        \begin{equation*}
            \lim_{N\to\infty}\frac{1}{2N^2}\E||\thermal{x x^T}- X X^T||^2 =
            \begin{cases}
                    1 - \frac{1}{2\lambda}\left(2-\frac{1}{\lambda}\right) - \left(1-\frac{1}{\lambda}\right)\left(1 - \frac{\alpha}{(\alpha-\sqrt{\lambda})^2}\right) & \mbox{if } \lambda > 1\\
                    \frac{1}{2} & \mbox{if } \lambda \leq 1.
            \end{cases}
        \end{equation*}
        In the Figure \ref{fig:MSE_MPspec} we plot the MSE corresponding to the mismatched Bayes estimator for different values of $\alpha\leq(\sqrt{5}-1)^2/4$. Observe that the same formula applies in case where the law was not centred (i.e., for the standard MP law).
        
        \begin{figure}[ht]\label{fig:MSE_MPspec}
            \centering{
                \includegraphics[width=0.4\linewidth]{images/MSE_MPspec_Bayes.png}
            }
            \caption{Value of the asymptotic MSE of the mismatched Bayes estimator for noise spectrum given by the centered Marchenko-Pastur distribution. For comparison, we present the results for three values of $\alpha$: 0.001, 0.3, and $(\sqrt{5}-1)^2/4$.}
        \end{figure}
        
        \paragraph{Uniform distribution.} Uniform distribution in $[-\alpha,\alpha]$, where $\alpha > 0$.
        
        $H(z) = \frac{1}{2\alpha}\ln\left(\frac{z+\alpha}{z-\alpha}\right)$, then $H_{max} = \infty$.
        
        Inverting we get that $K(x) = \frac{\alpha}{\tanh(\alpha x)}$.
        
        For the cumulants we use the expansion of $\coth(x)$ in terms of Bernoulli numbers.
  
%MANU: Does it make sense to include the two semicircle law example? The density is really similar to the free convolution of Rademacher and semicircle. I commented what was written on this. If someone wants to work out the example they can uncomment and complete the computations.  
  
%    \subsubsection{``Double semicircles'' spectrum.} Consider the eigenvalues density given by 
%        \begin{align*}
%            \rho(x)=
%            \begin{cases}
%              \frac1\pi \sqrt{|1 - (x - \sqrt{3/4})^2|} & \mbox{if }\ |x - \sqrt{3/4}| < 1, \\
%              \frac1\pi \sqrt{|1 - (x + \sqrt{3/4})^2|}& \mbox{if }\ |x + \sqrt{3/4}| < 1,\\
%              0  & \mbox{else }.
%              \end{cases}
%        \end{align*}
%        This is two semicircles centred in $\pm 3/4$. The variance of this measure is $1$. Its R-transform can be obtained... \manunote{Complete this example}



%\subsubsection{Gaussian prior}
%
%    Here we will prove the asymptotic limit of the expected free entropy in the case where the distribution of $\bX$ and the prior of $\bx$ are both standard gaussian distributions. In particular, we have the next proposition.
%    
%    \begin{proposition}\label{prop:fe_gaussian}
%        Under this setting, for every $\lambda,\lambda_* > 0$ we have
%        \begin{equation*}
%            \lim_{N\to\infty} f_{\veps,N} = \sup_{x\in\R_+} \left(f_\veps(\lambda x^2,\lambda_*) + \frac{1}{2}\left(\ln x + 1 - x - \frac{\lambda x^2}{2} \right)\right).
%        \end{equation*}
%    \end{proposition}
%    
%    \manunote{Discuss MSE formula in this case.}

==> images/sections/07App_PCAbackground.tex <==
In this appendix we present some of the known results for the spectrum of low rank perturbation of rotational invariant matrices as proved in \cite{benaych2011eigenvalues,benaych2012singular}. In particular, we present them in a different form more convenient for our discussion and we specialize them for rank-1 perturbations. For the full statement of the theorems, the reader should consult the references cited. The notations here are the same as the ones in Section \ref{sec:bayes}.

The first result we will include here characterizes the asymptotic value of the largest eigenvalue of the the perturbed matrix $\bY$.
\begin{thm}[Theorem 2.1 of \cite{benaych2011eigenvalues}]\label{thm:larg_eigen}
    As $N\to\infty$, the largest eigenvalue $\eigmax$ of $\bY$ converges a.s. to
    \begin{equation*}
        \eigmax := 
        \begin{cases}
            K_\rho(1/\sqrt{\lambda_*}) & \mbox{if }\ \hmax\sqrt{\lambda_*} \geq 1, \\
            \overline{\gamma} & \mbox{else}.
        \end{cases}
    \end{equation*}
\end{thm}
This theorem thus implies that, below the phase transition, the presence of the perturbation does not modify the largest eigenvalue of the matrix.

For the inner product between $\bX$ and the eigenvector corresponding to the largest eigenvalue, the authors prove the following asymptotic result.
\begin{thm}[Theorem 2.2 of \cite{benaych2011eigenvalues}]\label{thm:inner_eigen}
    As $N\to\infty$, the eigenvector $\overline{\bv}$ corresponding to the largest eigenvalue $\eigmax$ of $\bY$ is such that a.s.
    \begin{equation*}
        C(\rho,\lambda_*) := \lim_{N\to\infty} \frac{|\bX^T\overline{\bv}|}{N}^2 = 
        \begin{cases}
            1 - \frac{R'_\rho(\lambda_*^{-1/2})}{\lambda_*} & \mbox{if }\ \hmax\sqrt{\lambda_*} \geq 1, \\
            0 & \mbox{else}.
        \end{cases}
    \end{equation*}
\end{thm}
In this case, below the phase transition, the spectral estimators will not be correlated with the ground truth.

==> images/sections/08App_proofBayes.tex <==
For every $\theta > 0$ and matrix $\bA\in\R^{N\times N}$ the rank-1 spherical integral is defined according to
\begin{equation*}
    I_N(\theta,\bA) := \int d\mu_N(\bs) \exp\big(\theta \bs^\intercal\bA \bs\big);
\end{equation*}
where, as before, $\mu_N(\cdot)$ is the uniform measure over $\mathbb{S}^{N-1}(\sqrt{N})$.

It will be useful to define a slight generalization of the model \eqref{eq:spikedmodel} that includes a ``Wigner regularization'' of the rotationally-invariant noise. Namely, we will consider in this section the following generalized model for the data:
\begin{align}\label{eq:spikedmodel_wigReg}
\bY_\veps=\frac{\sqrt{\lambda}} {N} \bX\bX^\intercal + \bZ+\sqrt{\veps}\,\bW;
\end{align}
where, as before, $\bW$ is a standard Wigner matrix and $\veps>0$ is some constant. In a similar way as we did for the non-regularized problem, we will denote by $\thermal{\cdot}_\veps$ the mean of the Gibbs measure obtained by replacing $\bY$ for $\bY_\veps$ in equation \eqref{estimatorMis1}. The rest of the notations used here will be similar to the ones for the non-regularized model, though we will add a subscript $\veps$ when it is useful to remark dependence of a given quantity over this parameter. When this subscript is omitted, it is understood that $\veps=0$.
%Recall the form of the log-likelihood when assuming purely Wigner noise:
% \begin{equation*}
%     \mathcal{L}_N(\bx) = \frac{1}{2}\sqrt{\frac{\lambda }{N}}\bx^\intercal\bY_\veps \bx - \frac{\lambda}{4 N}\|\bx\|^4 .
% \end{equation*}
% Recall hypothesis \ref{hyp:eigen} for the noise $\bZ$.
% Our first intermediate result is a limit for the so-called expected \emph{free entropy}:
%     \begin{equation*}
%         f_{\veps,N} := \frac{1}{N}\E  \ln \int d\mu(\bx) \ e^{ \frac{1}{2}\sqrt{\frac{\lambda }{N}}\bx^\intercal\bY_\veps \bx  },
%     \end{equation*}
%     where, as before, $\mu(\cdot)$ is the uniform measure over $\mathbb{S}^{N-1} (\sqrt{N})$. Here we removed the term proportional to $\|\bx\|^4$ from the log-likelihood as in this case it is just a constant. In other words, in this case we have the free entropy is the mean rank-one spherical integral $$f_{\veps,N} = \frac{1}{N}\E\ln I_N(\sqrt{\lambda}/2,\bY_\veps/\sqrt{N}).$$

Our first intermediate result, Proposition~\ref{prop:fe_spherical}, characterizes the mean log-spherical integral for the regularized data matrix. Although this proposition may be interesting in itself, its main porpoise here will be to allow us to derive the MSE of the mismatched Bayes estimator in terms of derivatives of the the mean log-spherical integral with respect to ${\veps}$ and ${\lambda_*}$. This is in fact the reason for introducing the regularization in the first place.
 

% To state the result in this section, for every $\sqrt{\lambda_*}>1/\hmax$ and $\lambda > 0$ we will define the function $\tilde\phi_\rho(\lambda,\lambda_*)$ according to
% \begin{equation*}
%     \tilde\phi_\rho(\lambda,\lambda_*) :=
%     \begin{cases}
%         \frac{1}{2}\int_0^{\sqrt{\lambda}} R_\rho(t) dt & \mbox{if }  \sqrt{\lambda \lambda_*} < 1\\
%         \frac{\sqrt \lambda}2K_\rho(1/\sqrt{\lambda_*}) - \frac{1}{2}\int_\Sigma d\rho(t)\ln\left(\sqrt{\lambda} e(K_\rho(1/\sqrt{\lambda_*})-t)\right) & \mbox{if } \sqrt{\lambda\lambda_*} \geq 1.
%     \end{cases}
% \end{equation*}
% We will also define for $\lambda,\lambda_* > 0$ another function
% \begin{equation*}
%     \psi_\rho(\lambda,\lambda_*) :=
%     \begin{cases}
%         \phi_\rho(\sqrt{\lambda}/2) & \mbox{if }  \sqrt{\lambda_*} < \frac{1}{\hmax}\\
%         \tilde\phi_ {\rho}(\lambda,\lambda_*) & \mbox{if } \sqrt{\lambda_*} \geq \frac{1}{\hmax}.
%     \end{cases}
% \end{equation*}

% \begin{proposition}\label{prop:fe_spherical}
%     Under this setting, for each $\lambda,\lambda_* > 0$ we have $\lim_{N\to\infty} f_{\veps,N} = \psi_\rho(\lambda,\lambda_*)$.
% \end{proposition}

% \paragraph{Example.} \manunote{Add computation of example of noise with Rademacher eigenvalues. Include graphs and discussion.}


% JEAN: my computations yield the following (which matches Manuel's computation):
    % In the next proposition, we establish the limit value of the free entropy in the setting considered. 
    % For this, define
    % \begin{equation*}
    %     g_{\lambda,\veps}(x):=\frac{\sqrt\lambda}2x- \frac{1}{2}\int_K d\rho_{\veps}(t)\ln( x-t)-\frac12-\frac14\ln\lambda.
    % \end{equation*}
    % Notice that its derivative is given by
    % \begin{equation*}
    %     g'_{\lambda,\veps}(x)=\frac{\sqrt\lambda}2- \frac{1}{2}H_{\rho_\veps}(x).
    % \end{equation*}
    
    \begin{proposition}[Mean spherical integral]\label{prop:fe_spherical}
    Let $\rho_\veps(\cdot)$ be the weak limit of the empirical spectral density of $\bY_\veps$ and $R_\veps$ its associated R-transform. For every $\lambda,\veps>0$, define the function $g_{\lambda,\veps}:\R_{>\overline{\gamma}}\mapsto\R$ according to
    \begin{equation*}
        g_{\lambda,\veps}(x):=\frac{\sqrt\lambda}2x- \frac{1}{2}\int d\rho_{\veps}(t)\ln( x-t)-\frac12-\frac14\ln\lambda.
    \end{equation*}
        Then, under Hypothesis \ref{hyp:eigen} and for every $\lambda,\lambda_* > 0$ we have that 
        \begin{align*}
        \lim_{N\to+\infty} \frac{1}{N}\E\ln I_N\Big(\frac{\sqrt{\lambda}}2, \bY_\veps\Big)= f_\veps(\lambda,\lambda_*) :=
             \begin{cases}        
                g_{\lambda,\veps}(K_{\rho_\veps}(1/\sqrt{\lambda_*}))  &\mbox{if }  \hmax_\veps\sqrt{\lambda_*} \ge 1 \ \mbox{and}\ \lambda\lambda_*> 1,\\
                g_{\lambda,\veps}(\overline{\gamma}_\veps) &\mbox{if }  \hmax_\veps\sqrt{\lambda_*} < 1 \ \mbox{and}\ \sqrt{\lambda}>  \hmax_\veps,\\
                \frac12 \int_0^{\sqrt \lambda} R_{\rho_\veps}(t)dt   &\mbox{else}.
            \end{cases}   
        \end{align*}
    \end{proposition}



\subsection{Proof of Theorem \ref{thm:lim_mse}}

Like in the analysis of mismatched inference with gaussian noise of \cite{pourkamali2021mismatched}, we will make use of the following result for the asymptotic value of the rank-1 spherical integral.
\begin{thm}[Theorem 6 of \cite{guionnet2005fourier}]\label{thm:spher_int} Let $\eigmax_\veps$ be the limit of the maximum eigenvalue of $\bY_\veps$ and define $\hmax_\veps:=\lim_{z\downarrow\eigmax_\veps} H_{\rho_\veps}(z)$. Assume that Hypothesis \ref{hyp:eigen} holds, then
    \begin{equation*}
        \lim_{N\to\infty}\frac{1}{N} \ln I_N(\theta,\bY_\veps) = \phi_\veps(\theta) :=
        \begin{cases}
            \frac{1}{2}\int_0^{2\theta} R_{\rho_\veps}(t) dt & \mbox{if } 2\theta \leq \hmax_\veps\\
            \theta\eigmax_\veps - \frac{1}{2}\int_K d\rho(t)\ln\left(2\theta e(\eigmax_\veps-t)\right) & \mbox{if } 2\theta > \hmax_\veps.
        \end{cases}
    \end{equation*}
\end{thm}
    
\begin{proof}[Proof of Proposition \ref{prop:fe_spherical}]
    By Theorem \ref{thm:larg_eigen}, we are a.s. under the hypothesis of Theorem \ref{thm:spher_int}. We then have that almost surely
    \begin{equation*}
        \lim_{N\to\infty}\frac{1}{N}\ln \int d\mu_N(\bx) \ e^{ \frac{\sqrt{\lambda}}{2}\bx^T \bY \bx } = f_\veps(\lambda,\lambda_*).
    \end{equation*}
    Moreover, because by hypothesis the sequence of values of the largest eigenvalue of $\bZ$ is convergent, it is then bounded by some $C > 0$. Thus,
    \begin{equation*}
        \frac{\sqrt{\lambda}}{2}\bx^T \bY \bx \leq \frac{\sqrt{\lambda}}{2}(C+\sqrt{\lambda_*})N.
    \end{equation*}
    Then the result follows by dominated convergence.
\end{proof}

To establish this result, define the \emph{magnetization} according to $M_N := N^{-2} (\bX^T \bx)^2$ and the \emph{overlap} $Q_N := N^{-2} (\bx^{(1)T} \bx^{(2)})^2$. Here the supra-indices indicate two independent samples from the Gibbs measure with the same quenched disorder. Theorem \ref{thm:lim_mse} is the consequence of the asymptotic formulas for the mean magnetization and overlap of the Gibbs measure given in the next lemmas. 

\begin{lemma}\label{lem:mag_limit}
    In the setting considered, for all $\lambda,\lambda_* > 0$ fixed we have $\lim_{N\to\infty} \E\thermal{M_N}_0 = M(\lambda,\lambda_*)$.
\end{lemma}
\begin{proof}
    Because in the log-likelihood of the problem the only term in which $\lambda_*$ appears (when writing $\bY_\veps$ explicitly in terms of $\bX \bX^T$) is
    \begin{equation*}
        \frac{\sqrt{\lambda \lambda_*}}{2 N} (\bX^T \bx)^2 = N\frac{\sqrt{\lambda \lambda_*}}{2} M_N,
    \end{equation*}
    we then have that for all $N\geq1$
    \begin{equation*}
        \frac{\partial f_{0,N}}{\partial \sqrt{\lambda_*}} = \frac{\sqrt{\lambda}}{2}\E\thermal{M_N}_0.
    \end{equation*}
    By the convexity of $f_{0,N}$ w.r.t. $\sqrt{\lambda_*}$ and Proposition \ref{prop:fe_spherical} we get that
    \begin{equation*}
        \lim_{N\to\infty} \E\thermal{M_N}_0 = \frac{2}{\sqrt{\lambda}} \frac{\partial f_0(\lambda,\lambda_*)}{\partial \sqrt{\lambda_*}} = \frac{2}{\sqrt{\lambda}} \frac{\partial f_0(\lambda,\lambda_*)}{\partial \sqrt{\lambda_*}} = 4\sqrt{\frac{\lambda_*}{\lambda}} \frac{\partial f_0(\lambda,\lambda_*)}{\partial \lambda_*}.
    \end{equation*}
    The derivative with respect to $\lambda_*$ of $f_0$ is given by (recalling $K_0(x)=R_0(x)+1/x$)
    \begin{align*}
        \frac{df_0}{d\lambda_*}(\lambda_*,\lambda)=
         \begin{cases}        
            \frac{1}{4} \big(\frac{1}{(\lambda_*)^2}-\big(\frac{\lambda}{(\lambda_*)^3}\big)^{1/2}\big) \big(R'_\rho(1/\sqrt{\lambda_*})-\lambda_*\big)  &\mbox{if }  \sqrt{\lambda_*} \ge \frac{1}{\hmax} \ \mbox{and}\ \lambda\lambda_*> 1,\\
            0 &\mbox{else}.
        \end{cases}   
    \end{align*}
    From these two last equations, the result of the lemma follows.
\end{proof}

\begin{lemma}\label{lem:ovlap_limit}
    In the setting considered, for all $\lambda,\lambda_* > 0$ fixed we have $\lim_{N\to\infty} \E\thermal{Q_N}_0 = Q(\lambda)$.
\end{lemma}
\begin{proof}
    Because in the log-likelihood of the problem the only term in which $\veps$ appears (when writing $\bY_\veps$ explicitly in terms of $\bW$) is
    \begin{equation*}
        \frac{\sqrt{\lambda \veps}}{2} \bx^T \bW \bx,
    \end{equation*}
    we have that for every $N\geq1$
    \begin{equation*}
        \frac{\partial f_{0,N}}{\partial \sqrt{\veps}} = \frac{\sqrt{\lambda}}{2N}\E\thermal{\bx^T \bW \bx}_0.
    \end{equation*}
    Since $\bW$ is Wigner, its elements are distributed as independent Gaussian random variables. Using gaussian integration by parts in the r.h.s. of the last equation we get that
    \begin{equation*}
        \frac{\partial f_{0,N}}{\partial \sqrt{\veps}} = \frac{\lambda\sqrt{ \veps}}{2}(1 - \E\thermal{Q_N}_0).
    \end{equation*}
    By the convexity of $f_{\veps,N}$ w.r.t. $\sqrt{\veps}$ and Proposition \ref{prop:fe_spherical} we get that
    \begin{equation}\label{eq:ovlp_lim}
        \lim_{N\to\infty} \E\thermal{Q_N}_0 = 1 - \frac{2}{\lambda\sqrt{\veps}} \frac{\partial f_\veps(\lambda,\lambda_*)}{\partial \sqrt{\veps}}\Big|_{\veps=0} = 1 - \frac{4}{\lambda} \frac{\partial f_\veps(\lambda,\lambda_*)}{\partial \veps}\Big|_{\veps=0}.
    \end{equation}
    To find the asymptotic value of $\E\thermal{Q_N}_0$ we are thus left to compute $\partial_\veps f_\veps(\lambda,\lambda)$. We will then need to consider the three regimes of Proposition \ref{prop:fe_spherical}. 
    
    Firstly, if $\hmax\sqrt{\lambda_*}  \geq 1$ and $\lambda \lambda_* > 1$ then
    \begin{equation*}
        \begin{split}
            \frac{\partial f_\veps(\lambda,\lambda_*)}{\partial \veps} \Big|_{\veps=0} & = \frac{d }{d\veps}g_{\lambda,\veps}(K_{\rho_\veps}(\lambda_*^{-1/2})) \Big|_{\veps=0} \\
            & = \frac{\partial g_{\lambda,\veps}(x)}{\partial\veps}\Big|_{\veps=0,x=K_{\rho_0}(\lambda_*^{-1/2})} + \frac{\partial g_{\lambda,\veps}(x)}{\partial x}\Big|_{\veps=0,x=K_{\rho_0}(\lambda_*^{-1/2})} \frac{\partial K_{\rho_\veps}(\lambda_*^{-1/2})}{\partial\veps}\Big|_{\veps=0}.
        \end{split}
    \end{equation*}
    For computing $\partial_\veps g_{\lambda,\veps}(x)$ notice that the only term of $g_{\lambda,\veps}$ in which $\veps$ appears is
    \begin{equation*}
        - \frac{1}{2} \int d\rho_\veps(\gamma) \ln(x-\gamma) = -\frac{1}{2} \int_0^x H_{\rho_\veps}(z) dz.
    \end{equation*}
    Furthermore, by the Dyson Brownian motion characterization of the eigenvalues of the matrix $\bZ + \sqrt{\veps} \bW$ we have that the limiting Stieltjes transform $H_{\rho_\veps}(z)$ is a solution of Burger's equation (see for example, \cite[Proposition 4.3.10]{anderson2010introduction}); that is,
    \begin{equation}\label{eq:burguers}
        \frac{\partial H_{\rho_\veps}}{\partial \veps} = - H_{\rho_\veps} \frac{\partial H_{\rho_\veps}}{\partial z} = - \frac{1}{2} \frac{\partial (H_{\rho_\veps}^2)}{\partial z}.
    \end{equation}
    Integrating both sides of \eqref{eq:burguers} we get that
    \begin{equation}\label{eq:deriv_eps}
        \frac{\partial g_{\lambda,\veps}(x)}{\partial\veps} = \frac{1}{4} H_{\rho_\veps}^2(x).
    \end{equation}
    Which, in particular, means that
    \begin{equation}\label{eq:partial1}
        \frac{\partial g_{\lambda,\veps}(x)}{\partial\veps}\Big|_{\veps=0,x=K_{\rho_\veps}(\lambda_*^{-1/2})} = \frac{1}{4} H_{\rho_0}^2(K_{\rho_0}(\lambda_*^{-1/2})) = \frac{1}{4\lambda_*}.
    \end{equation}
    Furthermore, 
    \begin{equation}\label{eq:deriv_x}
        \frac{\partial g_{\lambda,\veps}(x)}{\partial x} = \frac{\sqrt{\lambda}}{2} - \frac{1}{2} H_{\rho_\veps}(x)
    \end{equation}
    and $\partial_\veps K_{\rho_\veps}(x) = x$. Then,
    \begin{equation}\label{eq:partial2}
        \frac{\partial g_{\lambda,\veps}(x)}{\partial x}\Big|_{\veps=0,x=K_{\rho_\veps}(\lambda_*^{-1/2})} \frac{\partial K_{\rho_\veps}(\lambda_*^{-1/2})}{\partial\veps}\Big|_{\veps=0} = \frac{1}{2}\left(1 - \frac{1}{\lambda_*}\right).
    \end{equation}
    Combining equations \eqref{eq:ovlp_lim}, \eqref{eq:partial1}, and \eqref{eq:partial2} we get that if $\hmax \sqrt{\lambda}   \geq 1$ and $\lambda_*\lambda > 1$, then
    \begin{equation*}
        \lim_{N\to\infty} \E\thermal{Q_N}_0 = 1 - \frac{1}{\lambda} \left(2 - \frac{1}{\lambda}\right).
    \end{equation*}
    

    \manunote{This paragraph is the new part of the proof. It would be good if someone double-checks it.} We will now establish the limit of the overlap when $\hmax\sqrt{\lambda_*} < 1$ and $\sqrt{\lambda} > \hmax$. In this region,
    \begin{equation}\label{eq:region_2}
        \frac{\partial f_\veps(\lambda,\lambda_*)}{\partial \veps} \Big|_{\veps=0}= \frac{d }{d\veps}g_{\lambda,\veps}(\overline{\gamma}_\veps)\Big|_{\veps=0} = \frac{\partial g_{\lambda,\veps}(x)}{\partial\veps}\Big|_{\veps=0,x=\overline{\gamma}_0} + \frac{\partial g_{\lambda,\veps}(x)}{\partial x}\Big|_{\veps=0,x=\overline{\gamma}_0} \frac{\partial \overline{\gamma}_\veps}{\partial\veps}\Big|_{\veps=0}.
    \end{equation}
    The partial derivatives $\partial_\veps g_{\lambda,\veps}(x)$ and $\partial_x g_{\lambda,\veps}(x)$ are obtained as before. Therefore, we only need to compute $\partial_\veps \overline{\gamma}|_{\veps=0}$. We will prove that as $\veps\to0$, $\overline{\gamma}_\veps = \overline{\gamma}_0 + \hmax_0 \veps + o(\veps)$. As a consequence of the Large Deviation Principle of \cite[Theorem 2.5]{guionnet2021large}, $\overline{\gamma}_\veps$ is equal to the supremum of the compact support $K_\veps$ of $\rho_\veps(\cdot)$. Notice that for all $\veps >0$, $\lim_{z\downarrow\overline{\gamma}_\veps} H'_{\rho_\veps} = -\infty$. This implies that $K'_{\rho_\veps}(\hmax_\veps) = 0$. Thus, $\hmax_\veps$ is a solution to the equation $K'_{\rho_0}(x) + \veps = 0$. And because $K'_{\rho_0}$ is analytic and monotonously increasing, the solution is unique and depends smoothly on $\veps$. Thus, $\hmax_\veps = \hmax_0 + \mathcal{O}(\veps)$ which means that
    \begin{equation*}
        \overline{\gamma}_\veps = K_{\rho_0}(\hmax_0) + \veps\hmax_0 + o(\veps) = \overline{\gamma}_0 + \veps\hmax_0 + o(\veps);
    \end{equation*}
    where we used that $K'_{\rho_0}(\hmax_0) = 0$. This proves that $\partial_\veps \overline{\gamma}_\veps|_{\veps=0} = \hmax_0$. Combining this with equations \eqref{eq:ovlp_lim}, \eqref{eq:deriv_eps}, \eqref{eq:deriv_x}, and \eqref{eq:region_2} gives the result in this region. 
    
    Finally, by Proposition \ref{prop:fe_spherical} and \eqref{eq:ovlp_lim} if $(\lambda,\lambda_*)$ does not verify either of the conditions considered above then
    \begin{equation*}
        \lim_{N\to\infty} \E\thermal{Q_N}_0 = 1- \frac{2}{\lambda}\int_0^{\sqrt{\lambda}}\partial_\veps R_{\rho_\veps}(x) dx = 1- \frac{2}{\lambda}\int_0^{\sqrt{\lambda}} x \ dx = 0.
    \end{equation*}
    This finishes the proof that $\lim_{N\to\infty} \E\thermal{Q_N}_0 = Q(\lambda)$.
\end{proof}

\begin{proof}[Proof of Theorem \ref{thm:lim_mse}]
    For establishing the formula for the MSE found in the theorem, it is enough to observe that
    \begin{equation*}
        \frac{1}{2N^2}\E ||\thermal{\bx \bx^T}_0 - \bX \bX^T||_F^2 = \frac{1}{2}(1 + \E\thermal{Q_N}_0 - 2 \E\thermal{M_N}_0),
    \end{equation*}
    and to use Lemmas \ref{lem:mag_limit} and \ref{lem:ovlap_limit}.
\end{proof}

%\subsection{Proof of Proposition \ref{prop:fe_gaussian}}
%    For proving this, we will first introduce an interpolation model and we will prove some technical lemmas for it. Let $\bS := \bX/||\bX||$ and, for every $t\in[0,1]$,
%    \begin{equation*}
%        \bY_t := \bZ + \sqrt{\lambda_* N} \bS {\bS}^T \left((1-t)\frac{||\bX||^2}{N}+t\right).
%    \end{equation*}
%    For every $t,\nu\in[0,1]$ we define the interpolating log-likelihood according to
%    \begin{equation*}
%        l_{N,t,\nu}(\bx) :=  -\frac{\lambda ||\bx||^4}{4 N} + (1-\nu)\ln I_N\left(\frac{\sqrt{\lambda}||\bx||^2}{2N},\frac{\bY_t}{\sqrt{N}}\right)+\nu N\psi_\rho(\lambda||\bx||^4/N^2,\lambda_*)
%    \end{equation*}
%    and we denote by $\langle\cdot\rangle_{t,\nu}$ and $f_{N,t,\nu}$ the corresponding Gibbs mean and expected free entropy. As noted by (Pourkamali and Macris, Mismatch), by the rotational invariance of the standard gaussian distribution, for every orthogonal matrix $\bO'\in\R^{N\times N}$, $\bx$ is equally distributed to $\bO' \bx$. Thus, if $M(\cdot)$ is the Haar measure over the orthogonal matrices on $\R^{N\times N}$
%    \begin{equation*}
%        \begin{split}
%            \int dG(\bx) e^{-\frac{\lambda ||\bx||^4}{4 N} + \frac{1}{2}\sqrt{\frac{\lambda }{N}}\bx^T \bY_0 \bx } & = \int dG(\bx) dM(\bO')  e^{-\frac{\lambda ||\bO' \bx||^4}{4 N} + \frac{1}{2}\sqrt{\frac{\lambda }{N}}(\bO'\bx)^T \bY_0 \bO' \bx}\\
%            & =  \int dG(\bx) e^{-\frac{\lambda ||\bx||^4}{4 N} + \ln I_N\left(\frac{\sqrt{\lambda}||\bx||^2}{2N},\frac{\bY_0}{\sqrt{N}}\right)};
%        \end{split}
%    \end{equation*}
%    where we used that $|\mbox{det}\ \bO'| = 1$. We then have that $f_{N,0,0} = f_N$.
    
%    The strategy of the proof will be the following. We will first show through interpolation that $f_{N,0,0}$ is equal to $f_{N,1,1}$ in the limit of $N\to\infty$. This requires the technical result given in Corollary \ref{cor:secmom_bound}. Then, we establish a large deviation principle for the squared norm of gaussian vectors and use it along with Lemma \ref{lem:varad_hyp} and Varadhan's Lemma to prove the asymptotic expected free entropy formula. It is important to note that although the strategy of the proof is different, the basic idea is the same as in (Pourkamali and Macris, Mismatch): use the change of variables above and Theorems \ref{thm:larg_eigen} and \ref{thm:spher_int} to express the limit of the expected free entropy as an optimisation problem.
    
%    \begin{lemma}\label{lem:exp_bound}
%        There is some $C > 0$ s.t. for every $t,\nu\in[0,1]$ and $N\geq1$
%        \begin{equation*}
%            \ln\langle e^{||\bx||^2/2}\rangle_{t,\nu} \leq N C (||\bX||^4/N^2 + ||\bX||^2/N + 1).
%        \end{equation*}
%    \end{lemma}
%    \begin{proof}
%        To see this, first notice that for every $N\geq1$, $t\in[0,1]$, and $\theta > 0$ we have that
%        \begin{equation}\label{eq:bound_si}
%            {\scriptstyle\left(\Sigma_{min}-\sqrt{\lambda_*}\left((1-t)\frac{||\bX||^2}{N}+t\right)\right)}\theta \leq \frac{1}{N}\ln I_N(\theta,\bY_t)\leq {\scriptstyle\left(\Sigma_{max}+\sqrt{\lambda_*}\left(\frac{(1-t)||\bX||^2}{N}+t\right)\right)}\theta.
%        \end{equation}
%        Because $\psi_\rho(\lambda||\bx||^4/N^2,\lambda_*)$ is the limit of $N^{-1}\ln I_N(\theta,\bY_1)$ evaluated at $\theta = \sqrt{\lambda}||\bx||^2/(2N)$, this implies that
%        \begin{equation}\label{eq:bound_psi}
%            (\Sigma_{min}-\sqrt{\lambda_*})\frac{\sqrt{\lambda}||\bx||^2}{2 N}  \leq \psi_\rho(\lambda||\bx||^4/N^2,\lambda_*) \leq (\Sigma_{max}+\sqrt{\lambda_*})\frac{\sqrt{\lambda}||\bx||^2}{2 N}.
%        \end{equation}
%        Therefore, for all $\bx\in\R^N$ and $t,\nu\in[0,1]$
%        \begin{equation}\label{eq:bound_ham}
%            \begin{split}
%                l_{N,t,\nu}(\bx) & \leq -\frac{\lambda ||\bx||^4}{4 N} + \left(\Sigma_{max}+\sqrt{\lambda_*}\left(\frac{||\bX||^2}{N}+1\right)\right)\frac{\sqrt{\lambda}||\bx||^2}{2 N}\\
%                & \leq \frac{N}{4}\left(\Sigma_{max}+\sqrt{\lambda_*}\left(\frac{||\bX||^2}{N}+1\right) \right)^2.
%            \end{split}
%        \end{equation}
%        On the other hand, if we define $A:=\{\bx\in\R^N:||\bx||^2\leq 2 N\}$ then by bounds \eqref{eq:bound_si} and \eqref{eq:bound_psi} we have that for all $t,\nu\in[0,1]$
%        \begin{equation}\label{eq:bound_parf}
%            \begin{split}
%                Z_N = \int_{\R^N} dG(\bx) e^{l_{N,t,\nu}(\bx)} & \geq \int_A dG(\bx) e^{l_{N,t,\nu}(\bx)} \\
%                & \geq e^{-\left(\lambda+\sqrt{\lambda\lambda_*}\left(\frac{||\bX||^2}{N}+1\right)-\sqrt{\lambda}\Sigma_{min}\right)N} G(\mathbb{I}_A).
%            \end{split}
%        \end{equation}
%        And because the law of large numbers implies that $G(\mathbb{I}_A)\to1$, equations \eqref{eq:bound_ham} and \eqref{eq:bound_parf} prove the conclusion of the Lemma.
%    \end{proof}
    
%    Observe that $||\bX||^2$ has a $\chi^2$-distribution with $N$ degrees of freedom and thus its fourth moment is a bounded sequence of $N\geq1$. From this, Lemma \ref{lem:exp_bound}, and (Lemma 3.1.8, Talagrand Mean) we obtain the following.
%    \begin{corollary}\label{cor:secmom_bound}
%        For all $t,\nu\in[0,1]$ and $N\geq1$ we have $\E\langle\frac{||\bx||^4}{N^2}\rangle_{t,\nu} \leq C$, with $C>0$ some constant.
%    \end{corollary}
    
%    Finally, we will prove that the bounded moment hypothesis of Varadhan's Lemma holds for $H_{N,1,1}(||\bx||^2)$ w.r.t. the standard gaussian density.
%    \begin{lemma}\label{lem:varad_hyp}
%        For every $\xi,\lambda,\lambda_* > 0$ and $N\geq1$, it holds that
%        \begin{equation*}
%            \frac{1}{N}\E \ln \left(\int_{\R^N}dG(\bx) e^{\xi N\left(-\frac{\lambda ||\bx||^4}{4 N^2} + \psi_\rho(\lambda||\bx||^4/N^2,\lambda_*)\right)}\right) \leq \frac{\xi}{4}\left(\Sigma_{max}+\sqrt{\lambda_*}-\frac{1}{\xi\sqrt{\lambda}}\right)^2.
%        \end{equation*}
%    \end{lemma}
%    \begin{proof}
%        Similarly to the way we got equation \eqref{eq:bound_ham}, it can be seen that
%        \begin{equation*}
%            \xi H_{N,1,1}(\bx) - \frac{||\bx||^2}{2} \leq N \frac{\xi}{4}\left(\Sigma_{max}+\sqrt{\lambda_*}-\frac{1}{\xi\sqrt{\lambda}}\right)^2.
%        \end{equation*}
%        From which the conclusion follows.
%    \end{proof}
    
%    We can now proceed with the proof of the main result of the section.
    
%    \begin{proof}[Proof of Proposition \ref{prop:fe_gaussian}]
%        We will first prove that $\lim_{N\to\infty}|f_{N,0,0} - f_{N,1,1}| = 0$. For this, observe that for all $t\in[0,1]$ we have
%        \begin{equation*}
%            \begin{split}
%                \left|\frac{d f_{N,t,0}}{dt}\right| & = \frac{\sqrt{\lambda\lambda_*}}{2 N}\left|\E\left(\langle({\bS}^T \bx)^2\rangle_{t,0} \left(1-\frac{||\bX||^2}{N}\right)\right)\right| \\
%                & \leq \frac{\sqrt{\lambda\lambda_*}}{2 N} \sqrt{\E\left\langle\frac{||\bx||^4}{N^2}\right\rangle_{t,0} \E\left(\frac{||\bX||^2}{N}-1\right)^2},
%            \end{split}
%        \end{equation*}
%        where we used Cauchy-Schwarz inequality. The right hand side of this last equation goes to $0$ because of Corollary \ref{cor:secmom_bound} and the fact that $||\bX||^2/N\xrightarrow{L^2}1$ (as $||\bX||^2$ is a $\chi^2$ r.v. with $N$ degrees of freedom). On the other hand, we have that
%        \begin{equation*}
%            \left|\frac{d f_{N,1,\nu}}{d\nu}\right| = \left|\E\left\langle \psi_\rho(\lambda||\bx||^4/N^2,\lambda_*) - \ln I_N\left(\frac{\sqrt{\lambda}||\bx||^2}{2N},\frac{\bY_1}{\sqrt{N}}\right) \right\rangle_{1,\nu}\right|
%        \end{equation*}
%        By Corollary \ref{cor:secmom_bound} and Chebyshev's inequality there exists a closed interval $F\subseteq\R$ and a constant $a > 0$ s.t. the probability of $\{||\bx||^2/N\not\in F\}$ is at most $a/N$. Furthermore, (Lemma 14 (1), Fourier View) implies that for all $\theta,\theta' \geq 0$ and $N\geq1$
%        \begin{equation}\label{eq:cont_si}
%            \left|\frac{1}{N} \ln I_N(\theta,\bY_1/\sqrt{N}) - \frac{1}{N} \ln I_N(\theta',\bY_1/\sqrt{N})\right| \leq L |\theta-\theta'|,
%        \end{equation}
%        where $L:= \max\{|\Sigma_{min}|,|\Sigma_{max}|\}+\sqrt{\lambda_*}$. This means that the family of functions of $\theta\in\R$ given by $\{N^{-1}\ln I_N(\theta,\bY_1/\sqrt{N}\}_{N\geq1}$ is uniformly equicontinuous. Then, because Theorem \ref{thm:spher_int} proves the pointwise convergence of this family, this convergence is uniform over compacts. If we define $A:=\{||\bx||^2/N\in F\}$, we then have
%        \begin{equation*}
%            \begin{split}
%                \left|\frac{d f_{N,t,0}}{dt}\right| \leq & \E\left\langle\left| \psi_\rho(\lambda||\bx||^4/N^2,\lambda_*) - \ln I_N\left(\frac{\sqrt{\lambda}||\bx||^2}{2N},\frac{\bY_1}{\sqrt{N}}\right) \right|\mathbb{I}_A\right\rangle_{1,\nu} \\
%                & \ \ \ \ \ + \E\left\langle\left| \psi_\rho(\lambda||\bx||^4/N^2,\lambda_*) - \ln I_N\left(\frac{\sqrt{\lambda}||\bx||^2}{2N},\frac{\bY_1}{\sqrt{N}}\right) \right|\mathbb{I}_{A^c}\right\rangle_{1,\nu}
%            \end{split}
%        \end{equation*}
%        By the uniform convergence of the spherical integral over compacts and a simple application of dominated convergence we have that the first term goes to zero. For the second one, note that \eqref{eq:cont_si} implies that $N^{-1}\ln I_N(\theta,\bY_1/\sqrt{N})$ and its limit are both Lipschitz with constant $L$ and thus this term is smaller or equal to
%        \begin{equation*}
%            \sqrt{\lambda}L\E\left\langle\frac{||\bx||^2}{N}\mathbb{I}_{A^c}\right\rangle_{1,\nu} \leq L\sqrt{\lambda\E\left\langle\frac{||\bx||^4}{N^2}\right\rangle_{1,\nu} \prob(A^c)}.
%        \end{equation*}
%        By Corollary \ref{cor:secmom_bound} we then conclude that this term goes to $0$. Thus, $\lim_{N\to\infty}|f_{N,0,0}-f_{N,1,1}| = 0$.
        
%        Because for a standard gaussian variable $g$, for $k < 1/2$, $\E\left(e^{k g^2}\right) = \frac{1}{\sqrt{1-2t}}$, by (Corollary 6.1.6, Large Deviations) we have that the law of $N^{-1} \sum_{i\leq N} \bx_i^2$ under a standard gaussian measure obeys a large deviation principle with good rate function
%        \begin{equation*}
%            I(x) = 
%            \begin{cases}
%                \frac{1}{2}(x-1-\ln x) & \mbox{if } x > 0 \\
%                \infty & o.w.
%            \end{cases}
%        \end{equation*}
%        Then, by Lemma \ref{lem:varad_hyp} and Varadhan's Lemma we have that
%        \begin{equation*}
%            \lim_{N\to\infty} f_{N,1,1} = \sup_{x\in\R_+} \left(\psi_\rho(\lambda x^2,\lambda_*) + \frac{1}{2}\left(\ln x + 1 - x - \frac{\lambda x^2}{2} \right)\right).
%        \end{equation*}
%        This together with the already proved fact that $\lim_{N\to\infty}|f_{N,0,0}-f_{N,1,1}| = 0$ finishes the proof.
%    \end{proof}

==> images/sections/09App_proofAMP.tex <==
\subsection{Auxiliary AMP}\label{subsec:auxAMP} The iterates of the auxiliary AMP are denoted by $\tilde{\bz}^t, \tilde{\bx}^t\in\mathbb R^N$, and they are computed as follows, for $t\ge 1$:
\begin{equation}\label{eq:auxAMP}
    \tilde{\bz}^t = \bZ \tilde{\bx}^t - \sum_{i=1}^t {\sf b}_{t, i}\tilde{\bx}^i, \quad \tilde{\bx}^{t+1} = \tilde{h}_{t+1}(\tilde{\bz}^1, \ldots, \tilde{\bz}^t, \hat{\bx}^1, \bX).
\end{equation}
The iteration is initialized with $\tilde{\bx}^1=\hat{\bx}^1$, where $\hat{\bx}^1$ is also the initialization of the true AMP (see \eqref{eq:AMPinit}). For $t\ge 1$, the functions $\tilde{h}_{t+1}:\mathbb R^{t+2}\to\mathbb R$ are applied component-wise, and they are recursively defined as
\begin{equation}\label{eq:deftildeh}
    \begin{split}
        \tilde{h}_{t+1}(z_1, \ldots, z_t, \hat{x}_1, x) = h_{t+1}\bigg(z_t+(\bB_t)_{t, 1} \hat{x}_1 &+ \sum_{i=2}^t (\bB_t)_{t, i}\tilde{h}_{i}\left(z_1, \ldots, z_{i-1}, \hat{x}_1, x\right)+\mu_t x\\
        &-\bar{\beta}_t \tilde{h}_{t-1}\left(z_1, \ldots, z_{t-2}, \hat{x}_1, x\right)\bigg).
    \end{split}
\end{equation}
Here, $h_{t+1}$ is the denoiser of the true AMP (see \eqref{eq:AMP}), and $(\mu_t, \bar{\beta}_t, \bB_t)$ come from the state evolution recursion of the true AMP: $\mu_1$ is given by \eqref{eq:SEinit}, and, for $t\ge 2$, $\mu_t$ is given by \eqref{eq:SEmu}; $\bar{\beta}_1=0$ and, for $t\ge 2$, $\bar{\beta}_t=\mathbb E[h_t'(x_{t-1})]$, where the law of $x_{t-1}$ is given by \eqref{eq:SElaws}; and $\bB_t$ is defined via \eqref{eq:defB}. It remains to discuss how to obtain the coefficients $\{{\sf b}_{t, i}\}_{i=1}^t$. Let us define the matrix $\bPhi_{t}\in\mathbb R^{t\times t}$ as
\begin{equation}\label{eq:defbPhi}
    \begin{split}
        (\bPhi_{t})_{i, j}&=0, \quad \mbox{ for }i\le j,\\
        (\bPhi_{t})_{i, j}&=\langle\partial_j \tilde{\bx}^i\rangle, \quad \mbox{ for }i> j,
    \end{split}
\end{equation}
where, for $j<i$, the vector $\langle\partial_j \tilde{\bx}_i\rangle\in \mathbb R^N$ denotes the partial derivative of $\tilde{h}_i:\mathbb R^{i+1}\to \mathbb R$ with respect to the $j$-th input (applied component-wise). Then, the vector $({\sf b}_{t, 1}, \ldots, {\sf b}_{t, t})$ is given by the last row of the matrix $\tilde{\bB}_{t}\in\mathbb R^{t\times t}$ defined as
\begin{equation}\label{eq:deftildeB}
    \tilde{\bB}_{t} = \sum_{j=0}^{t-1} \kappa_{j+1}\bPhi_{t}^j,
\end{equation}
where we recall that $\{\kappa_k\}_{k\ge 1}$ is the sequence of free cumulants associated to the matrix $\bZ$.

\subsection{State evolution of auxiliary AMP}\label{subsec:auxAMPSE} Using \cite[Theorem 2.3]{zhong2021approximate}, we first provide a state evolution result for the auxiliary AMP \eqref{eq:auxAMP}. In particular, we will show in Proposition \ref{prop:auxSE} that the joint empirical distribution of $(\tilde{\bz}^1, \ldots, \tilde{\bz}^t)$ converges to a $t$-dimensional Gaussian $\mathcal N(\bzero, \tilde{\bSigma}_t)$. 

The covariance matrices $\{\tilde{\bSigma}_t\}_{t\ge 1}$ are defined recursively, starting with $\tilde{\bSigma}_1=\bar{\kappa}_2\mathbb E[\hat{x}_1^2]$, where $\hat{x}_1$ is defined in \eqref{eq:AMPinit}. Given $\tilde{\bSigma}_t$, let 
\begin{equation}\label{eq:SElawsaux}
    \begin{split}
        (\tilde{z}_1&, \ldots, \tilde{z}_t)\sim\mathcal N(\bzero, \tilde{\bSigma}_t) \mbox{ and independent of }(X, \hat{x}_1),\\
         \tilde{x}_{s} &= \tilde{h}_{s}\left(\tilde{z}_1, \ldots, \tilde{z}_{s-1}, \hat{x}_{1}, X\right), \quad \mbox{ for } s\in \{2, \ldots, t+1\},
    \end{split}
\end{equation}
where $\tilde{h}_s$ is defined via \eqref{eq:deftildeh} and we set $\tilde{x}_{1}=\hat{x}_1$. Let $\tilde{\bPhi}_{t+1}, \tilde{\bDelta}_{t+1}\in\mathbb R^{(t+1)\times (t+1)}$ be symmetric matrices with entries given by  
\begin{equation}
    \begin{split}
        (\tilde{\bPhi}_{t+1})_{i, j}&=0, \quad \mbox{ for }i\le j,\qquad\qquad (\tilde{\bPhi}_{t+1})_{i, j}=\mathbb E[\partial_j \tilde{x}_i], \quad \mbox{ for }i> j,\\
        (\tilde{\bDelta}_{t+1})_{i, j} &= \mathbb E[\tilde{x}_{i}\,\tilde{x}_{j}], \quad 1\le i, j\le t+1,
    \end{split}
\end{equation}
where $\partial_j \tilde{x}_i$ denotes the partial derivative $\partial_{z_j} \tilde{h}_i(\tilde{z}_1, \ldots, \tilde{z}_{i-1}, \hat{x}_1, X)$. Then, we compute the covariance matrix $\tilde{\bSigma}_{t+1}$ as
\begin{equation}\label{eq:defSigmat}
    \tilde{\bSigma}_{t+1} = \sum_{j=0}^{2t}\bar{\kappa}_{j+2}\tilde{\bTheta}_{t+1}^{(j)}, \qquad \mbox{with}\quad\tilde{\bTheta}_{t+1}^{(j)} = \sum_{i=0}^j (\tilde{\bPhi}_{t+1})^i\tilde{\bDelta}_{t+1}(\tilde{\bPhi}_{t+1}^\intercal)^{j-i}.
\end{equation}
It can be verified that the $t\times t$ top left sub-matrix of $\tilde{\bSigma}_{t+1}$ is given by $\tilde{\bSigma}_t$. 


\begin{proposition}[State evolution for auxiliary AMP]
    Consider the auxiliary AMP in \eqref{eq:auxAMP} and the state evolution random variables defined in \eqref{eq:SElawsaux}. Let $\tilde{\psi}:\mathbb R^{2t+2} \to \mathbb R$ be any pseudo-Lipschitz functions of order 2. Then for each $t\ge 1$, we almost surely have
    \begin{align}
    & \lim_{N \to \infty}  \frac{1}{N} \sum_{i=1}^N  \tilde{\psi}\left((\tilde{\bz}^1)_i, \ldots, (\tilde{\bz}^t)_i, (\tilde{\bx}^1)_i, \ldots, (\tilde{\bx}^{t+1})_i, (\bX)_i\right) 
    = \E[ \tilde{\psi}(\tilde{z}_1, \ldots \tilde{z}_t, \tilde{x}_1, \ldots, \tilde{x}_{t+1}, X) ]. \label{eq:PL2aux}
    \end{align}
    Equivalently, as $N\to\infty$, almost surely:
    \begin{align*}
        %
        & (\tilde{\bz}^1, \ldots, \tilde{\bz}^{t}, \,  \tilde{\bx}^1, \ldots, \tilde{\bx}^{t+1}, \, \bX) \, \stackrel{\mathclap{W_2}}{\longrightarrow}  \,  (\tilde{z}_1, \ldots, \tilde{z}_t, \, \tilde{x}_1, \ldots, \tilde{x}_{t+1}, \, X).
    \end{align*}
    \label{prop:auxSE}
\end{proposition}
%
This proposition follows directly from Theorem 2.3 in \cite{zhong2021approximate}. In fact, the auxiliary AMP in \eqref{eq:auxAMP} is of the standard form for which that state evolution result applies. Furthermore, Assumption 2.1 holds because of the model assumptions on $\bZ$, Assumption 2.2(a) holds because $(\bX, \hat{\bx}^1)\stackrel{\mathclap{W_2}}{\longrightarrow} (X, \hat{x}_1)$ from \eqref{eq:AMPinit}, and Assumption 2.2(b) follows from the definition of $\tilde{h}_{t+1}$ in \eqref{eq:deftildeh} and our Assumption \textbf{(A1)} (see p.\pageref{assump:A1}).

\subsection{Proof of Theorem \ref{thm:AMP}}\label{subsec:proof}

We start by presenting a useful technical lemma. 

\begin{lemma}
    %
    \label{lem:lipderiv}
    Let $F : \mathbb R^t \to\mathbb R$ be a Lipschitz function, and let $\partial_k F$ denote its derivative with respect to the $k$-th argument, for $1 \le k \le t$. Assume that $\partial_k F$ is continuous almost everywhere in the $k$-th argument,  for each $k$. Let $(V_1^{(m)}, \ldots, V_t^{(m)})$  be a sequence of random vectors in $\mathbb R^t$ converging in distribution to the random vector $(V_1, \ldots,V_t)$ as $m \to \infty$. Furthermore, assume that the distribution of $(V_1, \ldots, V_t)$ is absolutely continuous with respect to the Lebesgue measure. Then, 
    \begin{equation}
         \lim_{m \to \infty}  \mathbb E[ \partial_k F(V_1^{(m)}, \ldots, V_t^{(m)})] = \mathbb E[ \partial_k F(V_1, \ldots, V_t) ], \qquad 1 \le k \le t.
    \end{equation}
\end{lemma}
The result was proved for $t=2$ in \cite[Lemma 6]{bayati2011dynamics}. The proof for $t > 2$ is essentially the same; see also \cite[Lemma 7.14]{feng2021unifying}.

At this point, we are ready to give the proof of Theorem \ref{thm:AMP}.

\begin{proof}[Proof of Theorem \ref{thm:AMP}]
The first step is to show the equivalence between the state evolution for the true AMP and the corresponding one for the auxiliary AMP. In particular, we prove that, for $t\ge 1$,
\begin{equation}\label{eq:equivSE}
    (\tilde{z}_1, \ldots, \tilde{z}_{t}) \stackrel{\rm d}{=} (z_1, \ldots, z_t) ,
\end{equation}
where the random variables on the left are defined in \eqref{eq:SElawsaux}, and the random variables on the right are defined in \eqref{eq:SElaws}. As $(\tilde{z}_1, \ldots, \tilde{z}_t)\sim\mathcal N(\bzero, \tilde{\bSigma}_t)$ and $(z_1, \ldots, z_t)\sim\mathcal N(\bzero, \bSigma_t)$, \eqref{eq:equivSE} is readily implied by 
\begin{equation}\label{eq:eqS}
    \tilde{\bSigma}_t=\bSigma_t, \qquad \mbox{ for all }t\ge 1.
\end{equation}
We now show that \eqref{eq:eqS} holds by induction. The base case ($t=1$) follows from the definitions of $\tilde{\bSigma}_1, \bSigma_1$. Towards induction, assume that $\tilde{\bSigma}_t=\bSigma_t$ for some $t\ge 1$. By comparing the definition of $\hat{x}_s$ in \eqref{eq:SElaws} with the definition of $\tilde{x}_s$ in \eqref{eq:SElawsaux} and by using the choice of $\tilde{h}_s$ in \eqref{eq:deftildeh} (for $s\in\{2, \ldots, t+1\}$), we readily obtain that $\Delta_{t+1}=\tilde{\Delta}_{t+1}$ and $\bar{\bPhi}_{t+1}=\tilde{\bPhi}_{t+1}$. Hence, by using \eqref{eq:defSigma} and \eqref{eq:defSigmat}, we have that $\tilde{\bSigma}_{t+1}=\bSigma_{t+1}$ and the proof of \eqref{eq:eqS} is complete. 

The second step is to show that, for any pseudo-Lipschitz function  $\psi: \mathbb R^{2t+2} \to \mathbb R$ of order 2, the following limit holds almost surely for $t \ge 1$: 
\begin{equation}\label{eq:PLsecondstep}
    \begin{split}
        \lim_{N \to \infty}  \Bigg\vert 
        \frac{1}{N}& \sum_{i=1}^{N} \psi\left((\bx^1)_i, \ldots, (\bx^t)_i, \,  (\hat{\bx}^1)_i, \ldots, (\hat{\bx}^{t+1})_i, \, (\bX)_i\right)
        \\
        & -   \frac{1}{N} \sum_{i=1}^{N} \psi\left((\bu^1)_i, \ldots, (\bu^t)_i, \,  (\tilde{\bx}^1)_i, \ldots, (\tilde{\bx}^{t+1})_i, \, (\bX)_i\right)  \Bigg \vert =0,
    \end{split}
\end{equation}
where, we have defined for $s\in \{1, \ldots, t\}$,
\begin{equation}\label{eq:defu}
    \bu^s = \tilde{\bz}^s+(\bB_s)_{s, 1} \tilde{\bx}^1 + \sum_{i=2}^s (\bB_s)_{s, i}\tilde{\bx}^i+\mu_s \bX-\bar{\beta}_s \tilde{\bx}^{s-1}.
\end{equation}
From here till the end of the argument, we use $C$ to denote a generic positive constant, which can change from line to line and is independent of $N$. All the limits hold almost surely, thus this is not explicitly stated every time. Since $\psi$ is pseudo-Lipschitz, we have
\begin{equation}
    \begin{split}
         \Bigg\vert 
         &\frac{1}{N} \sum_{i=1}^{N} \psi\left((\bx^1)_i, \ldots, (\bx^t)_i, \,  (\hat{\bx}^1)_i, \ldots, (\hat{\bx}^{t+1})_i, \, (\bX)_i\right)
        \\
        & \hspace{3em}-   \frac{1}{N} \sum_{i=1}^{N} \psi\left((\bu^1)_i, \ldots, (\bu^t)_i, \,  (\tilde{\bx}^1)_i, \ldots, (\tilde{\bx}^{t+1})_i, \, (\bX)_i\right)  \Bigg \vert\\
        & \le \frac{C}{N} \sum_{i=1}^{N} \left( 1+ |(\bX)_i| +2|(\hat{\bx}^1)_i| +\sum_{\ell=1}^t \Big( |(\bx^\ell)_i| +|(\bu^{\ell})_i|+ |(\hat{\bx}^{\ell+1})_i|  + |(\tilde{\bx}^{\ell+1})_i|  \Big) \right) \\
        &\hspace{3em} \cdot \left( \sum_{\ell=1}^t  \left(|(\bx^\ell)_i - (\bu^\ell)_i |^2  +  |(\hat{\bx}^{\ell+1})_i - (\tilde{\bx}^{\ell+1})_i |^2\right) \right)^{1/2} \\
        & \leq C(4t+3)\left[ 1 + \frac{\| \bX \|^2}{N} +  
        \sum_{\ell=1}^t \Big( \frac{\|\bx^\ell \|^2}{N} + \frac{\|\bu^\ell \|^2}{N} + \frac{\| \hat{\bx}^{\ell+1} \|^2}{N} + 
        \frac{\| \tilde{\bx}^{\ell+1} \|^2}{N} \Big) \right]^{1/2} \\
        &\hspace{3em}\cdot \left( \sum_{\ell=1}^t \left(\frac{\| \bx^\ell - \bu^{\ell}\|^2}{N} + \frac{\|\hat{\bx}^{\ell+1} - \tilde{\bx}^{\ell+1}\|^2}{N} \, \right)\right)^{1/2},  \label{eq:xz_diff}
    \end{split}
\end{equation}
where the last step uses Cauchy-Schwarz inequality (twice). We will inductively show that as $N \to \infty$: \emph{(i)} each of the terms in the last line of \eqref{eq:xz_diff} converges to zero, and \emph{(ii)} the terms within the square brackets in \eqref{eq:xz_diff} all converge to finite, deterministic limits. 

\noindent \underline{Base case ($t=1$).} We have that
\begin{equation}\label{eq:b1man}
    \begin{split}
        \bx^1-\bu^1 &= \bY\hat{\bx}^1-\tilde{\bz}^1-(\bB_1)_{1, 1}\tilde{\bx}^1-\mu_1\bX \\
        &=\bZ\hat{\bx}^1+\sqrt{\lambda}\frac{\langle \bX, \hat{\bx}^1\rangle}{N}\bX-\bZ\tilde{\bx}^1+{\sf b}_{1, 1}\tilde{\bx}^1-(\bB_1)_{1, 1}\tilde{\bx}^1-\mu_1\bX\\
        &=\sqrt{\lambda}\frac{\langle \bX, \hat{\bx}^1\rangle}{N}\bX+{\sf b}_{1, 1}\tilde{\bx}^1-(\bB_1)_{1, 1}\tilde{\bx}^1-\mu_1\bX,
    \end{split}
\end{equation}
where the first equality uses \eqref{eq:AMP} and \eqref{eq:defu}, the second equality uses \eqref{eq:spikedmodel} and \eqref{eq:auxAMP}, and the third equality uses that $\tilde{\bx}^1=\hat{\bx}^1$. Hence, by triangle inequality,
\begin{equation}\label{eq:base1}
    \begin{split}
        \frac{\|\bx^1-\bu^1\|^2}{N}&\le 2\left(\sqrt{\lambda}\frac{\langle \bX, \hat{\bx}^1\rangle}{N}-\mu_1\right)^2\frac{\|\bX\|^2}{N}+2\left({\sf b}_{1, 1}-(\bB_1)_{1, 1}\right)^2\frac{\|\tilde{\bx}^1\|^2}{N}\\
        &\le C\left(\left(\sqrt{\lambda}\frac{\langle \bX, \hat{\bx}^1\rangle}{N}-\mu_1\right)^2+\left({\sf b}_{1, 1}-(\bB_1)_{1, 1}\right)^2\right),
    \end{split}
\end{equation}
where the last inequality uses that $\tilde{\bx}^1=\hat{\bx}^1$ and that $(\bX, \hat{\bx}^1)$ converge in $W_2$ to random variables with finite second moments. By using \eqref{eq:AMPinit} and recalling that $\mu_1=\sqrt{\lambda}\epsilon$ (cf. \eqref{eq:SEinit}), we have 
\begin{equation}\label{eq:base2}
    \lim_{N\to\infty}\sqrt{\lambda}\frac{\langle \bX, \hat{\bx}^1\rangle}{N}=\sqrt{\lambda}\epsilon=\mu_1.
\end{equation}
Furthermore, note that  $(\bB_1)_{1, 1}=\bar{\kappa}_1$ (cf. \eqref{eq:SEinit}) and ${\sf b}_{1, 1}=\kappa_1$ (cf. \eqref{eq:deftildeB}) and, by the model assumptions, $\kappa_1\to\bar{\kappa}_1$, as $N\to\infty$. Hence, ${\sf b}_{1, 1}\to (\bB_1)_{1, 1}$ and, by combining this observation with \eqref{eq:base1} and \eqref{eq:base2}, we obtain that 
\begin{equation}\label{eq:it1}
    \lim_{N\to\infty}\frac{\|\bx^1-\bu^1\|^2}{N}=0.
\end{equation}
Next, by expressing $\hat{\bx}^2$ via \eqref{eq:AMP} and $\tilde{\bx}^2$ via \eqref{eq:auxAMP}, \eqref{eq:deftildeh} and \eqref{eq:defu}, we have that
\begin{equation}
    \hat{\bx}^2-\tilde{\bx}^2=h_2(\bx^1)-h_2(\bu^1).
\end{equation}
Thus, as $h_2$ is Lipschitz, \eqref{eq:it1} immediately implies that
\begin{equation}
    \lim_{N\to\infty}\frac{\|\hat{\bx}^2-\tilde{\bx}^2\|^2}{N}=0.
\end{equation}
An application of the triangle inequality gives that, for any $i\ge 1$,
\begin{equation}\label{eq:tr1}
    \begin{split}
        \|\bu^i\|- \|\bx^i-\bu^i\|&\le \|\bx^i\|\le \|\bu^i\|+ \|\bx^i-\bu^i\|, \\
         \|\tilde{\bx}^{i+1}\|- \|\hat{\bx}^{i+1}-\tilde{\bx}^{i+1}\| &\le \|\hat{\bx}^{i+1}\|\le \|\tilde{\bx}^{i+1}\|+ \|\hat{\bx}^{i+1}-\tilde{\bx}^{i+1}\|.
    \end{split}
\end{equation}
Thus, by using \eqref{eq:tr1} with $i=1$ and Proposition \ref{prop:auxSE}, we obtain that
\begin{equation}
    \begin{split}
        &\lim_{N\to\infty}\frac{\|\bx^1\|^2}{N}=\lim_{N\to\infty}\frac{\|\bu^1\|^2}{N}=\mathbb E[(\tilde{z}_1+(\bB_1)_{1, 1}\hat{x}_1+\mu_1 X)^2], \\
        &\lim_{N\to\infty}\frac{\|\hat{\bx}^2\|^2}{N}=\lim_{N\to\infty}\frac{\|\tilde{\bx}^2\|^2}{N}=\mathbb E[(\tilde{x}_2)^2],
    \end{split}
\end{equation}
which concludes the base step.

\noindent \underline{Induction step.} Assume towards induction that
\begin{align}
    &\lim_{N\to\infty}\frac{\|\bx^{j}-\bu^{j}\|^2}{N}=0,\quad \mbox{ for }j\in\{1, \ldots, t\},\label{eq:ind0}\\
    &\lim_{N\to\infty}\frac{\|\hat{\bx}^{j}-\tilde{\bx}^{j}\|^2}{N}=0,\quad \mbox{ for }j\in\{2, \ldots, t+1\},\label{eq:ind1}\\
    &\lim_{N\to\infty}\frac{\|\bx^{j}\|^2}{N}=\lim_{N\to\infty}\frac{\|\bu^{j}\|^2}{N}=\mathbb E\Bigg[\left(\tilde{z}_{j}+(\bB_{j})_{j, 1}\hat{x}_1+\sum_{i=2}^{j}(\bB_{j})_{j, i}\tilde{x}_i+\mu_{j}X-\bar{\beta}_{j}\tilde{x}_{j-1}\right)^2\Bigg], \,\,\, \mbox{ for }j\in\{1, \ldots, t\},\label{eq:ind1bis}\\
    &\lim_{N\to\infty}\frac{\|\hat{\bx}^{j}\|^2}{N}=\lim_{N\to\infty}\frac{\|\tilde{\bx}^{j}\|^2}{N}=\mathbb E[\tilde{x}_j^2], \quad \mbox{ for }j\in\{2, \ldots, t+1\}.\label{eq:ind2}
\end{align}
We now show that the following limits hold:
\begin{align}
    &\lim_{N\to\infty}\frac{\|\bx^{t+1}-\bu^{t+1}\|^2}{N}=0,\label{eq:indres1}\\
    &\lim_{N\to\infty}\frac{\|\hat{\bx}^{t+2}-\tilde{\bx}^{t+2}\|^2}{N}=0,\label{eq:indres2}\\
    &\lim_{N\to\infty}\frac{\|\bx^{t+1}\|^2}{N}=\lim_{N\to\infty}\frac{\|\bu^{t+1}\|^2}{N}\nonumber\\
    &\hspace{5.5em}=\mathbb E\Bigg[\left(\tilde{z}_{t+1}+(\bB_{t+1})_{t+1, 1}\hat{x}_1+\sum_{i=2}^{t+1}(\bB_{t+1})_{t+1, i}\tilde{x}_i+\mu_{t+1}X-\bar{\beta}_{t+1}\tilde{x}_{t}\right)^2\Bigg],\label{eq:indres3}\\
    &\lim_{N\to\infty}\frac{\|\hat{\bx}^{t+2}\|^2}{N}=\lim_{N\to\infty}\frac{\|\tilde{\bx}^{t+2}\|^2}{N}=\mathbb E[\tilde{x}_{t+2}^2].\label{eq:indres4}
\end{align}
By doing so, we will have proved also the induction step and consequently that \eqref{eq:PLsecondstep} holds. 

Using similar passages as in \eqref{eq:b1man}, we obtain
\begin{equation}
    \begin{split}
        \bx^{t+1}-\bu^{t+1} &= \bY\hat{\bx}^{t+1} - \beta_{t+1}\hat{\bx}^{t}-\tilde{\bz}^{t+1}-(\bB_{t+1})_{t+1, 1} \tilde{\bx}^1 - \sum_{i=2}^{t+1} (\bB_{t+1})_{t+1, i}\tilde{\bx}^i-\mu_{t+1} \bX+\bar{\beta}_{t+1} \tilde{\bx}^{t}\\
        &= \bZ\hat{\bx}^{t+1}+\sqrt{\lambda}\frac{\langle \bX, \hat{\bx}^{t+1}\rangle}{N}\bX - \beta_{t+1}\hat{\bx}^{t}-\bZ \tilde{\bx}^{t+1} + \sum_{i=1}^{t+1} {\sf b}_{t+1, i}\tilde{\bx}^i-(\bB_{t+1})_{t+1, 1} \tilde{\bx}^1 \\
        &\hspace{17em}- \sum_{i=2}^{t+1} (\bB_{t+1})_{t+1, i}\tilde{\bx}^i-\mu_{t+1} \bX+\bar{\beta}_{t+1} \tilde{\bx}^{t}.
    \end{split}
\end{equation}
Hence, by triangle inequality,
\begin{equation}\label{eq:decT}
    \begin{split}
        \frac{\|\bx^{t+1}-\bu^{t+1}\|^2}{N}&\le C\bigg(\frac{\|\bZ\hat{\bx}^{t+1}-\bZ\tilde{\bx}^{t+1}\|^2}{N}+\left(\sqrt{\lambda}\frac{\langle \bX, \hat{\bx}^{t+1}\rangle}{N}-\mu_{t+1}\right)^2\frac{\|\bX\|^2}{N}\\
        &\hspace{2em}+\sum_{i=1}^{t+1}\left({\sf b}_{t+1, i}-(\bB_{t+1})_{t+1, i}\right)^2\frac{\|\tilde{\bx}^i\|^2}{N}+(\bar{\beta}_{t+1}-\beta_{t+1})^2\frac{\|\hat{\bx}^t\|^2}{N}+\bar{\beta}_{t+1}\frac{\|\tilde{\bx}^t-\hat{\bx}^t\|^2}{N}\bigg)\\
        &:= C(T_1+T_2+T_3+T_4+T_5).
    \end{split}
\end{equation}
Consider the first term. Since $\|\bZ\|_{\rm op}\le C$, the induction hypothesis \eqref{eq:ind1} implies that $T_1\to 0$ as $N\to\infty$.

Consider the second term. The following chain of equalities holds:
\begin{equation}\label{eq:T2}
    \lim_{N\to \infty}\sqrt{\lambda}\frac{\langle \bX, \hat{\bx}^{t+1}\rangle}{N}=\lim_{N\to \infty}\sqrt{\lambda}\frac{\langle \bX, \tilde{\bx}^{t+1}\rangle}{N}=\sqrt{\lambda} \mathbb E[X\,\tilde{x}_{t+1}]=\sqrt{\lambda} \mathbb E[X\,\hat{x}_{t+1}]=\mu_{t+1}.
\end{equation}
Here, the first equality uses \eqref{eq:ind1} together with the fact that $\|\bX\|^2/ N$ is upper bounded by a constant independent of $N$; the second equality follows from Proposition \ref{prop:auxSE}; the third equality uses \eqref{eq:equivSE} and the definitions of $\hat{x}_{t+1}$ and $\tilde{x}_{t+1}$ in \eqref{eq:SElaws} and \eqref{eq:SElawsaux}, respectively; and the fourth equality uses the definition of $\mu_{t+1}$ in \eqref{eq:SEmu}. Finally, using \eqref{eq:T2} and again that $\|\bX\|^2/ N$ is upper bounded by a constant independent of $N$ gives that $T_2\to 0$ as $N\to\infty$.

Consider the third term. The following chain of equalities holds, for $1\le j<i\le (t+1)$,
\begin{equation}\label{eq:T3}
    \lim_{N\to \infty} (\bPhi_{t+1})_{i, j} =\lim_{N\to\infty}\langle\partial_j \tilde{\bx}^i\rangle =\mathbb E[\partial_j\tilde{x}_i] = \mathbb E[\partial_j\hat{x}_i] = (\bar{\bPhi}_{t+1})_{i, j}
\end{equation}
Here, the first equality uses the definition \eqref{eq:defbPhi}; the second equality follows from Lemma \ref{lem:lipderiv}, as $\tilde{\bx}^i=\tilde{h}_i(\tilde{\bz}^1, \ldots, \tilde{\bz}^{i-1}, \hat{\bx}^1, \bX)$ converges in $W_2$ (and therefore in distribution) to $\tilde{x}_i=\tilde{h}_i(\tilde{z}_1, \ldots, \tilde{z}_{i-1}, \hat{x}_1, X)$ and $h_i$ satisfies the assumptions in \textbf{(A1)}; the third equality uses \eqref{eq:equivSE} and the definitions of $\hat{x}_{i}$ and $\tilde{x}_{i}$ in \eqref{eq:SElaws} and \eqref{eq:SElawsaux}, respectively;  and the fourth equality uses the definition of $(\bar{\bPhi}_{t+1})_{i, j}$ in \eqref{eq:defbPhibar}. By the model assumptions, as $N\to\infty$, $\kappa_j\to\bar{\kappa}_j$ for all $j$. Thus, by combining \eqref{eq:T3} with the definitions of $\bB_{t+1}$ and $\tilde{\bB}_{t+1}$ in \eqref{eq:defB} and \eqref{eq:deftildeB}, respectively, we conclude that, as $N\to\infty$, ${\sf b}_{t+1, i}\to(\bB_{t+1})_{t+1, i}$ for $i\in \{1, \ldots, t+1\}$. By using the induction hypothesis \eqref{eq:ind2}, which shows that $\|\tilde{\bx}^i\|^2/N$ converges to a finite limit, we conclude that $T_3\to 0$ as $N\to\infty$.

Consider the fourth term. By using the induction hypothesis \eqref{eq:ind0} and \eqref{eq:ind1bis}, together with \eqref{eq:xz_diff}, we obtain that $\bx^t$ and $\bu^t$ have the same $W_2$ limit given by Proposition \ref{prop:auxSE}, namely,
\begin{equation*}
    \bx^t \, \stackrel{\mathclap{W_2}}{\longrightarrow}  \,    \tilde{z}_{t}+(\bB_{t})_{t, 1}\hat{x}_1+\sum_{i=2}^{t}(\bB_{t})_{t, i}\tilde{x}_i+\mu_{t}X-\bar{\beta}_{t}\tilde{x}_{t-1}.
\end{equation*}
Thus, by recalling that $\beta_{t+1} = \langle h_{t+1}'(\bx^t)\rangle$, an application of Lemma \ref{lem:lipderiv} gives that 
\begin{equation}\label{eq:T4}
    \lim_{N\to\infty}\beta_{t+1} = \mathbb E\bigg[h_{t+1}'\bigg(\tilde{z}_t+(\bB_t)_{t, 1} \hat{x}_1 + \sum_{i=2}^t (\bB_t)_{t, i}\tilde{x}_{i}+\mu_t X-\bar{\beta}_t \tilde{x}_{t-1}\bigg)\bigg].
\end{equation}
Furthermore, by using \eqref{eq:equivSE} and recalling the definition of $\bar{\beta}_{t+1}$, we have that the RHS of \eqref{eq:T4} is equal to  $\bar{\beta}_{t+1}$. Hence, by using the induction hypothesis \eqref{eq:ind2}, we obtain that $T_4\to 0$ as $N\to\infty$. Finally, by using the induction hypothesis \eqref{eq:ind1}, we 
conclude that also $T_5\to 0$ as $N\to\infty$.

As $T_i\to 0$ for $i\in \{1, \ldots, 5\}$, \eqref{eq:decT} implies that \eqref{eq:indres1} holds. Next, as $h_{t+1}$ is Lipschitz, \eqref{eq:indres1} immediately implies \eqref{eq:indres2}. Then, by using \eqref{eq:tr1} with $i=t+1$ and Proposition \ref{prop:auxSE}, we obtain that \eqref{eq:indres3} and \eqref{eq:indres4} hold, thus concluding the inductive proof. The result we have just proved by induction, combined with \eqref{eq:xz_diff}, gives that \eqref{eq:PLsecondstep} holds. 

Another application of Proposition \ref{prop:auxSE}, together with \eqref{eq:PLsecondstep}, gives that
\begin{equation}\label{eq:fin1}
    \begin{split}
         \lim_{N \to \infty}  
         \frac{1}{N}& \sum_{i=1}^{N} \psi\left((\bx^1)_i, \ldots, (\bx^t)_i, \,  (\hat{\bx}^1)_i, \ldots, (\hat{\bx}^{t+1})_i, \, (\bX)_i\right) =\mathbb E [ \psi(u_1, \ldots, u_t, \tilde{x}_1, \ldots, \tilde{x}_{t+1}, X) ],
     \end{split}
\end{equation}
where we have defined for $s\in \{1, \ldots, t\}$,
\begin{equation}
    u_s = \tilde{z}_s+(\bB_s)_{s, 1} \tilde{x}_1 + \sum_{i=2}^s (\bB_s)_{s, i}\tilde{x}_i+\mu_s X-\bar{\beta}_s \tilde{x}_{s-1}.
\end{equation}
Finally, by using \eqref{eq:equivSE}, we have that
\begin{equation}\label{eq:fin2}
    \mathbb E [ \psi(u_1, \ldots, u_t, \tilde{x}_1, \ldots, \tilde{x}_{t+1}, X) ] = \mathbb E [ \psi(x_1, \ldots, x_t, \hat{x}_1, \ldots, \hat{x}_{t+1}, X) ].
\end{equation}
By combining \eqref{eq:fin1} and \eqref{eq:fin2}, we obtain that the desired result \eqref{eq:PL2_main_resultx} holds, which concludes the proof. 


\end{proof}

==> sections/08App_proofAMP_old.tex <==
\subsection{Auxiliary AMP}\label{subsec:auxAMP} The iterates of the auxiliary AMP are denoted by $\tilde{\bz}^t, \tilde{\bx}^t\in\mathbb R^N$, and they are computed as follows, for $t\ge 1$:
\begin{equation}\label{eq:auxAMP}
    \tilde{\bz}^t = \bZ \tilde{\bx}^t - \sum_{i=1}^t {\sf b}_{t, i}\tilde{\bx}^i, \quad \tilde{\bx}^{t+1} = \tilde{h}_{t+1}(\tilde{\bz}^1, \ldots, \tilde{\bz}^t, \hat{\bx}^1, \bX).
\end{equation}
The iteration is initialized with $\tilde{\bx}^1=\hat{\bx}^1$, where $\hat{\bx}^1$ is also the initialization of the true AMP (see \eqref{eq:AMPinit}). For $t\ge 1$, the functions $\tilde{h}_{t+1}:\mathbb R^{t+2}\to\mathbb R$ are applied component-wise, and they are recursively defined as
\begin{equation}\label{eq:deftildeh}
    \begin{split}
        \tilde{h}_{t+1}(z_1, \ldots, z_t, \hat{x}_1, x) = h_{t+1}\bigg(z_t+(\bB_t)_{t, 1} \hat{x}_1 &+ \sum_{i=2}^t (\bB_t)_{t, i}\tilde{h}_{i}\left(z_1, \ldots, z_{i-1}, \hat{x}_1, x\right)+\mu_t x\\
        &-\bar{\beta}_t \tilde{h}_{t-1}\left(z_1, \ldots, z_{t-2}, \hat{x}_1, x\right)\bigg).
    \end{split}
\end{equation}
Here, $h_{t+1}$ is the denoiser of the true AMP (see \eqref{eq:AMP}), and $(\mu_t, \bar{\beta}_t, \bB_t)$ come from the state evolution recursion of the true AMP: $\mu_1$ is given by \eqref{eq:SEinit}, and, for $t\ge 2$, $\mu_t$ is given by \eqref{eq:SEmu}; $\bar{\beta}_1=0$ and, for $t\ge 2$, $\bar{\beta}_t=\mathbb E[h_t'(x_{t-1})]$, where the law of $x_{t-1}$ is given by \eqref{eq:SElaws}; and $\bB_t$ is defined via \eqref{eq:defB}. It remains to discuss how to obtain the coefficients $\{{\sf b}_{t, i}\}_{i=1}^t$. Let us define the matrix $\bPhi_{t}\in\mathbb R^{t\times t}$ as
\begin{equation}\label{eq:defbPhi}
    \begin{split}
        (\bPhi_{t})_{i, j}&=0, \quad \mbox{ for }i\le j,\\
        (\bPhi_{t})_{i, j}&=\langle\partial_j \tilde{\bx}^i\rangle, \quad \mbox{ for }i> j,
    \end{split}
\end{equation}
where, for $j<i$, the vector $\langle\partial_j \tilde{\bx}_i\rangle\in \mathbb R^N$ denotes the partial derivative of $\tilde{h}_i:\mathbb R^{i+1}\to \mathbb R$ with respect to the $j$-th input (applied component-wise). Then, the vector $({\sf b}_{t, 1}, \ldots, {\sf b}_{t, t})$ is given by the last row of the matrix $\tilde{\bB}_{t}\in\mathbb R^{t\times t}$ defined as
\begin{equation}\label{eq:deftildeB}
    \tilde{\bB}_{t} = \sum_{j=0}^{t-1} \kappa_{j+1}\bPhi_{t}^j,
\end{equation}
where we recall that $\{\kappa_k\}_{k\ge 1}$ is the sequence of free cumulants associated to the matrix $\bZ$.

\subsection{State evolution of auxiliary AMP}\label{subsec:auxAMPSE} Using \cite[Theorem 2.3]{zhong2021approximate}, we first provide a state evolution result for the auxiliary AMP \eqref{eq:auxAMP}. In particular, we will show in Proposition \ref{prop:auxSE} that the joint empirical distribution of $(\tilde{\bz}^1, \ldots, \tilde{\bz}^t)$ converges to a $t$-dimensional Gaussian $\mathcal N(\bzero, \tilde{\bSigma}_t)$. 

The covariance matrices $\{\tilde{\bSigma}_t\}_{t\ge 1}$ are defined recursively, starting with $\tilde{\bSigma}_1=\bar{\kappa}_2\mathbb E[\hat{x}_1^2]$, where $\hat{x}_1$ is defined in \eqref{eq:AMPinit}. Given $\tilde{\bSigma}_t$, let 
\begin{equation}\label{eq:SElawsaux}
    \begin{split}
        (\tilde{z}_1&, \ldots, \tilde{z}_t)\sim\mathcal N(\bzero, \tilde{\bSigma}_t) \mbox{ and independent of }(X, \hat{x}_1),\\
         \tilde{x}_{s} &= \tilde{h}_{s}\left(\tilde{z}_1, \ldots, \tilde{z}_{s-1}, \hat{x}_{1}, X\right), \quad \mbox{ for } s\in \{2, \ldots, t+1\},
    \end{split}
\end{equation}
where $\tilde{h}_s$ is defined via \eqref{eq:deftildeh} and we set $\tilde{x}_{1}=\hat{x}_1$. Let $\tilde{\bPhi}_{t+1}, \tilde{\bDelta}_{t+1}\in\mathbb R^{(t+1)\times (t+1)}$ be symmetric matrices with entries given by  
\begin{equation}
    \begin{split}
        (\tilde{\bPhi}_{t+1})_{i, j}&=0, \quad \mbox{ for }i\le j,\qquad\qquad (\tilde{\bPhi}_{t+1})_{i, j}=\mathbb E[\partial_j \tilde{x}_i], \quad \mbox{ for }i> j,\\
        (\tilde{\bDelta}_{t+1})_{i, j} &= \mathbb E[\tilde{x}_{i}\,\tilde{x}_{j}], \quad 1\le i, j\le t+1,
    \end{split}
\end{equation}
where $\partial_j \tilde{x}_i$ denotes the partial derivative $\partial_{z_j} \tilde{h}_i(\tilde{z}_1, \ldots, \tilde{z}_{i-1}, \hat{x}_1, X)$. Then, we compute the covariance matrix $\tilde{\bSigma}_{t+1}$ as
\begin{equation}\label{eq:defSigmat}
    \tilde{\bSigma}_{t+1} = \sum_{j=0}^{2t}\bar{\kappa}_{j+2}\tilde{\bTheta}_{t+1}^{(j)}, \qquad \mbox{with}\quad\tilde{\bTheta}_{t+1}^{(j)} = \sum_{i=0}^j (\tilde{\bPhi}_{t+1})^i\tilde{\bDelta}_{t+1}(\tilde{\bPhi}_{t+1}^\intercal)^{j-i}.
\end{equation}
It can be verified that the $t\times t$ top left sub-matrix of $\tilde{\bSigma}_{t+1}$ is given by $\tilde{\bSigma}_t$. 


\begin{proposition}[State evolution for auxiliary AMP]
    Consider the auxiliary AMP in \eqref{eq:auxAMP} and the state evolution random variables defined in \eqref{eq:SElawsaux}. Let $\tilde{\psi}:\mathbb R^{2t+2} \to \mathbb R$ be any pseudo-Lipschitz functions of order 2. Then for each $t\ge 1$, we almost surely have
    \begin{align}
    & \lim_{N \to \infty}  \frac{1}{N} \sum_{i=1}^N  \tilde{\psi}\left((\tilde{\bz}^1)_i, \ldots, (\tilde{\bz}^t)_i, (\tilde{\bx}^1)_i, \ldots, (\tilde{\bx}^{t+1})_i, (\bX)_i\right) 
    = \E[ \tilde{\psi}(\tilde{z}_1, \ldots \tilde{z}_t, \tilde{x}_1, \ldots, \tilde{x}_{t+1}, X) ]. \label{eq:PL2aux}
    \end{align}
    Equivalently, as $N\to\infty$, almost surely:
    \begin{align*}
        %
        & (\tilde{\bz}^1, \ldots, \tilde{\bz}^{t}, \,  \tilde{\bx}^1, \ldots, \tilde{\bx}^{t+1}, \, \bX) \, \stackrel{\mathclap{W_2}}{\longrightarrow}  \,  (\tilde{z}_1, \ldots, \tilde{z}_t, \, \tilde{x}_1, \ldots, \tilde{x}_{t+1}, \, X).
    \end{align*}
    \label{prop:auxSE}
\end{proposition}
%
This proposition follows directly from Theorem 2.3 in \cite{zhong2021approximate}. In fact, the auxiliary AMP in \eqref{eq:auxAMP} is of the standard form for which that state evolution result applies. Furthermore, Assumption 2.1 holds because of the model assumptions on $\bZ$, Assumption 2.2(a) holds because $(\bX, \hat{\bx}^1)\stackrel{\mathclap{W_2}}{\longrightarrow} (X, \hat{x}_1)$ from \eqref{eq:AMPinit}, and Assumption 2.2(b) follows from the definition of $\tilde{h}_{t+1}$ in \eqref{eq:deftildeh} and Assumption \ref{ass:AMP}.

\subsection{Proof of Theorem \ref{thm:AMP}}\label{subsec:proof}

We start by presenting a useful technical lemma. 

\begin{lemma}
    %
    \label{lem:lipderiv}
    Let $F : \mathbb R^t \to\mathbb R$ be a Lipschitz function, and let $\partial_k F$ denote its derivative with respect to the $k$-th argument, for $1 \le k \le t$. Assume that $\partial_k F$ is continuous almost everywhere in the $k$-th argument,  for each $k$. Let $(V_1^{(m)}, \ldots, V_t^{(m)})$  be a sequence of random vectors in $\mathbb R^t$ converging in distribution to the random vector $(V_1, \ldots,V_t)$ as $m \to \infty$. Furthermore, assume that the distribution of $(V_1, \ldots, V_t)$ is absolutely continuous with respect to the Lebesgue measure. Then, 
    \begin{equation}
         \lim_{m \to \infty}  \mathbb E[ \partial_k F(V_1^{(m)}, \ldots, V_t^{(m)})] = \mathbb E[ \partial_k F(V_1, \ldots, V_t) ], \qquad 1 \le k \le t.
    \end{equation}
\end{lemma}
The result was proved for $t=2$ in \cite[Lemma 6]{bayati2011dynamics}. The proof for $t > 2$ is essentially the same; see also \cite[Lemma 7.14]{feng2021unifying}.

At this point, we are ready to give the proof of Theorem \ref{thm:AMP}.

\begin{proof}[Proof of Theorem \ref{thm:AMP}]
The first step is to show the equivalence between the state evolution for the true AMP and the corresponding one for the auxiliary AMP. In particular, we prove that, for $t\ge 1$,
\begin{equation}\label{eq:equivSE}
    (\tilde{z}_1, \ldots, \tilde{z}_{t}) \stackrel{\rm d}{=} (z_1, \ldots, z_t) ,
\end{equation}
where the random variables on the left are defined in \eqref{eq:SElawsaux}, and the random variables on the right are defined in \eqref{eq:SElaws}. As $(\tilde{z}_1, \ldots, \tilde{z}_t)\sim\mathcal N(\bzero, \tilde{\bSigma}_t)$ and $(z_1, \ldots, z_t)\sim\mathcal N(\bzero, \bSigma_t)$, \eqref{eq:equivSE} is readily implied by 
\begin{equation}\label{eq:eqS}
    \tilde{\bSigma}_t=\bSigma_t, \qquad \mbox{ for all }t\ge 1.
\end{equation}
We now show that \eqref{eq:eqS} holds by induction. The base case ($t=1$) follows from the definitions of $\tilde{\bSigma}_1, \bSigma_1$. Towards induction, assume that $\tilde{\bSigma}_t=\bSigma_t$ for some $t\ge 1$. By comparing the definition of $\hat{x}_s$ in \eqref{eq:SElaws} with the definition of $\tilde{x}_s$ in \eqref{eq:SElawsaux} and by using the choice of $\tilde{h}_s$ in \eqref{eq:deftildeh} (for $s\in\{2, \ldots, t+1\}$), we readily obtain that $\Delta_{t+1}=\tilde{\Delta}_{t+1}$ and $\bar{\bPhi}_{t+1}=\tilde{\bPhi}_{t+1}$. Hence, by using \eqref{eq:defSigma} and \eqref{eq:defSigmat}, we have that $\tilde{\bSigma}_{t+1}=\bSigma_{t+1}$ and the proof of \eqref{eq:eqS} is complete. 

The second step is to show that, for any pseudo-Lipschitz function  $\psi: \mathbb R^{2t+2} \to \mathbb R$ of order 2, the following limit holds almost surely for $t \ge 1$: 
\begin{equation}\label{eq:PLsecondstep}
    \begin{split}
        \lim_{N \to \infty}  \Bigg\vert 
        \frac{1}{N}& \sum_{i=1}^{N} \psi\left((\bx^1)_i, \ldots, (\bx^t)_i, \,  (\hat{\bx}^1)_i, \ldots, (\hat{\bx}^{t+1})_i, \, (\bX)_i\right)
        \\
        & -   \frac{1}{N} \sum_{i=1}^{N} \psi\left((\bu^1)_i, \ldots, (\bu^t)_i, \,  (\tilde{\bx}^1)_i, \ldots, (\tilde{\bx}^{t+1})_i, \, (\bX)_i\right)  \Bigg \vert =0,
    \end{split}
\end{equation}
where, we have defined for $s\in \{1, \ldots, t\}$,
\begin{equation}\label{eq:defu}
    \bu^s = \tilde{\bz}^s+(\bB_s)_{s, 1} \tilde{\bx}^1 + \sum_{i=2}^s (\bB_s)_{s, i}\tilde{\bx}^i+\mu_s \bX-\bar{\beta}_s \tilde{\bx}^{s-1}.
\end{equation}
From here till the end of the argument, we use $C$ to denote a generic positive constant, which can change from line to line and is independent of $N$. All the limits hold almost surely, thus this is not explicitly stated every time. Since $\psi$ is pseudo-Lipschitz, we have
\begin{equation}
    \begin{split}
         \Bigg\vert 
         &\frac{1}{N} \sum_{i=1}^{N} \psi\left((\bx^1)_i, \ldots, (\bx^t)_i, \,  (\hat{\bx}^1)_i, \ldots, (\hat{\bx}^{t+1})_i, \, (\bX)_i\right)
        \\
        & \hspace{3em}-   \frac{1}{N} \sum_{i=1}^{N} \psi\left((\bu^1)_i, \ldots, (\bu^t)_i, \,  (\tilde{\bx}^1)_i, \ldots, (\tilde{\bx}^{t+1})_i, \, (\bX)_i\right)  \Bigg \vert\\
        & \le \frac{C}{N} \sum_{i=1}^{N} \left( 1+ |(\bX)_i| +2|(\hat{\bx}^1)_i| +\sum_{\ell=1}^t \Big( |(\bx^\ell)_i| +|(\bu^{\ell})_i|+ |(\hat{\bx}^{\ell+1})_i|  + |(\tilde{\bx}^{\ell+1})_i|  \Big) \right) \\
        &\hspace{3em} \cdot \left( \sum_{\ell=1}^t  \left(|(\bx^\ell)_i - (\bu^\ell)_i |^2  +  |(\hat{\bx}^{\ell+1})_i - (\tilde{\bx}^{\ell+1})_i |^2\right) \right)^{1/2} \\
        & \leq C(4t+3)\left[ 1 + \frac{\| \bX \|^2}{N} +  
        \sum_{\ell=1}^t \Big( \frac{\|\bx^\ell \|^2}{N} + \frac{\|\bu^\ell \|^2}{N} + \frac{\| \hat{\bx}^{\ell+1} \|^2}{N} + 
        \frac{\| \tilde{\bx}^{\ell+1} \|^2}{N} \Big) \right]^{1/2} \\
        &\hspace{3em}\cdot \left( \sum_{\ell=1}^t \left(\frac{\| \bx^\ell - \bu^{\ell}\|^2}{N} + \frac{\|\hat{\bx}^{\ell+1} - \tilde{\bx}^{\ell+1}\|^2}{N} \, \right)\right)^{1/2},  \label{eq:xz_diff}
    \end{split}
\end{equation}
where the last step uses Cauchy-Schwarz inequality (twice). We will inductively show that as $N \to \infty$: \emph{(i)} each of the terms in the last line of \eqref{eq:xz_diff} converges to zero, and \emph{(ii)} the terms within the square brackets in \eqref{eq:xz_diff} all converge to finite, deterministic limits. 

\noindent \underline{Base case ($t=1$).} We have that
\begin{equation}\label{eq:b1man}
    \begin{split}
        \bx^1-\bu^1 &= \bY\hat{\bx}^1-\tilde{\bz}^1-(\bB_1)_{1, 1}\tilde{\bx}^1-\mu_1\bX \\
        &=\bZ\hat{\bx}^1+\sqrt{\lambda}\frac{\langle \bX, \hat{\bx}^1\rangle}{N}\bX-\bZ\tilde{\bx}^1+{\sf b}_{1, 1}\tilde{\bx}^1-(\bB_1)_{1, 1}\tilde{\bx}^1-\mu_1\bX\\
        &=\sqrt{\lambda}\frac{\langle \bX, \hat{\bx}^1\rangle}{N}\bX+{\sf b}_{1, 1}\tilde{\bx}^1-(\bB_1)_{1, 1}\tilde{\bx}^1-\mu_1\bX,
    \end{split}
\end{equation}
where the first equality uses \eqref{eq:AMP} and \eqref{eq:defu}, the second equality uses \eqref{eq:spikedmodel} and \eqref{eq:auxAMP}, and the third equality uses that $\tilde{\bx}^1=\hat{\bx}^1$. Hence, by triangle inequality,
\begin{equation}\label{eq:base1}
    \begin{split}
        \frac{\|\bx^1-\bu^1\|^2}{N}&\le 2\left(\sqrt{\lambda}\frac{\langle \bX, \hat{\bx}^1\rangle}{N}-\mu_1\right)^2\frac{\|\bX\|^2}{N}+2\left({\sf b}_{1, 1}-(\bB_1)_{1, 1}\right)^2\frac{\|\tilde{\bx}^1\|^2}{N}\\
        &\le C\left(\left(\sqrt{\lambda}\frac{\langle \bX, \hat{\bx}^1\rangle}{N}-\mu_1\right)^2+\left({\sf b}_{1, 1}-(\bB_1)_{1, 1}\right)^2\right),
    \end{split}
\end{equation}
where the last inequality uses that $\tilde{\bx}^1=\hat{\bx}^1$ and that $(\bX, \hat{\bx}^1)$ converge in $W_2$ to random variables with finite second moments. By using \eqref{eq:AMPinit} and recalling that $\mu_1=\sqrt{\lambda}\epsilon$ (cf. \eqref{eq:SEinit}), we have 
\begin{equation}\label{eq:base2}
    \lim_{N\to\infty}\sqrt{\lambda}\frac{\langle \bX, \hat{\bx}^1\rangle}{N}=\sqrt{\lambda}\epsilon=\mu_1.
\end{equation}
Furthermore, note that  $(\bB_1)_{1, 1}=\bar{\kappa}_1$ (cf. \eqref{eq:SEinit}) and ${\sf b}_{1, 1}=\kappa_1$ (cf. \eqref{eq:deftildeB}) and, by the model assumptions, $\kappa_1\to\bar{\kappa}_1$, as $N\to\infty$. Hence, ${\sf b}_{1, 1}\to (\bB_1)_{1, 1}$ and, by combining this observation with \eqref{eq:base1} and \eqref{eq:base2}, we obtain that 
\begin{equation}\label{eq:it1}
    \lim_{N\to\infty}\frac{\|\bx^1-\bu^1\|^2}{N}=0.
\end{equation}
Next, by expressing $\hat{\bx}^2$ via \eqref{eq:AMP} and $\tilde{\bx}^2$ via \eqref{eq:auxAMP}, \eqref{eq:deftildeh} and \eqref{eq:defu}, we have that
\begin{equation}
    \hat{\bx}^2-\tilde{\bx}^2=h_2(\bx^1)-h_2(\bu^1).
\end{equation}
Thus, as $h_2$ is Lipschitz, \eqref{eq:it1} immediately implies that
\begin{equation}
    \lim_{N\to\infty}\frac{\|\hat{\bx}^2-\tilde{\bx}^2\|^2}{N}=0.
\end{equation}
An application of the triangle inequality gives that, for any $i\ge 1$,
\begin{equation}\label{eq:tr1}
    \begin{split}
        \|\bu^i\|- \|\bx^i-\bu^i\|&\le \|\bx^i\|\le \|\bu^i\|+ \|\bx^i-\bu^i\|, \\
         \|\tilde{\bx}^{i+1}\|- \|\hat{\bx}^{i+1}-\tilde{\bx}^{i+1}\| &\le \|\hat{\bx}^{i+1}\|\le \|\tilde{\bx}^{i+1}\|+ \|\hat{\bx}^{i+1}-\tilde{\bx}^{i+1}\|.
    \end{split}
\end{equation}
Thus, by using \eqref{eq:tr1} with $i=1$ and Proposition \ref{prop:auxSE}, we obtain that
\begin{equation}
    \begin{split}
        &\lim_{N\to\infty}\frac{\|\bx^1\|^2}{N}=\lim_{N\to\infty}\frac{\|\bu^1\|^2}{N}=\mathbb E[(\tilde{z}_1+(\bB_1)_{1, 1}\hat{x}_1+\mu_1 X)^2], \\
        &\lim_{N\to\infty}\frac{\|\hat{\bx}^2\|^2}{N}=\lim_{N\to\infty}\frac{\|\tilde{\bx}^2\|^2}{N}=\mathbb E[(\tilde{x}_2)^2],
    \end{split}
\end{equation}
which concludes the base step.

\noindent \underline{Induction step.} Assume towards induction that
\begin{align}
    &\lim_{N\to\infty}\frac{\|\bx^{j}-\bu^{j}\|^2}{N}=0,\quad \mbox{ for }j\in\{1, \ldots, t\},\label{eq:ind0}\\
    &\lim_{N\to\infty}\frac{\|\hat{\bx}^{j}-\tilde{\bx}^{j}\|^2}{N}=0,\quad \mbox{ for }j\in\{2, \ldots, t+1\},\label{eq:ind1}\\
    &\lim_{N\to\infty}\frac{\|\bx^{j}\|^2}{N}=\lim_{N\to\infty}\frac{\|\bu^{j}\|^2}{N}=\mathbb E\Bigg[\left(\tilde{z}_{j}+(\bB_{j})_{j, 1}\hat{x}_1+\sum_{i=2}^{j}(\bB_{j})_{j, i}\tilde{x}_i+\mu_{j}X-\bar{\beta}_{j}\tilde{x}_{j-1}\right)^2\Bigg], \,\,\, \mbox{ for }j\in\{1, \ldots, t\},\label{eq:ind1bis}\\
    &\lim_{N\to\infty}\frac{\|\hat{\bx}^{j}\|^2}{N}=\lim_{N\to\infty}\frac{\|\tilde{\bx}^{j}\|^2}{N}=\mathbb E[\tilde{x}_j^2], \quad \mbox{ for }j\in\{2, \ldots, t+1\}.\label{eq:ind2}
\end{align}
We now show that the following limits hold:
\begin{align}
    &\lim_{N\to\infty}\frac{\|\bx^{t+1}-\bu^{t+1}\|^2}{N}=0,\label{eq:indres1}\\
    &\lim_{N\to\infty}\frac{\|\hat{\bx}^{t+2}-\tilde{\bx}^{t+2}\|^2}{N}=0,\label{eq:indres2}\\
    &\lim_{N\to\infty}\frac{\|\bx^{t+1}\|^2}{N}=\lim_{N\to\infty}\frac{\|\bu^{t+1}\|^2}{N}\nonumber\\
    &\hspace{5.5em}=\mathbb E\Bigg[\left(\tilde{z}_{t+1}+(\bB_{t+1})_{t+1, 1}\hat{x}_1+\sum_{i=2}^{t+1}(\bB_{t+1})_{t+1, i}\tilde{x}_i+\mu_{t+1}X-\bar{\beta}_{t+1}\tilde{x}_{t}\right)^2\Bigg],\label{eq:indres3}\\
    &\lim_{N\to\infty}\frac{\|\hat{\bx}^{t+2}\|^2}{N}=\lim_{N\to\infty}\frac{\|\tilde{\bx}^{t+2}\|^2}{N}=\mathbb E[\tilde{x}_{t+2}^2].\label{eq:indres4}
\end{align}
By doing so, we will have proved also the induction step and consequently that \eqref{eq:PLsecondstep} holds. 

Using similar passages as in \eqref{eq:b1man}, we obtain
\begin{equation}
    \begin{split}
        \bx^{t+1}-\bu^{t+1} &= \bY\hat{\bx}^{t+1} - \beta_{t+1}\hat{\bx}^{t}-\tilde{\bz}^{t+1}-(\bB_{t+1})_{t+1, 1} \tilde{\bx}^1 - \sum_{i=2}^{t+1} (\bB_{t+1})_{t+1, i}\tilde{\bx}^i-\mu_{t+1} \bX+\bar{\beta}_{t+1} \tilde{\bx}^{t}\\
        &= \bZ\hat{\bx}^{t+1}+\sqrt{\lambda}\frac{\langle \bX, \hat{\bx}^{t+1}\rangle}{N}\bX - \beta_{t+1}\hat{\bx}^{t}-\bZ \tilde{\bx}^{t+1} + \sum_{i=1}^{t+1} {\sf b}_{t+1, i}\tilde{\bx}^i-(\bB_{t+1})_{t+1, 1} \tilde{\bx}^1 \\
        &\hspace{17em}- \sum_{i=2}^{t+1} (\bB_{t+1})_{t+1, i}\tilde{\bx}^i-\mu_{t+1} \bX+\bar{\beta}_{t+1} \tilde{\bx}^{t}.
    \end{split}
\end{equation}
Hence, by triangle inequality,
\begin{equation}\label{eq:decT}
    \begin{split}
        \frac{\|\bx^{t+1}-\bu^{t+1}\|^2}{N}&\le C\bigg(\frac{\|\bZ\hat{\bx}^{t+1}-\bZ\tilde{\bx}^{t+1}\|^2}{N}+\left(\sqrt{\lambda}\frac{\langle \bX, \hat{\bx}^{t+1}\rangle}{N}-\mu_{t+1}\right)^2\frac{\|\bX\|^2}{N}\\
        &\hspace{2em}+\sum_{i=1}^{t+1}\left({\sf b}_{t+1, i}-(\bB_{t+1})_{t+1, i}\right)^2\frac{\|\tilde{\bx}^i\|^2}{N}+(\bar{\beta}_{t+1}-\beta_{t+1})^2\frac{\|\hat{\bx}^t\|^2}{N}+\bar{\beta}_{t+1}\frac{\|\tilde{\bx}^t-\hat{\bx}^t\|^2}{N}\bigg)\\
        &:= C(T_1+T_2+T_3+T_4+T_5).
    \end{split}
\end{equation}
Consider the first term. Since $\|\bZ\|_{\rm op}\le C$, the induction hypothesis \eqref{eq:ind1} implies that $T_1\to 0$ as $N\to\infty$.

Consider the second term. The following chain of equalities holds:
\begin{equation}\label{eq:T2}
    \lim_{N\to \infty}\sqrt{\lambda}\frac{\langle \bX, \hat{\bx}^{t+1}\rangle}{N}=\lim_{N\to \infty}\sqrt{\lambda}\frac{\langle \bX, \tilde{\bx}^{t+1}\rangle}{N}=\sqrt{\lambda} \mathbb E[X\,\tilde{x}_{t+1}]=\sqrt{\lambda} \mathbb E[X\,\hat{x}_{t+1}]=\mu_{t+1}.
\end{equation}
Here, the first equality uses \eqref{eq:ind1} together with the fact that $\|\bX\|^2/ N$ is upper bounded by a constant independent of $N$; the second equality follows from Proposition \ref{prop:auxSE}; the third equality uses \eqref{eq:equivSE} and the definitions of $\hat{x}_{t+1}$ and $\tilde{x}_{t+1}$ in \eqref{eq:SElaws} and \eqref{eq:SElawsaux}, respectively; and the fourth equality uses the definition of $\mu_{t+1}$ in \eqref{eq:SEmu}. Finally, using \eqref{eq:T2} and again that $\|\bX\|^2/ N$ is upper bounded by a constant independent of $N$ gives that $T_2\to 0$ as $N\to\infty$.

Consider the third term. The following chain of equalities holds, for $1\le j<i\le (t+1)$,
\begin{equation}\label{eq:T3}
    \lim_{N\to \infty} (\bPhi_{t+1})_{i, j} =\lim_{N\to\infty}\langle\partial_j \tilde{\bx}^i\rangle =\mathbb E[\partial_j\tilde{x}_i] = \mathbb E[\partial_j\hat{x}_i] = (\bar{\bPhi}_{t+1})_{i, j}
\end{equation}
Here, the first equality uses the definition \eqref{eq:defbPhi}; the second equality follows from Lemma \ref{lem:lipderiv}, as $\tilde{\bx}^i=\tilde{h}_i(\tilde{\bz}^1, \ldots, \tilde{\bz}^{i-1}, \hat{\bx}^1, \bX)$ converges in $W_2$ (and therefore in distribution) to $\tilde{x}_i=\tilde{h}_i(\tilde{z}_1, \ldots, \tilde{z}_{i-1}, \hat{x}_1, X)$ and $h_i$ satisfies the assumptions in \textbf{(A1)}; the third equality uses \eqref{eq:equivSE} and the definitions of $\hat{x}_{i}$ and $\tilde{x}_{i}$ in \eqref{eq:SElaws} and \eqref{eq:SElawsaux}, respectively;  and the fourth equality uses the definition of $(\bar{\bPhi}_{t+1})_{i, j}$ in \eqref{eq:defbPhibar}. By the model assumptions, as $N\to\infty$, $\kappa_j\to\bar{\kappa}_j$ for all $j$. Thus, by combining \eqref{eq:T3} with the definitions of $\bB_{t+1}$ and $\tilde{\bB}_{t+1}$ in \eqref{eq:defB} and \eqref{eq:deftildeB}, respectively, we conclude that, as $N\to\infty$, ${\sf b}_{t+1, i}\to(\bB_{t+1})_{t+1, i}$ for $i\in \{1, \ldots, t+1\}$. By using the induction hypothesis \eqref{eq:ind2}, which shows that $\|\tilde{\bx}^i\|^2/N$ converges to a finite limit, we conclude that $T_3\to 0$ as $N\to\infty$.

Consider the fourth term. By using the induction hypothesis \eqref{eq:ind0} and \eqref{eq:ind1bis}, together with \eqref{eq:xz_diff}, we obtain that $\bx^t$ and $\bu^t$ have the same $W_2$ limit given by Proposition \ref{prop:auxSE}, namely,
\begin{equation*}
    \bx^t \, \stackrel{\mathclap{W_2}}{\longrightarrow}  \,    \tilde{z}_{t}+(\bB_{t})_{t, 1}\hat{x}_1+\sum_{i=2}^{t}(\bB_{t})_{t, i}\tilde{x}_i+\mu_{t}X-\bar{\beta}_{t}\tilde{x}_{t-1}.
\end{equation*}
Thus, by recalling that $\beta_{t+1} = \langle h_{t+1}'(\bx^t)\rangle$, an application of Lemma \ref{lem:lipderiv} gives that 
\begin{equation}\label{eq:T4}
    \lim_{N\to\infty}\beta_{t+1} = \mathbb E\bigg[h_{t+1}'\bigg(\tilde{z}_t+(\bB_t)_{t, 1} \hat{x}_1 + \sum_{i=2}^t (\bB_t)_{t, i}\tilde{x}_{i}+\mu_t X-\bar{\beta}_t \tilde{x}_{t-1}\bigg)\bigg].
\end{equation}
Furthermore, by using \eqref{eq:equivSE} and recalling the definition of $\bar{\beta}_{t+1}$, we have that the RHS of \eqref{eq:T4} is equal to  $\bar{\beta}_{t+1}$. Hence, by using the induction hypothesis \eqref{eq:ind2}, we obtain that $T_4\to 0$ as $N\to\infty$. Finally, by using the induction hypothesis \eqref{eq:ind1}, we 
conclude that also $T_5\to 0$ as $N\to\infty$.

As $T_i\to 0$ for $i\in \{1, \ldots, 5\}$, \eqref{eq:decT} implies that \eqref{eq:indres1} holds. Next, as $h_{t+1}$ is Lipschitz, \eqref{eq:indres1} immediately implies \eqref{eq:indres2}. Then, by using \eqref{eq:tr1} with $i=t+1$ and Proposition \ref{prop:auxSE}, we obtain that \eqref{eq:indres3} and \eqref{eq:indres4} hold, thus concluding the inductive proof. The result we have just proved by induction, combined with \eqref{eq:xz_diff}, gives that \eqref{eq:PLsecondstep} holds. 

Another application of Proposition \ref{prop:auxSE}, together with \eqref{eq:PLsecondstep}, gives that
\begin{equation}\label{eq:fin1}
    \begin{split}
         \lim_{N \to \infty}  
         \frac{1}{N}& \sum_{i=1}^{N} \psi\left((\bx^1)_i, \ldots, (\bx^t)_i, \,  (\hat{\bx}^1)_i, \ldots, (\hat{\bx}^{t+1})_i, \, (\bX)_i\right) =\mathbb E [ \psi(u_1, \ldots, u_t, \tilde{x}_1, \ldots, \tilde{x}_{t+1}, X) ],
     \end{split}
\end{equation}
where we have defined for $s\in \{1, \ldots, t\}$,
\begin{equation}
    u_s = \tilde{z}_s+(\bB_s)_{s, 1} \tilde{x}_1 + \sum_{i=2}^s (\bB_s)_{s, i}\tilde{x}_i+\mu_s X-\bar{\beta}_s \tilde{x}_{s-1}.
\end{equation}
Finally, by using \eqref{eq:equivSE}, we have that
\begin{equation}\label{eq:fin2}
    \mathbb E [ \psi(u_1, \ldots, u_t, \tilde{x}_1, \ldots, \tilde{x}_{t+1}, X) ] = \mathbb E [ \psi(x_1, \ldots, x_t, \hat{x}_1, \ldots, \hat{x}_{t+1}, X) ].
\end{equation}
By combining \eqref{eq:fin1} and \eqref{eq:fin2}, we obtain that the desired result \eqref{eq:PL2_main_resultx} holds, which concludes the proof. 
\end{proof}



==> sections/08App_proofBayes.tex <==
For every $\theta > 0$ and matrix $\bA\in\R^{N\times N}$ the rank-1 spherical integral is defined according to
\begin{equation*}
    I_N(\theta,\bA) := \int d\mu_N(\bs) \exp\big(\theta \bs^\intercal\bA \bs\big);
\end{equation*}
where, as before, $\mu_N(\cdot)$ is the uniform measure over $\mathbb{S}^{N-1}(\sqrt{N})$.

It will be useful to define a slight generalization of the model \eqref{eq:spikedmodel} that includes a ``Wigner regularization'' of the rotationally-invariant noise. Namely, we will consider in this section the following generalized model for the data:
\begin{align}\label{eq:spikedmodel_wigReg}
\bY_\veps=\frac{\sqrt{\lambda}} {N} \bX\bX^\intercal + \bZ+\sqrt{\veps}\,\bW;
\end{align}
where, as before, $\bW$ is a standard Wigner matrix and $\veps>0$ is some constant. In a similar way as we did for the non-regularized problem, we will denote by $\thermal{\cdot}_\veps$ the mean of the Gibbs measure obtained by replacing $\bY$ for $\bY_\veps$ in equation \eqref{estimatorMis1}. The rest of the notations used here will be similar to the ones for the non-regularized model, though we will add a subscript $\veps$ when it is useful to remark dependence of a given quantity over this parameter. When this subscript is omitted, it is understood that $\veps=0$.
%Recall the form of the log-likelihood when assuming purely Wigner noise:
% \begin{equation*}
%     \mathcal{L}_N(\bx) = \frac{1}{2}\sqrt{\frac{\lambda }{N}}\bx^\intercal\bY_\veps \bx - \frac{\lambda}{4 N}\|\bx\|^4 .
% \end{equation*}
% Recall hypothesis \ref{hyp:eigen} for the noise $\bZ$.
% Our first intermediate result is a limit for the so-called expected \emph{free entropy}:
%     \begin{equation*}
%         f_{\veps,N} := \frac{1}{N}\E  \ln \int d\mu(\bx) \ e^{ \frac{1}{2}\sqrt{\frac{\lambda }{N}}\bx^\intercal\bY_\veps \bx  },
%     \end{equation*}
%     where, as before, $\mu(\cdot)$ is the uniform measure over $\mathbb{S}^{N-1} (\sqrt{N})$. Here we removed the term proportional to $\|\bx\|^4$ from the log-likelihood as in this case it is just a constant. In other words, in this case we have the free entropy is the mean rank-one spherical integral $$f_{\veps,N} = \frac{1}{N}\E\ln I_N(\sqrt{\lambda}/2,\bY_\veps/\sqrt{N}).$$

Our first intermediate result, Proposition~\ref{prop:fe_spherical}, characterizes the mean log-spherical integral for the regularized data matrix. Although this proposition may be interesting in itself, its main porpoise here will be to allow us to derive the MSE of the mismatched Bayes estimator in terms of derivatives of the the mean log-spherical integral with respect to ${\veps}$ and ${\lambda_*}$. This is in fact the reason for introducing the regularization in the first place.
 

% To state the result in this section, for every $\sqrt{\lambda_*}>1/\hmax$ and $\lambda > 0$ we will define the function $\tilde\phi_\rho(\lambda,\lambda_*)$ according to
% \begin{equation*}
%     \tilde\phi_\rho(\lambda,\lambda_*) :=
%     \begin{cases}
%         \frac{1}{2}\int_0^{\sqrt{\lambda}} R_\rho(t) dt & \mbox{if }  \sqrt{\lambda \lambda_*} < 1\\
%         \frac{\sqrt \lambda}2K_\rho(1/\sqrt{\lambda_*}) - \frac{1}{2}\int_\Sigma d\rho(t)\ln\left(\sqrt{\lambda} e(K_\rho(1/\sqrt{\lambda_*})-t)\right) & \mbox{if } \sqrt{\lambda\lambda_*} \geq 1.
%     \end{cases}
% \end{equation*}
% We will also define for $\lambda,\lambda_* > 0$ another function
% \begin{equation*}
%     \psi_\rho(\lambda,\lambda_*) :=
%     \begin{cases}
%         \phi_\rho(\sqrt{\lambda}/2) & \mbox{if }  \sqrt{\lambda_*} < \frac{1}{\hmax}\\
%         \tilde\phi_ {\rho}(\lambda,\lambda_*) & \mbox{if } \sqrt{\lambda_*} \geq \frac{1}{\hmax}.
%     \end{cases}
% \end{equation*}

% \begin{proposition}\label{prop:fe_spherical}
%     Under this setting, for each $\lambda,\lambda_* > 0$ we have $\lim_{N\to\infty} f_{\veps,N} = \psi_\rho(\lambda,\lambda_*)$.
% \end{proposition}

% \textbf{Example.} \manunote{Add computation of example of noise with Rademacher eigenvalues. Include graphs and discussion.}


% JEAN: my computations yield the following (which matches Manuel's computation):
    % In the next proposition, we establish the limit value of the free entropy in the setting considered. 
    % For this, define
    % \begin{equation*}
    %     g_{\lambda,\veps}(x):=\frac{\sqrt\lambda}2x- \frac{1}{2}\int_K d\rho_{\veps}(t)\ln( x-t)-\frac12-\frac14\ln\lambda.
    % \end{equation*}
    % Notice that its derivative is given by
    % \begin{equation*}
    %     g'_{\lambda,\veps}(x)=\frac{\sqrt\lambda}2- \frac{1}{2}H_{\rho_\veps}(x).
    % \end{equation*}
    
    \begin{proposition}[Mean spherical integral]\label{prop:fe_spherical}
    Let $\rho_\veps(\cdot)$ be the weak limit of the empirical spectral density of $\bY_\veps$ and $R_\veps$ its associated R-transform. For every $\lambda,\veps>0$, define the function $g_{\lambda,\veps}:\R_{>\overline{\gamma}}\mapsto\R$ according to
    \begin{equation*}
        g_{\lambda,\veps}(x):=\frac{\sqrt\lambda}2x- \frac{1}{2}\int d\rho_{\veps}(t)\ln( x-t)-\frac12-\frac14\ln\lambda.
    \end{equation*}
        Then, under Hypothesis \ref{hyp:eigen} and for every $\lambda,\lambda_* > 0$ we have that 
        \begin{align*}
        \lim_{N\to+\infty} \frac{1}{N}\E\ln I_N\Big(\frac{\sqrt{\lambda}}2, \bY_\veps\Big)= f_\veps(\lambda,\lambda_*) :=
             \begin{cases}        
                g_{\lambda,\veps}(K_{\rho_\veps}(1/\sqrt{\lambda_*}))  &\mbox{if }  \hmax_\veps\sqrt{\lambda_*} \ge 1 \ \mbox{and}\ \lambda\lambda_*> 1,\\
                g_{\lambda,\veps}(\overline{\gamma}_\veps) &\mbox{if }  \hmax_\veps\sqrt{\lambda_*} < 1 \ \mbox{and}\ \sqrt{\lambda}>  \hmax_\veps,\\
                \frac12 \int_0^{\sqrt \lambda} R_{\rho_\veps}(t)dt   &\mbox{else}.
            \end{cases}   
        \end{align*}
    \end{proposition}



\subsection{Proof of Theorem \ref{thm:lim_mse}}

Like in the analysis of mismatched inference with gaussian noise of \cite{pourkamali2021mismatched}, we will make use of the following result for the asymptotic value of the rank-1 spherical integral.
\begin{thm}[Theorem 6 of \cite{guionnet2005fourier}]\label{thm:spher_int} Let $\eigmax_\veps$ be the limit of the maximum eigenvalue of $\bY_\veps$ and define $\hmax_\veps:=\lim_{z\downarrow\eigmax_\veps} H_{\rho_\veps}(z)$. Assume that Hypothesis \ref{hyp:eigen} holds, then
    \begin{equation*}
        \lim_{N\to\infty}\frac{1}{N} \ln I_N(\theta,\bY_\veps) = \phi_\veps(\theta) :=
        \begin{cases}
            \frac{1}{2}\int_0^{2\theta} R_{\rho_\veps}(t) dt & \mbox{if } 2\theta \leq \hmax_\veps\\
            \theta\eigmax_\veps - \frac{1}{2}\int_K d\rho(t)\ln\left(2\theta e(\eigmax_\veps-t)\right) & \mbox{if } 2\theta > \hmax_\veps.
        \end{cases}
    \end{equation*}
\end{thm}
    
\begin{proof}[Proof of Proposition \ref{prop:fe_spherical}]
    By Theorem \ref{thm:larg_eigen}, we are a.s. under the hypothesis of Theorem \ref{thm:spher_int}. We then have that almost surely
    \begin{equation*}
        \lim_{N\to\infty}\frac{1}{N}\ln \int d\mu_N(\bx) \ e^{ \frac{\sqrt{\lambda}}{2}\bx^T \bY \bx } = f_\veps(\lambda,\lambda_*).
    \end{equation*}
    Moreover, because by hypothesis the sequence of values of the largest eigenvalue of $\bZ$ is convergent, it is then bounded by some $C > 0$. Thus,
    \begin{equation*}
        \frac{\sqrt{\lambda}}{2}\bx^T \bY \bx \leq \frac{\sqrt{\lambda}}{2}(C+\sqrt{\lambda_*})N.
    \end{equation*}
    Then the result follows by dominated convergence.
\end{proof}

To establish this result, define the \emph{magnetization} according to $M_N := N^{-2} (\bX^T \bx)^2$ and the \emph{overlap} $Q_N := N^{-2} (\bx^{(1)T} \bx^{(2)})^2$. Here the supra-indices indicate two independent samples from the Gibbs measure with the same quenched disorder. Theorem \ref{thm:lim_mse} is the consequence of the asymptotic formulas for the mean magnetization and overlap of the Gibbs measure given in the next lemmas. 

\begin{lemma}\label{lem:mag_limit}
    In the setting considered, for all $\lambda,\lambda_* > 0$ fixed we have $\lim_{N\to\infty} \E\thermal{M_N}_0 = M(\lambda,\lambda_*)$.
\end{lemma}
\begin{proof}
    Because in the log-likelihood of the problem the only term in which $\lambda_*$ appears (when writing $\bY_\veps$ explicitly in terms of $\bX \bX^T$) is
    \begin{equation*}
        \frac{\sqrt{\lambda \lambda_*}}{2 N} (\bX^T \bx)^2 = N\frac{\sqrt{\lambda \lambda_*}}{2} M_N,
    \end{equation*}
    we then have that for all $N\geq1$
    \begin{equation*}
        \frac{\partial f_{0,N}}{\partial \sqrt{\lambda_*}} = \frac{\sqrt{\lambda}}{2}\E\thermal{M_N}_0.
    \end{equation*}
    By the convexity of $f_{0,N}$ w.r.t. $\sqrt{\lambda_*}$ and Proposition \ref{prop:fe_spherical} we get that
    \begin{equation*}
        \lim_{N\to\infty} \E\thermal{M_N}_0 = \frac{2}{\sqrt{\lambda}} \frac{\partial f_0(\lambda,\lambda_*)}{\partial \sqrt{\lambda_*}} = \frac{2}{\sqrt{\lambda}} \frac{\partial f_0(\lambda,\lambda_*)}{\partial \sqrt{\lambda_*}} = 4\sqrt{\frac{\lambda_*}{\lambda}} \frac{\partial f_0(\lambda,\lambda_*)}{\partial \lambda_*}.
    \end{equation*}
    The derivative with respect to $\lambda_*$ of $f_0$ is given by (recalling $K_0(x)=R_0(x)+1/x$)
    \begin{align*}
        \frac{df_0}{d\lambda_*}(\lambda_*,\lambda)=
         \begin{cases}        
            \frac{1}{4} \big(\frac{1}{(\lambda_*)^2}-\big(\frac{\lambda}{(\lambda_*)^3}\big)^{1/2}\big) \big(R'_\rho(1/\sqrt{\lambda_*})-\lambda_*\big)  &\mbox{if }  \sqrt{\lambda_*} \ge \frac{1}{\hmax} \ \mbox{and}\ \lambda\lambda_*> 1,\\
            0 &\mbox{else}.
        \end{cases}   
    \end{align*}
    From these two last equations, the result of the lemma follows.
\end{proof}

\begin{lemma}\label{lem:ovlap_limit}
    In the setting considered, for all $\lambda,\lambda_* > 0$ fixed we have $\lim_{N\to\infty} \E\thermal{Q_N}_0 = Q(\lambda)$.
\end{lemma}
\begin{proof}
    Because in the log-likelihood of the problem the only term in which $\veps$ appears (when writing $\bY_\veps$ explicitly in terms of $\bW$) is
    \begin{equation*}
        \frac{\sqrt{\lambda \veps}}{2} \bx^T \bW \bx,
    \end{equation*}
    we have that for every $N\geq1$
    \begin{equation*}
        \frac{\partial f_{0,N}}{\partial \sqrt{\veps}} = \frac{\sqrt{\lambda}}{2N}\E\thermal{\bx^T \bW \bx}_0.
    \end{equation*}
    Since $\bW$ is Wigner, its elements are distributed as independent Gaussian random variables. Using gaussian integration by parts in the r.h.s. of the last equation we get that
    \begin{equation*}
        \frac{\partial f_{0,N}}{\partial \sqrt{\veps}} = \frac{\lambda\sqrt{ \veps}}{2}(1 - \E\thermal{Q_N}_0).
    \end{equation*}
    By the convexity of $f_{\veps,N}$ w.r.t. $\sqrt{\veps}$ and Proposition \ref{prop:fe_spherical} we get that
    \begin{equation}\label{eq:ovlp_lim}
        \lim_{N\to\infty} \E\thermal{Q_N}_0 = 1 - \frac{2}{\lambda\sqrt{\veps}} \frac{\partial f_\veps(\lambda,\lambda_*)}{\partial \sqrt{\veps}}\Big|_{\veps=0} = 1 - \frac{4}{\lambda} \frac{\partial f_\veps(\lambda,\lambda_*)}{\partial \veps}\Big|_{\veps=0}.
    \end{equation}
    To find the asymptotic value of $\E\thermal{Q_N}_0$ we are thus left to compute $\partial_\veps f_\veps(\lambda,\lambda)$. We will then need to consider the three regimes of Proposition \ref{prop:fe_spherical}. 
    
    Firstly, if $\hmax\sqrt{\lambda_*}  \geq 1$ and $\lambda \lambda_* > 1$ then
    \begin{equation*}
        \begin{split}
            \frac{\partial f_\veps(\lambda,\lambda_*)}{\partial \veps} \Big|_{\veps=0} & = \frac{d }{d\veps}g_{\lambda,\veps}(K_{\rho_\veps}(\lambda_*^{-1/2})) \Big|_{\veps=0} \\
            & = \frac{\partial g_{\lambda,\veps}(x)}{\partial\veps}\Big|_{\veps=0,x=K_{\rho_0}(\lambda_*^{-1/2})} + \frac{\partial g_{\lambda,\veps}(x)}{\partial x}\Big|_{\veps=0,x=K_{\rho_0}(\lambda_*^{-1/2})} \frac{\partial K_{\rho_\veps}(\lambda_*^{-1/2})}{\partial\veps}\Big|_{\veps=0}.
        \end{split}
    \end{equation*}
    For computing $\partial_\veps g_{\lambda,\veps}(x)$ notice that the only term of $g_{\lambda,\veps}$ in which $\veps$ appears is
    \begin{equation*}
        - \frac{1}{2} \int d\rho_\veps(\gamma) \ln(x-\gamma) = -\frac{1}{2} \int_0^x H_{\rho_\veps}(z) dz.
    \end{equation*}
    Furthermore, by the Dyson Brownian motion characterization of the eigenvalues of the matrix $\bZ + \sqrt{\veps} \bW$ we have that the limiting Stieltjes transform $H_{\rho_\veps}(z)$ is a solution of Burger's equation (see for example, \cite[Proposition 4.3.10]{anderson2010introduction}); that is,
    \begin{equation}\label{eq:burguers}
        \frac{\partial H_{\rho_\veps}}{\partial \veps} = - H_{\rho_\veps} \frac{\partial H_{\rho_\veps}}{\partial z} = - \frac{1}{2} \frac{\partial (H_{\rho_\veps}^2)}{\partial z}.
    \end{equation}
    Integrating both sides of \eqref{eq:burguers} we get that
    \begin{equation}\label{eq:deriv_eps}
        \frac{\partial g_{\lambda,\veps}(x)}{\partial\veps} = \frac{1}{4} H_{\rho_\veps}^2(x).
    \end{equation}
    Which, in particular, means that
    \begin{equation}\label{eq:partial1}
        \frac{\partial g_{\lambda,\veps}(x)}{\partial\veps}\Big|_{\veps=0,x=K_{\rho_\veps}(\lambda_*^{-1/2})} = \frac{1}{4} H_{\rho_0}^2(K_{\rho_0}(\lambda_*^{-1/2})) = \frac{1}{4\lambda_*}.
    \end{equation}
    Furthermore, 
    \begin{equation}\label{eq:deriv_x}
        \frac{\partial g_{\lambda,\veps}(x)}{\partial x} = \frac{\sqrt{\lambda}}{2} - \frac{1}{2} H_{\rho_\veps}(x)
    \end{equation}
    and $\partial_\veps K_{\rho_\veps}(x) = x$. Then,
    \begin{equation}\label{eq:partial2}
        \frac{\partial g_{\lambda,\veps}(x)}{\partial x}\Big|_{\veps=0,x=K_{\rho_\veps}(\lambda_*^{-1/2})} \frac{\partial K_{\rho_\veps}(\lambda_*^{-1/2})}{\partial\veps}\Big|_{\veps=0} = \frac{1}{2}\left(1 - \frac{1}{\lambda_*}\right).
    \end{equation}
    Combining equations \eqref{eq:ovlp_lim}, \eqref{eq:partial1}, and \eqref{eq:partial2} we get that if $\hmax \sqrt{\lambda}   \geq 1$ and $\lambda_*\lambda > 1$, then
    \begin{equation*}
        \lim_{N\to\infty} \E\thermal{Q_N}_0 = 1 - \frac{1}{\lambda} \left(2 - \frac{1}{\lambda}\right).
    \end{equation*}
    

    \manunote{This paragraph is the new part of the proof. It would be good if someone double-checks it.} We will now establish the limit of the overlap when $\hmax\sqrt{\lambda_*} < 1$ and $\sqrt{\lambda} > \hmax$. In this region,
    \begin{equation}\label{eq:region_2}
        \frac{\partial f_\veps(\lambda,\lambda_*)}{\partial \veps} \Big|_{\veps=0}= \frac{d }{d\veps}g_{\lambda,\veps}(\overline{\gamma}_\veps)\Big|_{\veps=0} = \frac{\partial g_{\lambda,\veps}(x)}{\partial\veps}\Big|_{\veps=0,x=\overline{\gamma}_0} + \frac{\partial g_{\lambda,\veps}(x)}{\partial x}\Big|_{\veps=0,x=\overline{\gamma}_0} \frac{\partial \overline{\gamma}_\veps}{\partial\veps}\Big|_{\veps=0}.
    \end{equation}
    The partial derivatives $\partial_\veps g_{\lambda,\veps}(x)$ and $\partial_x g_{\lambda,\veps}(x)$ are obtained as before. Therefore, we only need to compute $\partial_\veps \overline{\gamma}|_{\veps=0}$. We will prove that as $\veps\to0$, $\overline{\gamma}_\veps = \overline{\gamma}_0 + \hmax_0 \veps + o(\veps)$. As a consequence of the Large Deviation Principle of \cite[Theorem 2.5]{guionnet2021large}, $\overline{\gamma}_\veps$ is equal to the supremum of the compact support $K_\veps$ of $\rho_\veps(\cdot)$. Notice that for all $\veps >0$, $\lim_{z\downarrow\overline{\gamma}_\veps} H'_{\rho_\veps} = -\infty$. This implies that $K'_{\rho_\veps}(\hmax_\veps) = 0$. Thus, $\hmax_\veps$ is a solution to the equation $K'_{\rho_0}(x) + \veps = 0$. And because $K'_{\rho_0}$ is analytic and monotonously increasing, the solution is unique and depends smoothly on $\veps$. Thus, $\hmax_\veps = \hmax_0 + \mathcal{O}(\veps)$ which means that
    \begin{equation*}
        \overline{\gamma}_\veps = K_{\rho_0}(\hmax_0) + \veps\hmax_0 + o(\veps) = \overline{\gamma}_0 + \veps\hmax_0 + o(\veps);
    \end{equation*}
    where we used that $K'_{\rho_0}(\hmax_0) = 0$. This proves that $\partial_\veps \overline{\gamma}_\veps|_{\veps=0} = \hmax_0$. Combining this with equations \eqref{eq:ovlp_lim}, \eqref{eq:deriv_eps}, \eqref{eq:deriv_x}, and \eqref{eq:region_2} gives the result in this region. 
    
    Finally, by Proposition \ref{prop:fe_spherical} and \eqref{eq:ovlp_lim} if $(\lambda,\lambda_*)$ does not verify either of the conditions considered above then
    \begin{equation*}
        \lim_{N\to\infty} \E\thermal{Q_N}_0 = 1- \frac{2}{\lambda}\int_0^{\sqrt{\lambda}}\partial_\veps R_{\rho_\veps}(x) dx = 1- \frac{2}{\lambda}\int_0^{\sqrt{\lambda}} x \ dx = 0.
    \end{equation*}
    This finishes the proof that $\lim_{N\to\infty} \E\thermal{Q_N}_0 = Q(\lambda)$.
\end{proof}

\begin{proof}[Proof of Theorem \ref{thm:lim_mse}]
    For establishing the formula for the MSE found in the theorem, it is enough to observe that
    \begin{equation*}
        \frac{1}{2N^2}\E ||\thermal{\bx \bx^T}_0 - \bX \bX^T||_F^2 = \frac{1}{2}(1 + \E\thermal{Q_N}_0 - 2 \E\thermal{M_N}_0),
    \end{equation*}
    and to use Lemmas \ref{lem:mag_limit} and \ref{lem:ovlap_limit}.
\end{proof}

%\subsection{Proof of Proposition \ref{prop:fe_gaussian}}
%    For proving this, we will first introduce an interpolation model and we will prove some technical lemmas for it. Let $\bS := \bX/||\bX||$ and, for every $t\in[0,1]$,
%    \begin{equation*}
%        \bY_t := \bZ + \sqrt{\lambda_* N} \bS {\bS}^T \left((1-t)\frac{||\bX||^2}{N}+t\right).
%    \end{equation*}
%    For every $t,\nu\in[0,1]$ we define the interpolating log-likelihood according to
%    \begin{equation*}
%        l_{N,t,\nu}(\bx) :=  -\frac{\lambda ||\bx||^4}{4 N} + (1-\nu)\ln I_N\left(\frac{\sqrt{\lambda}||\bx||^2}{2N},\frac{\bY_t}{\sqrt{N}}\right)+\nu N\psi_\rho(\lambda||\bx||^4/N^2,\lambda_*)
%    \end{equation*}
%    and we denote by $\langle\cdot\rangle_{t,\nu}$ and $f_{N,t,\nu}$ the corresponding Gibbs mean and expected free entropy. As noted by (Pourkamali and Macris, Mismatch), by the rotational invariance of the standard gaussian distribution, for every orthogonal matrix $\bO'\in\R^{N\times N}$, $\bx$ is equally distributed to $\bO' \bx$. Thus, if $M(\cdot)$ is the Haar measure over the orthogonal matrices on $\R^{N\times N}$
%    \begin{equation*}
%        \begin{split}
%            \int dG(\bx) e^{-\frac{\lambda ||\bx||^4}{4 N} + \frac{1}{2}\sqrt{\frac{\lambda }{N}}\bx^T \bY_0 \bx } & = \int dG(\bx) dM(\bO')  e^{-\frac{\lambda ||\bO' \bx||^4}{4 N} + \frac{1}{2}\sqrt{\frac{\lambda }{N}}(\bO'\bx)^T \bY_0 \bO' \bx}\\
%            & =  \int dG(\bx) e^{-\frac{\lambda ||\bx||^4}{4 N} + \ln I_N\left(\frac{\sqrt{\lambda}||\bx||^2}{2N},\frac{\bY_0}{\sqrt{N}}\right)};
%        \end{split}
%    \end{equation*}
%    where we used that $|\mbox{det}\ \bO'| = 1$. We then have that $f_{N,0,0} = f_N$.
    
%    The strategy of the proof will be the following. We will first show through interpolation that $f_{N,0,0}$ is equal to $f_{N,1,1}$ in the limit of $N\to\infty$. This requires the technical result given in Corollary \ref{cor:secmom_bound}. Then, we establish a large deviation principle for the squared norm of gaussian vectors and use it along with Lemma \ref{lem:varad_hyp} and Varadhan's Lemma to prove the asymptotic expected free entropy formula. It is important to note that although the strategy of the proof is different, the basic idea is the same as in (Pourkamali and Macris, Mismatch): use the change of variables above and Theorems \ref{thm:larg_eigen} and \ref{thm:spher_int} to express the limit of the expected free entropy as an optimisation problem.
    
%    \begin{lemma}\label{lem:exp_bound}
%        There is some $C > 0$ s.t. for every $t,\nu\in[0,1]$ and $N\geq1$
%        \begin{equation*}
%            \ln\langle e^{||\bx||^2/2}\rangle_{t,\nu} \leq N C (||\bX||^4/N^2 + ||\bX||^2/N + 1).
%        \end{equation*}
%    \end{lemma}
%    \begin{proof}
%        To see this, first notice that for every $N\geq1$, $t\in[0,1]$, and $\theta > 0$ we have that
%        \begin{equation}\label{eq:bound_si}
%            {\scriptstyle\left(\Sigma_{min}-\sqrt{\lambda_*}\left((1-t)\frac{||\bX||^2}{N}+t\right)\right)}\theta \leq \frac{1}{N}\ln I_N(\theta,\bY_t)\leq {\scriptstyle\left(\Sigma_{max}+\sqrt{\lambda_*}\left(\frac{(1-t)||\bX||^2}{N}+t\right)\right)}\theta.
%        \end{equation}
%        Because $\psi_\rho(\lambda||\bx||^4/N^2,\lambda_*)$ is the limit of $N^{-1}\ln I_N(\theta,\bY_1)$ evaluated at $\theta = \sqrt{\lambda}||\bx||^2/(2N)$, this implies that
%        \begin{equation}\label{eq:bound_psi}
%            (\Sigma_{min}-\sqrt{\lambda_*})\frac{\sqrt{\lambda}||\bx||^2}{2 N}  \leq \psi_\rho(\lambda||\bx||^4/N^2,\lambda_*) \leq (\Sigma_{max}+\sqrt{\lambda_*})\frac{\sqrt{\lambda}||\bx||^2}{2 N}.
%        \end{equation}
%        Therefore, for all $\bx\in\R^N$ and $t,\nu\in[0,1]$
%        \begin{equation}\label{eq:bound_ham}
%            \begin{split}
%                l_{N,t,\nu}(\bx) & \leq -\frac{\lambda ||\bx||^4}{4 N} + \left(\Sigma_{max}+\sqrt{\lambda_*}\left(\frac{||\bX||^2}{N}+1\right)\right)\frac{\sqrt{\lambda}||\bx||^2}{2 N}\\
%                & \leq \frac{N}{4}\left(\Sigma_{max}+\sqrt{\lambda_*}\left(\frac{||\bX||^2}{N}+1\right) \right)^2.
%            \end{split}
%        \end{equation}
%        On the other hand, if we define $A:=\{\bx\in\R^N:||\bx||^2\leq 2 N\}$ then by bounds \eqref{eq:bound_si} and \eqref{eq:bound_psi} we have that for all $t,\nu\in[0,1]$
%        \begin{equation}\label{eq:bound_parf}
%            \begin{split}
%                Z_N = \int_{\R^N} dG(\bx) e^{l_{N,t,\nu}(\bx)} & \geq \int_A dG(\bx) e^{l_{N,t,\nu}(\bx)} \\
%                & \geq e^{-\left(\lambda+\sqrt{\lambda\lambda_*}\left(\frac{||\bX||^2}{N}+1\right)-\sqrt{\lambda}\Sigma_{min}\right)N} G(\mathbb{I}_A).
%            \end{split}
%        \end{equation}
%        And because the law of large numbers implies that $G(\mathbb{I}_A)\to1$, equations \eqref{eq:bound_ham} and \eqref{eq:bound_parf} prove the conclusion of the Lemma.
%    \end{proof}
    
%    Observe that $||\bX||^2$ has a $\chi^2$-distribution with $N$ degrees of freedom and thus its fourth moment is a bounded sequence of $N\geq1$. From this, Lemma \ref{lem:exp_bound}, and (Lemma 3.1.8, Talagrand Mean) we obtain the following.
%    \begin{corollary}\label{cor:secmom_bound}
%        For all $t,\nu\in[0,1]$ and $N\geq1$ we have $\E\langle\frac{||\bx||^4}{N^2}\rangle_{t,\nu} \leq C$, with $C>0$ some constant.
%    \end{corollary}
    
%    Finally, we will prove that the bounded moment hypothesis of Varadhan's Lemma holds for $H_{N,1,1}(||\bx||^2)$ w.r.t. the standard gaussian density.
%    \begin{lemma}\label{lem:varad_hyp}
%        For every $\xi,\lambda,\lambda_* > 0$ and $N\geq1$, it holds that
%        \begin{equation*}
%            \frac{1}{N}\E \ln \left(\int_{\R^N}dG(\bx) e^{\xi N\left(-\frac{\lambda ||\bx||^4}{4 N^2} + \psi_\rho(\lambda||\bx||^4/N^2,\lambda_*)\right)}\right) \leq \frac{\xi}{4}\left(\Sigma_{max}+\sqrt{\lambda_*}-\frac{1}{\xi\sqrt{\lambda}}\right)^2.
%        \end{equation*}
%    \end{lemma}
%    \begin{proof}
%        Similarly to the way we got equation \eqref{eq:bound_ham}, it can be seen that
%        \begin{equation*}
%            \xi H_{N,1,1}(\bx) - \frac{||\bx||^2}{2} \leq N \frac{\xi}{4}\left(\Sigma_{max}+\sqrt{\lambda_*}-\frac{1}{\xi\sqrt{\lambda}}\right)^2.
%        \end{equation*}
%        From which the conclusion follows.
%    \end{proof}
    
%    We can now proceed with the proof of the main result of the section.
    
%    \begin{proof}[Proof of Proposition \ref{prop:fe_gaussian}]
%        We will first prove that $\lim_{N\to\infty}|f_{N,0,0} - f_{N,1,1}| = 0$. For this, observe that for all $t\in[0,1]$ we have
%        \begin{equation*}
%            \begin{split}
%                \left|\frac{d f_{N,t,0}}{dt}\right| & = \frac{\sqrt{\lambda\lambda_*}}{2 N}\left|\E\left(\langle({\bS}^T \bx)^2\rangle_{t,0} \left(1-\frac{||\bX||^2}{N}\right)\right)\right| \\
%                & \leq \frac{\sqrt{\lambda\lambda_*}}{2 N} \sqrt{\E\left\langle\frac{||\bx||^4}{N^2}\right\rangle_{t,0} \E\left(\frac{||\bX||^2}{N}-1\right)^2},
%            \end{split}
%        \end{equation*}
%        where we used Cauchy-Schwarz inequality. The right hand side of this last equation goes to $0$ because of Corollary \ref{cor:secmom_bound} and the fact that $||\bX||^2/N\xrightarrow{L^2}1$ (as $||\bX||^2$ is a $\chi^2$ r.v. with $N$ degrees of freedom). On the other hand, we have that
%        \begin{equation*}
%            \left|\frac{d f_{N,1,\nu}}{d\nu}\right| = \left|\E\left\langle \psi_\rho(\lambda||\bx||^4/N^2,\lambda_*) - \ln I_N\left(\frac{\sqrt{\lambda}||\bx||^2}{2N},\frac{\bY_1}{\sqrt{N}}\right) \right\rangle_{1,\nu}\right|
%        \end{equation*}
%        By Corollary \ref{cor:secmom_bound} and Chebyshev's inequality there exists a closed interval $F\subseteq\R$ and a constant $a > 0$ s.t. the probability of $\{||\bx||^2/N\not\in F\}$ is at most $a/N$. Furthermore, (Lemma 14 (1), Fourier View) implies that for all $\theta,\theta' \geq 0$ and $N\geq1$
%        \begin{equation}\label{eq:cont_si}
%            \left|\frac{1}{N} \ln I_N(\theta,\bY_1/\sqrt{N}) - \frac{1}{N} \ln I_N(\theta',\bY_1/\sqrt{N})\right| \leq L |\theta-\theta'|,
%        \end{equation}
%        where $L:= \max\{|\Sigma_{min}|,|\Sigma_{max}|\}+\sqrt{\lambda_*}$. This means that the family of functions of $\theta\in\R$ given by $\{N^{-1}\ln I_N(\theta,\bY_1/\sqrt{N}\}_{N\geq1}$ is uniformly equicontinuous. Then, because Theorem \ref{thm:spher_int} proves the pointwise convergence of this family, this convergence is uniform over compacts. If we define $A:=\{||\bx||^2/N\in F\}$, we then have
%        \begin{equation*}
%            \begin{split}
%                \left|\frac{d f_{N,t,0}}{dt}\right| \leq & \E\left\langle\left| \psi_\rho(\lambda||\bx||^4/N^2,\lambda_*) - \ln I_N\left(\frac{\sqrt{\lambda}||\bx||^2}{2N},\frac{\bY_1}{\sqrt{N}}\right) \right|\mathbb{I}_A\right\rangle_{1,\nu} \\
%                & \ \ \ \ \ + \E\left\langle\left| \psi_\rho(\lambda||\bx||^4/N^2,\lambda_*) - \ln I_N\left(\frac{\sqrt{\lambda}||\bx||^2}{2N},\frac{\bY_1}{\sqrt{N}}\right) \right|\mathbb{I}_{A^c}\right\rangle_{1,\nu}
%            \end{split}
%        \end{equation*}
%        By the uniform convergence of the spherical integral over compacts and a simple application of dominated convergence we have that the first term goes to zero. For the second one, note that \eqref{eq:cont_si} implies that $N^{-1}\ln I_N(\theta,\bY_1/\sqrt{N})$ and its limit are both Lipschitz with constant $L$ and thus this term is smaller or equal to
%        \begin{equation*}
%            \sqrt{\lambda}L\E\left\langle\frac{||\bx||^2}{N}\mathbb{I}_{A^c}\right\rangle_{1,\nu} \leq L\sqrt{\lambda\E\left\langle\frac{||\bx||^4}{N^2}\right\rangle_{1,\nu} \prob(A^c)}.
%        \end{equation*}
%        By Corollary \ref{cor:secmom_bound} we then conclude that this term goes to $0$. Thus, $\lim_{N\to\infty}|f_{N,0,0}-f_{N,1,1}| = 0$.
        
%        Because for a standard gaussian variable $g$, for $k < 1/2$, $\E\left(e^{k g^2}\right) = \frac{1}{\sqrt{1-2t}}$, by (Corollary 6.1.6, Large Deviations) we have that the law of $N^{-1} \sum_{i\leq N} \bx_i^2$ under a standard gaussian measure obeys a large deviation principle with good rate function
%        \begin{equation*}
%            I(x) = 
%            \begin{cases}
%                \frac{1}{2}(x-1-\ln x) & \mbox{if } x > 0 \\
%                \infty & o.w.
%            \end{cases}
%        \end{equation*}
%        Then, by Lemma \ref{lem:varad_hyp} and Varadhan's Lemma we have that
%        \begin{equation*}
%            \lim_{N\to\infty} f_{N,1,1} = \sup_{x\in\R_+} \left(\psi_\rho(\lambda x^2,\lambda_*) + \frac{1}{2}\left(\ln x + 1 - x - \frac{\lambda x^2}{2} \right)\right).
%        \end{equation*}
%        This together with the already proved fact that $\lim_{N\to\infty}|f_{N,0,0}-f_{N,1,1}| = 0$ finishes the proof.
%    \end{proof}
